Understanding and Reducing Metadata-Driven Host Overheads in Sampling-Based GNN Training

Modern deep learning workloads increasingly exhibit dynamic, metadata-driven execution, where runtime-generated information determines memory provisioning and kernel launch decisions. In sampling-based graph neural network (GNN) training, this behavior places the CPU on the critical path, introducing persistent host-device orchestration overhead and frequent GPU-CPU synchronization, which dominate end-to-end runtime when GPU computation is small. Existing approaches, including CUDA Graphs and GPU dynamic parallelism, fail to address this problem because the metadata-driven control loop remains host-mediated, and execution structure varies across iterations. We present ZEROGNN, a system that removes the host from the metadata-driven control loop and enables fully GPU-resident execution under dynamic behavior. ZEROGNN keeps runtime metadata on-device, mediates dynamic execution within a fixed launch structure, and provisions a conservative yet tight execution envelope to restore CUDA Graph replayability. Experiments on sampling-based GNN workloads show that ZEROGNN achieves up to 5.28 x end-to-end speedup, near 100% GPU execution fraction, and memory efficiency comparable to ideal metadata-informed allocation, while enabling strong multi-GPU scaling by eliminating host-side bottlenecks.

==> tex/challenge.tex <==
%Next section examines if we can achieve them together, and also discusses prior works
%{\color{red}
%The simple and extensible nature of {\graphpy}

% Integrating systems research (e.g., writing new kernels to avoid using bitmap in Python, or any other kernel optimization) to any DL framework does not have a standard approach today.
% Unifying and simplifying such integration can provide a very useful platform. 

%If one observes operating systems, POSIX specification made userspace application development very portable and modular. One hardly has to rely on OS-specific header files or follow its internal development guidelines to start developing new application, and enables reusability across POSIX compliant OS. Our work is inspired by such observations, and centers around innovations in the infrastructure and interface design.
%This and next sections explains such challenges, and the novel solutions.
%as well as the extensible use-cases in detail.
%}
% including deep learning and traditional graph analysis.

%\subsection{Challenges and Prior Works} \label{sec.challenges}

% \subsection{Challenge \#1: Tensor and Graph Exchange } \label{sec.science.challenges}

% %\noindent \textbf{and Memory Management.}
% %To provide the DL use cases, we observe that two modules are needed: \textit{\graphpy-Kernel} and \textit{\graphpy-Workflow}. 
% %Table~\ref{table-kernel} provides the {Kernel} APIs, 
% As we pointed out earlier, implementing DL kernels such as gSPMM, etc. alone is not enough as DL training requires support for computation graph, tensor management and back-propagation to update the model parameters. 
% %There exist some DL frameworks such as PyTorch providing automatic support for invocation of back-propagation. 
% %Specifically, the edge of the  computation graph denotes the kernel invocation in the forward computation, the back-propagation calls kernels to perform the gradient computation using the same computation graph but in the reverse order (Fig.~\ref{fig-forward}).
% Back-propagation needs to use the input and output tensors as states (\cref{sec.background.dl}), hence de-allocation of the tensors need to be delayed until back-propagation has used them for each epoch. 
% Moreover, the Kernel APIs also require access of graph $g$. 
% %Graph creation from raw data could be made part of the Kernel, but is actually a standalone operation that could be treated as pre-processing step. 
% It needs a forward graph or its inverse depending on whether a DL kernel is invoked in the forward or back-propagation.  


% Hence, apart from {\graphpy-Kernel} (or Simply Kernel if referring to prior works), we need \textit{{\graphpy}-Workflow} (or simply Workflow), to provide many of these support by itself (computation graph, tensor management, correct graph passing, etc.) or using some well laid out protocols to achieve them together with Kernel module. At the end, we expect to integrate kernel APIs to DL frameworks so that DL training process can happen. 
% Next, we examine how such integration tasks can be achieved currently using DL frameworks.
% %and whether they are simple and obvious or requires huge efforts by researchers and learners. 




% \noindent
% $\bullet$ \textit{Approach \#a.}  Both the Workflow and Kernel modules can be implemented using C++ plugin directly by including the necessary LibTorch header files, and following the specific LibTorch development guidelines. We did not find any existing work that uses this approach, so we implemented this approach ourselves. 

% \noindent
% $\bullet$ \textit{Approach \#b.} In this approach, the Kernel is implemented using C++ by including the necessary LibTorch header files, while using Python to implement the Workflow using LibTorch guidelines. Pytorch-Geometric~\cite{pytorchg2019}, GNNAdvisor~\cite{GNNAdvisor} follow this approach. 

%\subsubsection{Tensor and Graph Exchange: Challenges and Prior Works.}
%\subsubsection{Use DL Framework's Tensor}
%{\color{red}
%DL training requires computation graphs and tensor support, hence GNN systems rely on existing DL frameworks for the same. 



% \subsection{Challenge \#2: Missing Baseline}

% \noindent \textbf{Out-of-Memory Condition and Framework Overhead.}
% Our measurements show that many current GNN systems show out-of-memory condition frequently on even slightly larger dataset in  single GPU setup. 
% Reddit graph, which has less than 230 million edges, can not be trained on A100 GPU which has 40 GB memory by PyG, GNNadvisor on any of their supported models. DGL cannot run slightly complex GAT model, while it still consumes way more than 16 GB memory for GCN, and simple GAT model. Hence, it is unsuitable on low- and mid- grade GPUs that has small memory, such as Nvidia GTX 1080 Ti.
% Hence, many prior GNN systems have only demonstrated smaller dataset for performance, which then are affected due to framework overheads that we discuss shortly. 
% Moreover, many works that do evaluate larger dataset have only focused on kernel benchmarking, but has many issues (\cref{sec.science.challenges}). 

% %DGL~\cite{dgl2019} is another GNN system, however it suffers from many framework level issues, that does not let it function as a baseline system.
% We investigate if end-to-end training performance comparison on smaller dataset can really rank systems based on their kernel performance.
% Table~\ref{table-motivation-overhead} shows overhead for GCN on two smaller dataset of Cora and Pubmed in an A100 Nvidia GPU that includes the time taken by rest of the  Python and C++ code but not kernel time; as well as total training time. The methodology and dataset are described in \cref{sec.exp-gnn.time}. It is very clear from this table that the total training time for Pubmed actually does not depend on the kernel time, as total training time is almost equal to the overhead time. Hence, any optimization of the gSpMM kernel will not show up if using DGL to prototype kernels. However, many systems who use PyTorch's plugin approach to prototype GNN on this dataset shows huge performance improvement compared to DGL. Hence, how can we be sure if the performance improvement is purely due to better kernel implementation and not due to difference in the overhead, when we are not able to evaluate larger dataset. 
% %Also, if the performance improvement is due to overhead differences, how can we propose a better framework that does not cause such huge overhead, and allow us to run larger dataset so that it can be used as better baseline. 

% \begin{table}[t]
% \small
% \vspace{-6pt}
% \caption{Framework Overhead of DGL (in Seconds)} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| c cc|c|} 
%     \hline\hline 
%     Graph & Startup & Runtime & Total & Training\\ [0.5ex] % inserts table
%     Dataset & Cost  & Cost  & Overhead  & Time \\
%     %heading
%     \hline % inserts single horizontal line
%     Cora & 0.828 &  0.512 & 1.340 & 1.347  \\ 
%     PubMed & 0.786 & 0.684 & 1.470 & 1.480  \\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-motivation-overhead} % is used to refer this table in the text
% \end{table}

% %And because of these two costs, DGL performs poorly (more than 2$\times$)  compared to reference implementation (not optimized) of {\graphpy} for GNNs on several dataset, despite DGL kernels performing better than {\graphpy} kernels. Since DGL has a large overhead, it is not surprising that many prior GNN systems~\cite{GNNAdvisor,huang2021understanding}, which do \textit{not} use DGL for their integration, have a huge speedup. \td

% %To this end, {\graphpy} through its lightweight design minimizes both the overheads, and hence is well-suited not only for future systems research prototypes, but also as a baseline to understand the true impact of prior system optimizations.

% Hence, none of the prior systems present a good baseline for end-to-end training on which future system research can do performance evaluation that is needed for progress of system research. 

% %Our limited survey of other works that modified DGL to demonstrate better performance, also relied on CSR/CSC format. We suspect that such researchers may have found that modifying whole DGL Kernel a tedious process when format changes are involved. \td.

% %Hence, the lightweight Kernel module in the plug-and-play eco-system of {\graphpy} provides enough space for innovations without the need to spend efforts on graph preparation or in supporting the APIs that are not applicable for deep learning purpose.

% %Writing interfaces for a new kernel in DGL is still a complex problem due to involvement of tensor library and memory management. 
 

% % %On the other hand, DGL/PyG takes only COO arrays as input in their initialization API. 
% % %Further, the generation of critical boiler-plate code, makes integration effortless. 
% % \noindent \textbf{Sparse Data.}
% % We also implemented {\graphpy-Kernel} for GNN as proof of concept and reference. We mostly focused on CSR/CSC format for reference and comparison, 
% % It includes an unweighted gSpMM kernel to support GCN and GIN; a weighted gSpMM kernel, and two versions of gSDDMM kernel for GAT as mentioned in Table~\ref{table-kernel}. 
% % %Both of these are sufficient for a graph-specific softmax layer, and for edge-level attention score from vertex-level features.
% % We use pull-style computation that avoids usage of atomic instructions: so CSC for forward and CSR for backward computation or wherever inverse graph is needed.
% % We used OpenMP for vertex-level parallelism in CPU. % and use vertex-centric computation.
% % To support GPUs, we implemented kernels in CUDA. The same {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved using $model.to(cuda)$, where cuda is the device context. Similarly, the adapter of {\graphpy-Workflow} allocates tensors directly on GPU.

% % We also implemented another format borrowed from prior graph analytics work~\cite{gstore}, which is very different from CSR/CSC format to demonstrate that an entirely different format can be implemented with same ease, using the same set of Kernel APIs. We used the same {\graphpy-Workflow} code, including the GNN model, graph convolution layers. We do not use that format for comparison.
% % % \noindent 
% % % $\bullet$ \textbf{GPU Support.} 
% % % The specialized kernel is also implemented in GPUs by using the same boiler-plate code. The same {$wrap\_graph$()} API instead of simply wrapping the CPU version of Numpy arrays, it copies them to GPU memory, and then wraps them up in $g$ object. Thus, the rest of the kernel APIs (Table~\ref{table-kernel}) get the GPU version of the graph, and Python binding code of the kernel invokes the GPU kernels. Thus, the same piece of {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved easily using $model.to(cuda)$, where cuda is the device context. Similarly, the {\graphpy-Workflow} allocates tensors directly on cuda or device memory.


% % \vspace{1mm}
% % \noindent \textbf{Motivation and Challenges.}
% % \textbf{Challenge \#1. Graph Data Engineering.}
% % All graph data science works assume that the graph representation already exists. In other words, if the data scientist wants to use the prior system techniques of graph analytics works, they need to first perform the graph data engineering task to create a graph representation in the right format from the raw data. The raw data could be in any readable format, starting from a plain graph format to a CSV, JSON, XML or binary files.

% % Also, the graph representation varies slightly from case to case. E.g. in GCN case, the graph is assumed to be a simple graph having no edge properties. But in case of knowledge graph, each edge has a edge or relationship type, that is stored as part of the graph. Further, attention based GNNs such as GAT need to keep attention score for each edge of the graph. 
% % However, preparing graph representation does not stop here. Recent works~\cite{hamilton2018embedding} have used various other data engineering tasks including sampling, community identification, union of sub-graphs etc to prepare the final graph representation.\td {write down a few lines here}
% % \td. What are other variations?

% % Hence, capability to create graph from raw data, as well as post-processing steps to create the final graphs is desired to ease the job of deep learning on graphs, and requires supporting graphs with arbitrary vertex and edge properties.
% % This procedure is not only difficult and time-consuming, but also ad hoc{\td} a few more keywords. 

% % Further, this capability must be a part of python programming environment, as it has become a de-facto programming environment for data science. It has an interpreter based execution, and no good support for multi-threading, the actual computation happens using back-end, which is written in high-performance languages like C/C++ and CUDA. 
% % Unfortunately, the like the current GNN systems, the prior graph analytics works also lack support for data engineering operations. GNNs expect the data scientists to do all the data engineering tasks to create this limited representation as they support just one type of graph with no edge properties, E.g., NeuGraph does not support attention based GNNs yet.

% % On the other hand, there are a few python based graph data engineering frameworks, such as NetworkX, which is being used by DGL. However, it is purely python based package, and  stores the graph data in  python using dictionary of dictionary format. 
% % The graph representation of NetworkX needs more memory space, have scalability problem. If the graph structure is large, it cannot fit into the memory, and suffers due to absence of good multi-threading in the python programming environment.
% % Hence, one can conclude that GNN systems are limited by the scalability of pure python packages. 
% % Therefore, the data engineering tasks preceding the deep learning kernels must be performed in a high-performance back-end to provide a uniform experience, high performance and scalability to larger dataset.


% % \textbf{Challenge \#2. Implementing Deep Learning Workflow.}
% % The second challenge is on how to use the existing code base of prior works that have proposed novel systems design to test the efficacy of their techniques in the field of deep learning. Since, these works mostly offer GAS or sparse linear algebra based programming framework, they are well-suited to support the kernels required by GNNs. Hence, the question here is what it takes to integrate such code base to do the GNN operations, specifically how to minimize the changes that are required to make this code base ready for deep learning, such as gradient computation without requiring huge coding.

% % \begin{figure}
% %   \includegraphics[scale= 0.26]{result/framework.pdf}
% %   \caption{The framework of {\graphpy}}
% %   \label{fig:boat1}
% % \end{figure}    




==> tex/extend.tex <==

\begin{table}[t]
\footnotesize
\caption{\small {\graphpy-GNN} System APIs. Goal: a) Passing graph object as is, and remaining independent of DL framework; b) Their implementation must invoke the CUDA or device kernels internally.} 
\vspace{-6pt}
\centering % used for centering table
\setlength{\tabcolsep}{1mm}
\begin{tabular}{|l|} % centered columns (4 columns)
    \hline %inserts a single line
    % \textbf{Graph Handling APIs (\cref{sec.engg})} \\
    % \hline
    % g  \hspace{8mm} wrap$\_$graph(np$\_$array, np$\_$array, np$\_$array, np$\_$array, dict$\_$param) \\
    % status \hspace{2mm} save$\_$graph(g, path) \\
    % g \hspace{8mm} load$\_$graph(path) \\
    % % \hline
    % % \hspace{6mm} \textbf{APIs on $g$} \\
    % % \hline
    % % int \hspace{14mm} get-vcount1() \\
    % % int \hspace{14mm} get-vcount2() \\
    % % np$\_$array \hspace{6mm} get-degree1() \\
    % % np$\_$array \hspace{6mm} get-degree2() \\
    % \hline
    \textbf{{\graphpy-GNN} APIs for System Integrator (Not for Data Scientist)} \\
    \hline
    status \hspace{2mm} gSpMMv(g, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    % \hline
    status \hspace{2mm} gSpMMveid(g, \textit{in-tensor}, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    status \hspace{2mm} gSpMMeid(g, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    % \hline
    status \hspace{2mm} gSDDMMvv(g, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    status \hspace{2mm} gSDDMMve(g, \textit{in-tensor}, \textit{in-tensor}, \textit{out-tensor}, eFn, Flag)\\
    \hline
    % status \hspace{2mm} spmm(g, \textit{in-tensor}, \textit{in-tensor}, \textit{out-tensor}, Flag)\\
    % % \hline
    % status \hspace{2mm} sddmm(g, \textit{in-tensor}, \textit{in-tensor}, \textit{\textit{out-tensor}}, Flag)\\
    % \hline
\end{tabular}
\label{table-kernel} % is used to refer this table in the text
%  \vspace{-2pt}
\end{table}



\subsection{{\graphpy}: GNN Specific Design} \label{sec.baseline}

We design {\graphpy} Based on the above analysis. It has two components, {\graphpy-Kernel} which is responsible for CUDA kernel API definition and implementation, and {\graphpy-GNN} which interfaces Pytorch using Python binding, and internally calls {\graphpy-Kernel} CUDA APIs. 

\subsubsection{Storage Format} 
We take advantage of dataset symmetry and store just the CSR topology that serves as both the CSR and CSC. For the COO, it is stored in CSR-way, and hence it shares the format with the CSR storage. 

For the transpose need of an edge-level tensor, we decided to use the edge ID rather than developing transposed gSpMM versions. The reason is that the algorithm for transposed gSpMM is not well developed by the community. Our naive version relied on a naive scatter method where each row scattered message atomically to every non-zero column using an atomic instruction. Secondly, it requires the support of various reduction operations, for which atomic operations are not supported out of the box. We believe transposed gSpMM requires its own independent discussion, and leave it as a future work.   

Hence, we decided to rely on the edge ID abstraction but store the edge ID for CSC only. CSR is assumed to be containing an implicit edge ID to CSR. Since the COO shares the CSR storage, both of them have an implicit edge ID. Thus, only one edge ID array is stored.
In total the format costs CSR $(|V| + |E|)$ + COO ($|E|$) + Edge ID array ($|E|$). Thus reducing the memory consumption by almost 3$\times$ due to storage design alone compared to DGL without introducing any trade-off.
%where the last $|E|$ is for COO as half of its storage is shared with CSR.

\subsubsection{APIs}
We now present kernels that are directly suited for Class A and B GNN use cases based on the insight gathered from the design analysis. The APIs (Table~\ref{table-kernel}) are directly invoked by {\graphpy-GNN} system to avoid the kernel mismatch without any need for any additional intermediate kernel.
We define usual gSpMMve, and gSDDMM. However, we introduce two different kernels compared to prior works to take care of GNN-specific requirements.

%without incurring any requirement mismatch overhead. %The proposed CUDA kernels have almost similar signatures as the system APIs of Table~\ref{table-api}. {\graphpy} internally defines and designs GNN-specific kernels, 
%Hence, the proposed internal CUDA kernel signature follows a similar signature as the system API to directly map the requirements. This was needed to show that avoiding the generalization cost of prior kernel design can save memory and gain performance.


\noindent \textbf{gpk$\_$gSpMMveid.}
This {\graphpy} kernel is a weighted gSpMM that accepts a vertex-level and an edge-level tensor. However, it accesses the edge-level tensor using edge ID which is part of the graph storage. We also support a vector feature for each edge, which is used by the multi-head GAT model.

%\textit{gSpMMveid} invokes just one kernel that directly expects a graph with edge ID to avoid the need for a separate eShuffle CUDA kernel and never generates additional intermediate results. It is used to perform transposed gSpMMve.
Memory saving and performance gains are achieved by {\graphpy} just because of the new API design compared to all prior systems. (1) It accesses the edge-level tensors directly using the edge ID, hence eShuffle kernel is completely avoided, and so is the need to materialize an additional tensor of size O($|E|$), thus saving memory. (2) This kernel is faster than even a workload-balanced gSpMMve plus a separate eShuffle kernel. (3) The multi-head gSpMMveid cannot be simulated by the CuSparse-compatible gSpMMve kernel.


% To recap, our investigation in \cref{sec.obs} and \cref{sec.usecase} pointed out that not just DGL (or CuSparse), but many others~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} have continued developing CuSparse compliant-gSpMMve for GNN use-cases.  
%for at least class B GNN, namely gSpMMveid, while many still provide gSpMMve for class A GNN. 
%Also, APIs for CuSparse are not well-suited GNN use cases as discussed in \cref{sec.dgl}, which other works continue to optimize, such as gSpMMve, and not gSpMMveid which they should. 
%We define new signatures of \textit{gSpMMv} and \textit{gSpMMveid}. 

 
% Similarly, \textit{gSpMMv} system API invokes a kernel definition that does not need any dummy edge-level tensors and supports normalization by degree as an option. The forward gSpMMv in GCN uses this option, but backward gSpMMv does not rely on this kernel fusion. However, it invokes normalization separately before calling the gSpMMv cuda kernel. 

\noindent \textbf{gpk$\_$gSpMMv.}
This kernel is unweighted gSpMM. Hence, it only accepts a vertex-level tensor as input along with reduction operation type, such as \textit{sum, min, max} but not any edge-level tensor. The API also accepts an optional boolean flag to indicate normalization by degree flag. When the flag is true, it only normalizes the result of gSpMM as part of the same kernel. Hence, in the backward computation, the flag should be set as false, and a separate normalization kernel should be called. This API is used by class B GNNs. 

This kernel definition, though very intuitive 
%differs from prior works. CuSparse, FeatGraph, Huang et al offer gSpMMve. GNNAdvisor does not make normalization optional and ends up with the wrong fusion during backward. GE-SpMM has mostly focused on gSpMMve, and silently implements gSpMMv without the normalization option. 
provides substantial memory saving to {\graphpy} on two accounts. (1) Compared to CuSparse compliant gSpMMve, {\graphpy-GNN} never need to allocate dummy edge-level tensor saving O($|E|$) memory. This also results in a substantial performance gain. 
(2) Even in the case of a separate normalization, {\graphpy} uses the same tensor as input and output both by using in-place normalization inside {\graphpy-GNN}. 
%On the other hand, DGL performs normalization at the Python level using  PyTorch's CUDA API that can only perform out-of-place normalization, Thus increasing the memory consumption by O($|V|$*feature-length). Hence, DGL-integrated systems, such as GE-SpMM and FeatGraph likely to consume additional memory as well.


% We did not define gpk$\_$gSDDMMveid, as we generated COO in a way that can rely on an implicit edge ID equivalent of the position of each edge in the COO. %to use gpk$\_$gSDDMMve. 
% %COO offers edge-parallel implementation, which achieves fully workload-balanced implementation. 

% \noindent \textbf{gpk$\_$gSDDMMvv.}
% It remains the same as discussed in \cref{sec.obs}.



% \noindent
% \textbf{1. Framework Overhead Reduction.}
% %\red{DGL has significant overhead for small datasets. To reduce the Framework overhead, }
% Prior works reduced framework overhead by moving the model layer to C++, which did not follow the guidelines property, as it could be complex to write those correctly. We left the model layer code in Python. However, we reduced the framework overhead by removing the system initialization steps of DGL which allocates many intermediate memory objects to bridge the requirement mismatch which takes a huge time (\cref{sec.exp-gnn}). 
% %dummy edge-level tensors, 
% Further, {\graphpy} uses code generation to define and implement interfaces. In doing so, it generates separate interfaces for each gSpMM and gSDDMM variant, thereby simplistic nature of {\graphpy} interfaces can invoke the right kernel variant quickly as we avoid having a message passing infrastructure and other overheads of DGL to locate the exact kernel variant to invoke. 
% %Further, for fused kernel design, {\graphpy} generates a new kernel from the DSL specification of the kernel. 
% Therefore, {\graphpy} optimized the training for small datasets.


% As we mention in \cref{sec.usecase}, DGL relies on CuSparse which creates requirement mismatch, hence DGL invokes additional kernels while materializing many intermediate results. We explain  how we remove these overheads.
% %class A type of GNN models use the unweighted sum for aggregation and use vertex-level tensor only. 
% %Class B type of GNN models touches both vertex level and edge level tensor. 
% %DGL uses gSpMMve kernel to handle  this. \red{ which involves extra unneeded computation. To optimize this situation, } {\graphpy} separates the gSpMM kernel into two specific designed kernels: gSpMMv designed for class A GNN which does not fetch the edge level tensor;  gSpMMve, designed for class B operates on vertex-level and edge-level tensors. \red{Since gSpMMv kernel does not fetch the unneeded edge-level weight anymore, the class A type of GNN models can achieve both better memory-saving and better time-saving. }
% (a) DGL uses a dummy edge-level tensor with each value as 1.0 to implement gSpMMv using CuSparse API, we directly implement gSpMMv without this dummy edge-level tensor. 
% (b) CuSparse does not offer edge-ID indirection, hence DGL first re-arranges the edge-level tensors using the edge ID, called \textbf{eShuffle}, for each gSpMMve kernel invocation. {\graphpy} supports merges eShuffle inside its new gSpMMve implementation using edge ID in its graph storage.  (c) DGL does \textbf{two additional transposes} using CuBLAS library because CuSparse API that DGL uses expects tensors in column-major layout. 
% %Here is a comment from its code base re-produced almost verbatim that explains the rationale: “\textit{We use CuSparse to perform the following operation: C = A x B, where A is a sparse matrix in CSR format, and B is the dense matrix for the node feature tensor. However, since CuSparse only supports column-major, while our tensor is stored in row-major, the actual computation is: C = trans(A x trans(B)). Currently, we use CuBLAS to implement transposition and allocate intermediate workspace memory for this.}''.
% (d) CuSparse API does not fuse normalization by degree array; hence, DGL calls normalization separately using PyTorch API in Python. {\graphpy} gSpMMv kernel is written using template meta-programming which uses normalization as a template parameter and hence can handle both cases efficiently. 

% \textbf{3. No Transpose and Shuffle Kernels.}
% \red{Unlike existing works, {\graphpy} removes the need for some computations by re-defining the computation kernel. For example, In both the class A and class B type of GNN models, {\graphpy} avoid the need to transpose on vertex-level features as our gSpMM variants support row-major operations directly.}
% % For both the GNN classes, we avoid the need to transpose on vertex-level features as our gSpMM variants support row-major operations directly.
% %For class A type of GNN, Without integrating with CuSparse, GraphPy can omit the requirement that the input should be column-based. Therefore, two additional transpose computations are not needed. 
% %By removing these additional computations, our end-to-end time does speed up. 
% For the class B type of GNN, GraphPy introduces an edge ID directly as an edge property in the graph using DType, and gSpMMve uses the edge ID directly in the computation. Hence, it also removes eShuffle kernel. By removing this kernel, we do not need to materialize the shuffle output.

% \textbf{4. Kernel Fusion with careful investigation}
% Although existing works fuse several kernels to improve the performance, they~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn} fuse the kernel wrongly. By realizing these issues, 
% {\graphpy} fuses the kernel carefully by understanding the requirement from an end-to-end systems perspective.  For example in GCN, {\graphpy} performs the aggregation first and then normalizes the result with the degree array in the forward direction. However, in backward, {\graphpy} normalizes the input tensor first and then performs the kernel computation. 
% Similarly, for gSpMMve, {\graphpy} implicitly fuses eShuffle and gSpMM computation.
% %Therefore, {\graphpy} can be viewed as the improved baseline. (\td measure our way is slow. Gnnadvisor is wrong but fast)



% \subsection{Optimizations}
% \label{sec.optimization}

% % \begin{figure}[h]
% %   \includegraphics[scale= 0.5]{result/mul_graph.pdf}
% %   \caption{Supporting sparse models need for multiple graphs. It can also be a bipartite graph, such as layer parameters of sparely connected layer.}
% %   \label{fig-mul_graph}
% % \end{figure}

% % It should be noted that this specific kernel is also a from of SPMM, but it is truly SPMM unlike the weighted aggregation that is used in GAT. Specifically, in GAT, the vector feature vector of each vertex is multiplied with a scalar attention score of each edge before aggregation (which is more like SpMV). But in sparse connected layer, it is truly SpMM where input dense matrix is multiplied with sparse tensor matrix.


% The focus of the paper is on the interface design, and abstraction of common tasks to independent modules, however we do implement some known parallelization strategy, which makes our kernel implementation different than DGL and Pytorch Geometric (\cref{sec.exp}). We also propose following new optimizations to demonstrate that new optimization can easily be implemented.

% \noindent \textbf{Edge ID Reordering.}
% We observe that sparse version of fully connected layer and GAT, both keep edge-level tensors or weights, which is used by forward computation, and accepts gradients during backward. This is different from traditional graph analysis where edge does not need to materialize the edge level messages. So, the performance is sensitive to how the edge IDs are allocated to the edges to avoid performing random read and write to edge level tensors. Current allocation scheme is to allocate edge IDs sequentially based on edge log, which results in random edge IDs in both the CSR and CSC, as both are involved in the computation.
% % However, we can only provide sequential edge ID in one of them. 
% We propose reordering the edge IDs in CSC to allocate them sequentially. That is, the in-neighbor list of vertex 0 was allocated edge IDs from 0 to N(0) (the length of in-neighbor list of vertex 0). Similarly, the in-neighbors of vertex 1 was assigned from N(0) to N(0)+N(1), and so on. 
% % Thus, edge IDs in CSR became random. 
% We were able to achieve this easily by writing a custom code inside $wrap\_graph()$ API of the kernel.

% We also have the option to regenerate COO format to provide it sequential edge IDs as per allocation in CSC. This was useful for SDDMM kernels to increase the parallelism. Hence, we are able to achieve sequential edge IDs in two of the graph formats, while prior works had sequential edge IDs only in COO, and not in CSR and CSC.

% \noindent \textbf{Kernel Fusion.}
% For GCN model, we observe that it performs tensor normalization by dividing the tensor elements with vertex degree. We fused this operation with the GCN's core kernel (gathering features of neighbors of a vertex to update the self). Kindly note that the order of normalization and gathering features changes in the backward computation compared to forward computation. Hence one must take care of this fact while fusing the kernel.

==> tex/impact.tex <==
%\section{GNN Training: Observation and Analysis} 
\section{Impact Analysis} \label{sec.impact}

In this section, we discuss the impact of these pitfalls. We include how these pitfalls affect the realistic performance when deployed. Moreover, we categorize these pitfalls into different levels of pitfalls based on their severe degree. Table~\ref{table-pitfall} shows the result. (\td not dangerous pitfalls make our paper weak. we can say that section 5 is not comprehensive long-term thinking, it is piece-by-piece works, lacks of unifying end-to-end system-level pipeline thinking )



\begin{table}[t]
\small
%\vspace{-6pt}
\caption{\small category the pitfalls based on their severe degree.} % title of Table
\vspace{-6pt}
\centering % used for centering table
\begin{tabular}{|l| r|r |r|r|} 
    \hline\hline 
    %heading
  %  \cline{2-7}
    Pitfalls & normal & dangerous  \\
    \hline % inserts single horizontal line
%    Cora & 1,719 & 1,349   & 1,719 &1,375 &&\\ 
%    PubMed & 1,767 & 1,395  &1809& 1,503 && \\
%    Citeseer& 1,697&1,381   & 1,759 &1,409 &&\\ 
    P1 &  & \checkmark \\
    \hline 
    P2 &  & \checkmark \\
    \hline 
    P3 & \checkmark &\\
    %OGB-Pr & 25,551 &OOM & 20,789 & OOM  &32,285& OOM\\
    % & 76.47 &  76.52 & & \\
    \hline %inserts single line
\end{tabular}
%\vspace{-6pt}
\label{table-pitfall} % is used to refer this table in the text
\end{table}


==> tex/intro.tex <==

\section{Introduction} \label{sec.intro}
%Getting insights from data is very important, and hence 
Many applications have become data-driven today. 
%These applications are now popularly known as \textit{data science}. 
Within this ecosystem, a lot of real-world data can be stored as \textit{sparse matrices} or \textit{graphs}, such as social networks, chemistry, biology, recommendation system, scene description generation, knowledge bases, etc~\cite{fan2019graph, zitnik2018modeling, schlichtkrull2018modeling,hamilton2018embedding,ying2018graph,krahmer2003graph,perera2017recent,rgcn2018,wang2020entity}. 
%We call these data-driven use-cases as \textit{graph data science} 
To this end, many graph neural network (GNN) models, e.g., GCN~\cite{gcn17iclr}, graph attention network~\cite{gat18iclr}(GAT), GIN~\cite{xu2019powerful}, and others~\cite{gatedgraph2017,zhang18, graphsage17}, etc. have been proposed. 



% \noindent \textbf{Deep Learning on Sparse Data.}
% The neighborhood in graphs is different from other regular data, such as an image which has a fixed number of neighborhoods. To handle it, \textit{graph neural network}(GNN), has been proposed~\cite{gcn17iclr,gat18iclr,gatedgraph2017,gaan2018}. The GNN models can be trained efficiently if the graph can be used for storage. However, the current DL frameworks, such as PyTorch~\cite{pytorch2019} or TensorFlow~\cite{tensorflow2016} lack the same level of operational support for the sparse matrix that they have for dense matrix, as the original code-base of GCN~\cite{gcn17iclr}, GAT~\cite{gat18iclr} etc. have relied on bitmask at Python level to model sparsity on top of dense matrices that actually do not reduce computation or memory consumption. %because the underlying kernel still uses the dense matrix.


% traditional GNNs use the adjacency matrix to represent the graph structure and tensor operation to perform the forward and backward computations. 
% However, due to the sparsity, this will trigger the out-of-memory problem to represent a sizeable sparse graph and will cause computation inefficiency for tensor operation. 

% Since deep learning techniques can achieve excellent prediction, many graph neural network (GNN) works were proposed. Graph neural network (GNN) is about applying deep learning algorithms on the graph structure to do classification and prediction tasks, such as node classification, edge/link prediction, and graph classification. 
% The node classification denotes that given a graph structure and a subset of nodes with labels, the graph deep learning algorithm should predict the label of the remaining nodes. 
% In contrast, the link prediction tasks are predicting whether an edge exists between two given nodes or not, such as in auto-completing knowledge bases.


% \noindent \textbf{Deep Learning On Sparse Tensors.}
% DL Model compression techniques, such as weight pruning ~\cite{han2015learning,han2016iclr},  convert a dense model layer to a sparse layer by removing a lot of low-impact model parameters. 
% These techniques help to deploy large models on resource-constrained devices because the compressed models need less memory and CPU. Before deploying them, the compressed models undergo \textit{re-training}. This re-training step can be more efficient if the graph is used to model sparse layers. However, prior works~\cite{han2015learning} used bit-mask matrix in Python, and underlying dense matrix to achieve sparsity. Thereby, the \textit{re-training process did not really consume less memory}, hence we may not be able to use resource-constrained systems to do re-training, which are low on memory.

%These models also have inspired a number of systems optimizations~\cite{wang2021gnnadvisor,huang2021understanding,gespmmsc2020,fu2022tlpgnn,wu2021seastar,chen2020fusegnn}. However, our study finds that many of these design decisions indicate inadequate understanding because 

It should be noted that GNN is a special kind of deep learning (DL) model, and hence its training has a unique computation need. \textit{Forward computation} calls many \textit{kernels} (operations on data) from the input layer to the output layer to derive the prediction values which are compared with the ground truth to calculate the loss.
% and plug the loss into the backward procedure. 
Then, \textit{backward computation} uses the loss to derive the gradient by invoking kernels from the output layer to the input layer to update the model parameters.
%It uses the chain rule of gradient back-propagation to update the model parameter from it. 
Kindly note that the backward computation accesses results that are either accessed or produced in the forward computation and are called \textit{state tensors} (Fig.~\ref{fig-format}(a)). This computation paradigm differs from the prior forward-only related fields, e.g., graph analytics.
 
\noindent \textbf{Motivation: Missing End-to-End Focus.}
 Many prior GNN system optimization works~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing,yan2020hygcn,liang2020engn,zhang2021boostgcn, geng2020awb} have established a clear trend of not measuring the GNN training accuracy, and many have only implemented forward computation.
%Many prior works either do not provide a full GNN model for training or do not measure training accuracy, 
Our analysis shows that it has led to significant practical issues, including questioning their proposed optimization techniques as presented next. %including the

Consider the case of the GAT model that calls 18 kernels in each layer~\cite{fu2022tlpgnn} in its forward computation. An obvious optimization technique is to fuse them into just one, as done by prior works~\cite{fu2022tlpgnn,huang2021understanding}. However, they have not implemented backward computation. The absence of end-to-end focus allowed them to avoid materializing the edge-level tensor($W_e$, a trainable GAT model parameter), and thereby not keeping edge ID(\cref{sec.background}) in their graph to access the same. 
Similarly, GNNAdvisor~\cite{wang2021gnnadvisor} does not measure the training accuracy. We point out that its codebase does not fuse the kernel correctly in the backward computation of GCN, and its model does not use bias, a vital model parameter, gaining performance unknowingly at the expense of accuracy. 

Hence all their demonstrated optimizations are not yet practical and require more investigation to implement backward computation to show training accuracy, which is likely to alter the very basic foundation of many proposed optimizations.
%Such additional steps would have enforced a brainstorming around the need for \textit{state tensors} and other GNN-specific requirements. 
%Fused kernels that avoid producing such tensors in the forward computation must implement backward computation to show that such fusion is feasible and justify them through training accuracy measurements.
%do not understand the system requirement from the GNN perspective. 
%Unfortunately,
%Hence, their optimization has no significance at this moment. We present various such observations in \cref{sec.obs}, however, the pressing question is whether such optimizations really advance the state-of-the-art. 
%and whether these mistakes are systematic.


%Further observations point us that many researchers do not understand GNN workflow exactly
%For example, 

%GE-SpMM~\cite{gespmmsc2020} forgets to consider the edge-level tensor when implementing the kernels. Section (\td) explains this analysis in detail. 



%\noindent \textbf{Systematic Lack}:
%We argue that these mistakes are systematic in nature. We present the following arguments to explain it. 

% No architecture papers \cite{yan2020hygcn,liang2020engn,zhang2021boostgcn}
%{\td  \cite{zhang2021boostgcn, geng2020awb, yan2020characterizing} only for inference and no accuracy}: Will see them later whether to include or not.
%\cite{baruah2021gnnmark} uses dgl and pyg, so not citing here.

%--------------
%(1) \textbf{No Training Accuracy Measurements and/or Missing Backward Computation.} 
% Indeed many prior works~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing} do not measure the training accuracy either because they do not implement the backward computation or simply do not measure it despite having an end-to-end implementation.
% Hence, they may be totally unaware of the mistakes. 
% For example, GNNAdvisor~\cite{wang2021gnnadvisor}, and end-to-end GNN system does not fuse the normalization kernel correctly in the backward computation, while omitting the bias parameter from each GCN  layer (\cref{sec.obs}).
% %provides a more detailed analysis for this example). 
% Similarly, Huang et al~\cite{huang2021understanding}, and TLPGNN~\cite{fu2022tlpgnn} optimized the GAT model's forward computation without implementing its backward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. Wrongly fused kernels can also alter the requirement significantly as they do not keep edge ID in their graph to access the attention score tensor in GAT(\cref{sec.obs}).


%Clearly, the research community has also not forced these works to measure training accuracy. 

%in form a natural boundary across which they cannot be blindly fused in the forward computation as they are needed in the backward 

% (2) \textbf{No Backward Computation.} Many prior works~\cite{huang2021understanding,fu2022tlpgnn}[\red{what about seastar and other works}] have not implemented a backward computation at all, and their optimizations focused on only the forward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. We believe general awareness of GNN workflow and understanding is lacking, such as the need for \textit{state tensors}. Kernels producing such tensors form a natural boundary across which kernels cannot be fused in the forward computation. Wrongly fused kernels can also alter the requirement significantly. For example, Huang et al\cite{huang2021understanding}, and  TLPGNN\cite{fu2022tlpgnn} do not keep edge ID in their graph to access attention score tensor in GAT(\cref{sec.obs}). %(Section {\td} provides a more detailed analysis for this example). 
% %This mistake will be realized easily if these works implemented the backward kernel.
% % (3) One of the observations from such works is that they try to write GNN systems from scratch using current DL frameworks, such as PyTorch, TensorFlow, etc. 

% We explore the current methodology and find that it is very complex to write a GNN system from scratch because  passing the graph object and tensors to an independent module is very complex, and on top of this, users have to learn new build systems (Ninja), Python binding, memory management (due to delayed free of state tensors), etc. to integrate their code with a DL framework. We experienced the same issues ourselves when we tried to build a new baseline that resulted in exhaustion in just setting up the system. And, hence such exhaustion may force the researchers to not build an end-to-end system. 


%\noindent \textbf{End-to-End Systems Teaching.} 
%The academic community is also not encouraging end-to-end \textit{system} teaching. E.g., publicly listed assignments on DL/GNN {systems} courses offered by many universities~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} \textit{focus only on the forward kernel} of an operator, and in Python without its integration in an end-to-end DL/GNN system. Hence, students cannot fully understand, appreciate, and gather complete requirements. Rather, industry partners have voiced concern about the availability of candidates with good systems and data science knowledge in an NSF workshop~\cite{storage2025NSF}.


%On the other hand, writing a GNN system from scratch gives the new system an immediate performance advantage, and we empirically show that prior work has been implicitly removed once other works develop a GNN system from scratch rather than integrating with DGL. can achieve performance improvement easily without any actual systems optimization. 

\begin{figure*}[t]
  \includegraphics[scale= 0.55]{result/edge_id_crop.pdf}
  \vspace{-12pt}
  \caption{\small (a) One GNN layer using GAS (gather-apply-scatter) to model the kernel: X and Y are intermediate features, and $W_e$ is the model parameter of the layer, e.g. attention score in case of GAT. X, Y, and $W_e$ tensors are \textit{state}, as they are used in backward. $A$ and $A^T$ are graph and its inverse respectively. (b) Sample graph (c and d) CSR and CSC representation along with edge ID indirection.}
  \label{fig-format}
 \vspace{-12pt}
\end{figure*}



\noindent \textbf{Contribution.}
This paper, called \textbf{\graphpy}, presents our observations that system optimizations based on a partial understanding of the GNN model may not lead to a practical system. {\graphpy} highlights the need for end-to-end model implementation to measure accuracy before showing the performance gain. 
To this end, {\graphpy} presents an ecosystem to perform it productively, and have following contributions. 

% focuses on two goals:
% (1) Writing a new GNN baseline by focusing on overhead reduction.
% (2) Explaining the critical pieces of the resultant architecture that has been extracted to develop an education and research tool to encourage the implementation of end-to-end DL/GNN systems. A detailed explanation of these contributions is below.


\noindent
\textbf{1. In-Depth Analysis (\cref{sec.obs} and \cref{sec.usecase}).}
We are the first ones to analyze existing GNN system optimizations, the current practices to integrate GNN systems to a DL framework, and the interfaces between GNN systems and the low-level GPU kernel implementation. A brief summary is provided here.

\noindent $\bullet$
\textbf{Accuracy and Performance Benchmarking.}
We observe many critical benchmarking issues due to missing end-to-end model implementation, and the absence of training accuracy measurements. 
{We also point out that relying exclusively on smaller datasets to show performance gain as done by prior GNN systems~\cite{wang2021gnnadvisor,gespmmsc2020} does not compare the impact of kernel performance but rather compares \textit{framework overhead}. To this end, we are the first to develop a  \textit{methodology} to measure the framework overhead. Overall, the investigation {questions the practical aspects of many proposed optimizations}.
%These issues also make DGL~\cite{dgl2019} the only end-to-end reliable \textit{baseline} that can be used to quantify the performance of future GNN systems. despite claims in several recent publications~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,gespmmsc2020, wu2021seastar,chen2020fusegnn,featgraphsc20}. 
%These issues lead to two important use cases for which several interface-level limitations exist today as explained below.
%The full model implementation and accuracy measurement is needed to show the correctness of the developed kernel.  

% \red{\noindent $\bullet$
% \textbf{Framework Overhead Analysis and Methodology.}
% We are the first ones to state that the performance evaluation should rely on large data sets instead of the small data set because the overall training time in small data sets is dominated by the GNN system's framework overhead. Based on this observation, we also propose a methodology that can evaluate the framework overhead.}

\noindent $\bullet$
\textbf{DL Framework to GNN System (high-level) Interfaces.} End-to-end prototyping is needed to measure the accuracy to avoid the mentioned issues. But current DL frameworks do not allow passing any custom object, such as a graph to GNN systems, leading to reliance on workarounds for integration. This results in unstable system APIs whose signature changes for every custom graph storage. It deters innovation in graph storage and causes productivity and compatibility loss. %Hence, prior tools do not encourage end-to-end GNN system development.
%tensors to an independent module is very complex,
%out that a few GNN systems have critical issues in understanding system requirements, implementation 
%(a) The performance improvement stated in many prior works is not useful and prohibits their deployment to real-world GNN applications.
%{(b) Need of a Better GNN Baseline:}
%In this work, we observe (\cref{sec.obs}) many such issues in existing works, including an absence of end-to-end model implementation, avoiding training accuracy measurements, etc. 
%As we study code base of prior works and evaluate their work, we find that the optimization achieved by these works cannot be relied upon as they do not fully implement the GNN model correctly. Hence, 
%they would have benefited by following our recommendations such as enforcing GNN training accuracy, and using larger datasets for performance measurement.
%Similarly, assignments and tools should be developed to impart an end-to-end understanding of DL/GNN systems to future systems researchers and engineers.
%while the performance measurement should happen on larger datasets.


\noindent $\bullet$
\textbf{GNN Systems to CUDA kernel (low-level) Interfaces.}
CuSparse library defined general-purpose sparse kernels over a decade ago. However, it is not directly suited as kernels for GNN use cases. This low-level interface mismatch introduces extra memory allocation, additional kernel calls, and the materialization of intermediate results causing a slowdown and increased memory consumption in DGL. However, others~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} continue to optimize the same kernel definitions and suffers from the cost of generality and mismatch.

\noindent
\textbf{2. Research Tool (\cref{sec.usecase} and \cref{sec.science}).}
To this end, {\graphpy} \textit{auto-generates codes to integrate GNN systems to DL frameworks} based on a simple domain-specific language. 
%users to write the kernel, called \textit{\graphpy-Kernel} independently without involving any DL frameworks, and have no version dependency whatsoever. {\graphpy} 
It relies on a proposed \textit{Half DLPack protocol} to offer DL framework-specific tensors to GNN systems using flat arrays. This achieves DL framework-independent GNN system, which in turn, removes all restrictions on passing graph objects to it. Further, {\graphpy} proposes \textit{graph storage management} module to prepare and export graphs to GNN systems as per GNN-specific graph edge property requirements. 

Through these mechanisms, {\graphpy} achieve \textit{productivity and re-usability} of GNN system across DL frameworks and their versions and also streamlines the interfaces for graph handling.
Further, we are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

%The proposed tool also reduces the framework overhead due to its simplistic design. 

 
%\bullet$
%\noindent
%\textbf{3. Graph Storage Management (\cref{sec.engg}).}
% Analyzing different GNN models shows the need for graph storage with different edge properties. The current ad hoc approaches to handling graph storage present another productivity issue and a challenge to interface design and system integration. 
% We separate the graph storage management to another independent module to prepare graphs by specifying GNN specific edge properties succinctly using a single API. The API exports the prepared graph using \textit{zero-copy} arrays to the GNN system. 
% We are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

%to satisfy the diverse storage needs of various classes of GNN, which cannot be supported by current tools.
%to achieve better performance in graph preparation and productivity in
%By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) same as dense matrix (e.g., image data) for storage specification and exchange purpose. 
%Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.


% $\bullet$
\noindent
\textbf{3. GNN Inspired Kernels and an Optimized Baseline (\cref{sec.baseline}).}
We capture the system requirement using a new set of kernel definitions  that can directly be used inside GNN systems without any requirement mismatch and memory overhead. 
Based on these new kernels, we present a new GNN baseline 
%by removing the various overheads and fusing the kernels by carefully studying the GNN models
ensuring correct training accuracy and better performance amid low memory consumption. 


%presents much more than memory and performance optimization. It rather establishes a new  

% \noindent $\bullet$ 
% \textbf{Graph Data Management for DL.}
% We separate the graph storage management to another independent module, \textit{\graphpy-SM}, to handle multi-field graph properties using a single set of API by using \textit{NumPy Dtype}, while exporting the prepared graph storage to {\graphpy-Kernel} using \textit{zero-copy} NumPy arrays. 
% %and allow innovations in interface design
% By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) the same as a dense matrix (e.g., image data) for storage specification and exchange purposes. 
% Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.
% We are unaware of any high-performance Python package that can support arbitrary multi-field graph properties. It also cannot be designed without significant innovations(\cref{sec.engg}).

%We demonstrate the usefulness of {\graphpy} with the implementation and evaluation (\cref{sec.exp}) of many GNN models. 
%on an average 1.64$\times$ and 1.42$\times$ speedup and 1.30$\times$ and 2.29$\times$ speedup over DGL, and PyTorch Geometric for various GNN models in GPU and CPU respectively. 
%Further, frequent out-of-memory conditions by DGL, Pytorch-Geometric, and GNNAdvisor force measurements to be performed on smaller dataset only. Measurements on smaller prevalent dataset do not show advantage of kernel optimization due to framework overhead.

Our evaluations (\cref{sec.exp}) show that {\graphpy} reduces memory consumption on average by 6.92$\times$ on GCN, 3.4$\times$ on GIN, and 1.96$\times$ on GAT-1 models in comparison to DGL, while DGL, Pytorch-Geometric~\cite{pytorchg2019} (PyG) have many out-of-memory conditions. 
Further, {\graphpy} achieves on average 1.38$\times$ 1.51$\times$, 1.58$\times$, 1.32$\times$ speedup for GCN, GIN, GAT-1, and GAT-3 compared to DGL on larger datasets. 
We also show that GNN-specific kernel definition alone without any workload balancing technique can perform much better (1.16$\times$ -- 2.95$\times$) than optimized and workload-balanced generic kernels of FeatGraph~\cite{featgraphsc20}, GE-SpMM~\cite{gespmmsc2020}, GNNAdvisor~\cite{wang2021gnnadvisor}, and Huang et al~\cite{huang2021understanding}, which can not be run end-to-end along with CuSparse and DGL.
Lastly, focus on interface design minimizes the framework overhead of {\graphpy} by 1.54$\times$, and 1.35$\times$ than DGL and PyG.
%to achieve better performance on smaller datasets. 

%To show the extensibility of {\graphpy}, we also demonstrate the implementation of sparse tensors (not sparse data) on LeNet-300-100.

%Therefore, future systems optimizations can benchmark their performance against our baseline to advance the state-of-the-art rather than comparing against various overheads.

%Empirical evaluations show that our optimized implementation achieves 1.62$\times$ and 1.35$\times$ over DGL and PyTorch for various GNN models on many datasets in GPU, and 1.55$\times$ and 1.88$\times$ on CPU respectively with similar accuracy readings.\td[end]
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research. 
%A better GNN performance using the reference implementation, less framework overhead, and low memory consumption make {\graphpy} an ideal baseline for performance benchmarking for future research. 


% The remainder of the paper is organized as follows. We present background on graphs and DL in \cref{sec.background}. 
% %The motivation, challenges, and overview of {\graphpy} are presented in \cref{sec.overview}. 
% The detailed use cases are presented in \cref{sec.after_observation}, technical challenges and prior works in \cref{sec.challenges}.  Implementation details are presented in \cref{sec.science} and \cref{sec.engg}, evaluations in \cref{sec.exp}, and we finally conclude in \cref{sec.conclusion}.


The paper specifies many practical issues with GNN systems and provides a practical yet powerful framework to overcome those issues. 
More importantly, the proposed baseline allows {\graphpy} to train GCN on a billion-edge graph on a single GPU due to memory saving while prior works cannot train even a 500 million-edge graph. 
The new baseline also offers  newer opportunities for practical optimizations. 
%where {\graphpy} offers researchers a powerful mechanism to design end-to-end systems productively. 
Indeed, there is an immediate scope for optimizing the proposed GNN-specific kernels through various format-specific and workload-balanced designs that can be compared against the proposed baseline to show the practical impact.
Lastly, the proposed tool and mechanisms may be used for end-to-end system education to train learners on system requirement gathering for GNN/DL models and implementation, which has been flagged as a major concern in an NSF workshop~\cite{storage2025NSF}. 


==> tex/new_added.tex <==
\section{New added sections} \label{sec.new}
\subsection{Research aspect}
Many existing works, [GNNadvisor, zhai, gespmm, ] mainly focus on optimizing the kernel implementation. (TODO GNNadvisor has a python model, zhai has a simulated GNN). However, based on our analysis, we are the first one to find that kernel implementation alone is not sufficient enough for system research to avoid mistakes and improve end-to-end DL training time.
The following sections will provide more details to support our findings. 
 
\subsubsection{End-to-end training is needed in GNN systems}


\textbf{Without end-to-end training, many implementation requirements are ignored by the researchers}
 
 
Different classes of GNN(GAT, GCN and GIN)
The GNN models can be classified into different classes based on their aggregation method. The GNN models which have unweighted sum aggregation are one class, such as GCN and GIN. The GNN models with the weighted sum aggregation method is another class, such as GAT, etc(todo we can cite more attention-based paper) Because of the aggregation difference, different types of GNN models have different system-level implementation requirements.  



Edge id indirection is needed, (Copy from 2d-snb)
As we mentioned in the background, Attention-based GNN models use attention(importance) scores to aggregate the neighbor values. Attention-based GNN models first generate the O(E) level attention score A. In the aggregation process, 

 Given a target node i, the model first fetches the attention score $A_{k}$ of its neighbors ($k \in N(v)$), then aggregate by sum$(A_{k} * H_{k})$ to updated the $H_{i}$. This process will be iterated until all nodes’ embedding is updated. This updated H will be used for the later computation. 

In the forward process, the kernel fetches the A by the normal graph order and performs the later computation, and saved it for the backward computation. 
In the backward process, the kernel needs to reload the saved A and fetch it again but in the reverser graph order. 
Here the problem comes, Since the graph is now reversed, the order of the edge list now is different than its order in the normal graph. If we still use the forward fetching order to fetch the A in the backward process, each attention score $W_{k}$ will be wrong. The incorrect fetched $W_{k}$ will cause a wrong backward computation, which corrupts the whole model training process.
While this  problem can also apply to compressed layers. E.g., in weight-pruned fully connected layers, as shown in Fig.~\ref{fig-prun}, the data is the dense matrix and the layers are sparse matrices.
To solve this problem, it is mandatory to maintain the edge indirection property so that  the kernel can fetch the correct $W_{k}$ in both the forward process and the backward process.

Zhai -- GAT problem
(copy from 2d-snb ended)
 
The corresponding DGL kernel of this computation is ‘gspmm’. To support this requirement, DGL provides an extra shuffle kernel to reorder the edge id list each time before fetching the edge score tensor. After that, DGL transposes the input tensor and uses the cusparse library to perform the computation. This extra shuffle kernel, transpose computation, and the system overhead time between them lead to extra time cost at the end-to-end training process. (todo find the line of code with shuffle + gspmm) 
If the requirement(above process) is not fully understood by researchers, even if they replaced the cusparse library with an optimized kernel, the overall end-to-end training process will not be optimized. 
Hardly do these previous papers discuss this edge id indirection requirement. Instead, Their kernel implementation can only support specific types of gspmm, such as GCN and GIN. 
 

Zhai’s work does not consider this requirement when implementing the kernel also. It fetches the edge tensor in sequence, this incorrect fetching will lead to the wrong aggregation result.
Although the integration between the kernel and the GNN model is correct, the overall simulated GNN has Some mistakes. (todo Not sure what this problem is: Input tensor and output send them as the same tensor)
Because of these mistakes, even if the simulated end-to-end training time shows improvement, this result is not trusted and cannot represent real-world GAT training. 
Gespmm forgets to consider edge id indirection also.

Therefore, if the researchers only focus on kernel implementation, it is likely for them to ignore some requirements and make some mistakes.
With an End-end training platform, it becomes easy to let researchers know that some extra requirements, such as edge id indirection property, needed to be taken care. With understanding this requirement, researchers are free to follow the DGL solution or propose their own solution. 


\textbf{Implement kernel only can cause end-end training accuracy problem}

Firstly, without end-to-end training, the kernel implementation may be incorrect.
One straightforward example is forgetting to meet some extra requirements we mentioned above(in the above section)
Secondly, even if the kernel implementation is correct, the overall training loop may be still wrong. For example, GNNadvisor implements it’s gspmm kernel alone correctly. But its experiment shows in (todo section ) show that it does not achieve correct accuracy. That is because it does not fuse the normalization computation with the gspmm kernel correctly for the backward process. In the backward process,  the fused kernel should do normalization first and then perform the aggregation.
(\todo zhai problem and gat)




To sum up, existing GNN system level optimization works, GNNadvisors, zhai, gespmm read the DGL code base to understand the requirement. ( need some reference email them) 
However, GNN model works, such as GCN, and GAT(these papers just provides the basic mechanism of the dense matrix) and GNN System works, such as DGL do not provide clear system-level requirement description. It is not guaranteed that all people can understand them correctly. Examples in the above section (todo list GNNadvisor, zhai, gespmm citation here) show that even researchers may ignore some requirements easily. 
 
Therefore, these requirements are very important in GNN systems but none of the Previous works explain them in the paper.  We are the first one to explain these requirements and illustrate their importance. We also state that with an end-to-end training platform to test the accuracy, these ignored requirements will be found. 

\subsubsection{A baseline is needed in GNN system area}


\textbf{End-to-end training time is controlled by overhead}

Our experiment in section (todo) shows that existing GNN systems, DGL, PyG have large overhead for the small data sets. To be more specific, the end-to-end training time is controlled by system overhead.
This large overhead has two negative effects. Firstly, since the work that implements most computation in cuda and c++ can avoid the system overhead and achieve huge end-to-end improvement, it is hard to measure the real effectiveness of performance improvement for these types of works. We do not know whether the improvement comes from the c++, cuda implementation, or the optimization techniques mentioned in these works(such as graph reordering, techniques to improve data locality, and better parallelism).

Secondly, the large overhead misleads the potential optimization directions for researchers.
That is because most researchers verify the effectiveness of their optimization techniques by performing an end-to-end training on small datasets.
In that case, the end-to-end training time will not change even if the kernel is optimized well, 
To solve this problem, GraphPy was optimized to achieve a small overhead so that the Kernel improvement can play more role in the end-to-end training. 

\textbf{Overhead neutralize the effectiveness of kernel improvement}
Besides the overhead on small datasets, framework overhead prohibits the improvement of the overall end-to-end training even if the kernel itself is well optimized. 
 
A straightforward example is DGL. DGL adopts the cusparse, an accelerated linear library optimized and provided by Nvidia over decades, as the core kernel for gspmm(mainly kernel used in GCN and GAT).
However, DGL’s gspmm kernel cannot achieve the same speed as cusparse. Instead, it has a 2 X, 3X slowdown compared with cusparse. (todo Test cuspare, and gspmm kernel in DGL to show the performace different in ogb dataset) 
That is because the gspmm in DGL is designed for both unweighted aggregation and weighted aggregation. It needs to apply one shuffle kernel each time before launching the cusparse to support edge id indirection(refer to next section). Moreover, since cusparse library can only accept column-level input, DGL needs to transpose the input tensor before using the cusparse library. These two more steps, shuffle, and transpose, cost some extra time. If the researchers just fuse these two steps together or remove the need for transpose for cusparese library and do not apply any optimization techniques, the end-to-end training time will improve a lot. 
 
But if the researchers do not understand these steps correctly, and design some optimized kernel to just replace the cusparse. Even if the optimized kernel is faster than cusparse, the end-to-end training time will not be improved. (todo not sure whether this DGL example is overhead or not)
 


(Todo Another example is the Gespmm, although its optimized kernel is faster than cusparse, after it integrated its kernel to DGL the overall training time does not have significant improvement. )



 
Our Experiment in section (todo), Figure (todo) also shows that even if our reference kernel gspmm is slower than cuspares, our GCN end-to-end training time achieves a (TODO) speedup compared to DGL among different datasets. 


(todo not sure Because of edge id indirection provided by our framework). Even if our kernel is slow alone, Our end to end training time still achieves huge speed up.
 
Therefore, Just focusing on the kernel implementation cannot lead to a good end-to-end performance. Moreover, since researchers study the kernels for more than 10 years, the new optimization mostly triggers an incremental improvement such as 10 percent - 15percent. From the above, we find that the end-to-end training time bottleneck comes from not only the kernel but also other parts.
 
Researchers need to understand not only just the kernel(The kernel here is different than the kernel in DGL, but not sure how to explain the difference) but also the other parts. This understanding can only be achieved by end-to-end testing. 

In that way, there is a need for an easily plugged-in platform to let researchers understand the roles of the kernels in the whole GNN training process. With a better understanding of the kernel role, researchers can implement the proper kernel which speeds up the overall training performance. 


\textbf{huge memory consumption causes problems}
As we know, DL needs to consume huge memory which will lead to a high energy cost. (citation to do takes 1-week energy of the whole city) Therefore, memory consumption becomes an important metric for DL systems. In this work, GraphPy provides a low memory consumption. It saves the number of E memory, which leads to 4 bits in GAT 1, and 12 bits in GAT3. For a graph with one billion edges, GraphPy saves 4 GB of memory. Moreover,  GraphPy can Save a number of vertex memory in features tensor compared to DG.L(todo add some details in interfaced design to explain).  In total, GraphPy can minimize 50% to 100 % memory consumption saving compared to DGL, which is a huge saving for energy costs. 
 
Another problem high memory consumption causes is graph splitting. For a large graph, the dataset cannot fit in a single GPU. Researchers need to split the large graph into multiple subgraphs and send them to multiple GPUs to do parallel training (todo citations). This multiple GPU setting makes the problem become more complex, and many concerns needed to be worried, such as how to synchronize the results, how to minimize the overhead, and how to optimize the communication between each split subgraph(Graph Partition is an NP-hard problem).
 
However, GraphPy provides low memory consumption to enable researchers to run GAT models on large datasets with a single GPU setting and avoid the complex multiple GPU problem settings. 


\textbf{Other problems with existing works}
Besides the overhead problem, there are other reasons that make the existing works cannot be used as a baseline.
As we mentioned in the above section, GNNadvisor has an accuracy problem in end-to-end training. It does not consider the edge id indirection at all so that it can only support a specific type of GNN model, such as GCN, GIN. It cannot work on another class of GNN, such as GAT.
Although zhai’s work supports GAT kernel, its kernel implementation is wrong because of the missing edge Id indirection. Moreover, Zhai’s work does not contain the end-to-end training loop. It is also impossible for researchers to implement a training loop by themselves because zhai’s work does not provide a backward process. 
Gespmm does not support edge indirection property either, which means that it cannot support GAT. 
PyG meets the OOM problem even for the median size data set. It also has a Large overhead for small datasets.
Therefore, none of the existing works can be treated as the baseline. 
There is a need for a Baseline in GNN systems, which is better than DGL in end-to-end training but does not include any novel opt techniques so that new optimization techniques can be added.

\textbf{Summary}
 
To sum up, wring the kernel alone is not enough. There is a need to provide a platform to let researchers really understand the kernel requirements and related topics.
 
To fix this gap, GraphPy focuses on interface design. By providing modular-based kernel, GraphPy
provides the opportunities and options system researchers can pursue which is not explored by the early framework.
 
To be more specific, the Kernel interface in GraphPy is not as simple as DGL expects. In the DGL, the core kernel for ‘gspmm’ is the cusparse kernel. To integrate with DGL, researchers can only implement new kernels to replace the cusparse. As we mentioned above, replacing cusparse cannot achieve end-to-end performance improvement.
However, GraphPy provides a more customized kernel interface so that researchers can decide whether they want to implement a new kernel that replaces all the above computations or just replace the cusparse. The optimized small overhead of GraphPy provides researchers the opportunity to check the effectiveness of the kernel in the end-to-end overall training.
(todo need to explain this part well. What is the difference between graphpy kernel and the DGL kernel? Not very precise What impact the overhead places here)


(todo Hardware evaluation. Or just kernel evaluation. (Possible for overhead analysis))



\subsection{Education aspect}
For education purposes, there are several educational attributes GraphPy provides.

\textbf{Just writing kernels in c++ or python is not enough}

The real-world GNN system[AWS, Azure, etc todo need citation] contains two aspects: c++/cuda based kernel implementation to provide fast speed computation and python-based wrapped kernel and GNN layers to let the data scientist customize their GNN models. 
 
 
 
 
 
 
The goal of the teaching is to let students understand both these two aspects.
 
Only teaching how to implement the kernel in c++/python is not enough. It is not just teaching students how to write the kernel and how to use pybind to wrap the kernel out in python.
Writing the kernel only cannot let students understand the exact requirement as we mentioned in the above research section. (todo cite the section number here) 
For example, GNNadvisor does not fuse the normalization and the computation kernel correctly in the backward process. But it is hard to explain this requirement to students on the kernel implementation. Only with an end-to-end system teaching, students will know this difficulty of kernel fusion. To be more specific, if we assign an assignment to let students fuse these kernels directly, students just implement the fused kernel without thinking of any requirement about this fusion process. 
But with an end-to-end system, the instructor can teach students these requirements and let them play with different kernel fusions and understand whether the requirement is satisfied or not from the accuracy. 
 
The existing platform does not provide an end-to-end system. They standford, berkely[need some citations] just provides pooling, softmax, batch normalization (not sure of convolutional layer) in the forward. Students still do not know how the backward process doing and how to use the wrapped kernel in an end-to-end training loop. 
 
It is hard for students to have a whole-picture view of how the GNN system works. With Graphpy, students can practice these steps and learn some practical tricky implementation techniques. And understand how each step works in an end-to-end training process.  This education training will help the students get a deep understanding of GNN systems, which will help them a lot in the future job market or academic research. 
 
Besides this, GraphPy also provides several educational attributes so that students can learn the GNN system easily.


\textbf{Easily plugged in kernel module}

In the GNN systems education teaching, there is a need to let the student write the kernel. However, this implementation process should be kernel focused only. That is because most students do not have enough background and time to explore the integration code and pybind wrapping technique.
GraphPy focuses on the interface design to provide the independent kernel module and auto-generated integration code to let students write the kernel easily and not need to learn the programming framework.


\textbf{Customized Python GNN layers}
Besides the kernel implementation, GraphPy wrappers the GAS kernel out in the python environment and provide the GNN model layers.
Students can modify them easily to learn the GNN models’ configurations and how the GNN model uses the GAS kernel.


\subsection{Graph system works cannot be extended to GNN}
Merril’s work handled the workload imbalance, which lead to a great performance improvement in spmv. However, it needs to preprocess the metadata first and use this metadata to do later things. These metadata structures cannot be passed to DL backends such as TF and Pytorch. (To do how to provide it cannot ). Many other works [citations] also rely on the preprocessed additional data structure.
 


\subsection{GraphPy can also work on unlabeled datasets}

For the unlabeled dataset, GraphPy can randomly generate the label for the training node id and test node id. With this synthetic label, these unlabeled datasets can be viewed as labeled dataset. 



==> tex/observation.tex <==
%\subsection{Memory Usage \& Evaluation Pitfalls} \label{sec.mem}

\subsection{{EVAL-P3}: Framework Memory Overhead} \label{sec.mem}

% \noindent \textbf{Memory Consumption and Scant or Inconclusive Evaluation on Mid-Size Datasets (Mem-P1).}
%DGL and PyG have already addressed the system design pitfalls (\cref{sec.semantic}) even before they appeared in other works, as they were proposed several years ago. However, 
Several papers have shown frequent OOM on slightly older GPUs for mid-size datasets on PyG and DGL, which is aligned with our measurement. 
However, the excessive memory consumption has forced prior GNN systems to heavily or even exclusively rely on smaller datasets for comparing training runtime leading to EVAL-P1 (\cref{sec.overhead}). While we already discussed the reason behind OOM for PyG in \cref{sec.spmmt}; the framework (DGL) design causes huge memory consumption and not GNN implementation in DGL.

%two critical pitfalls which unlike other pitfalls are not related to correctness but are more about \textit{system design and integration efficiency}. We then show that how these pitfalls have impacted almost every GNN system.

%in evaluating training runtime comparison, as discussed in \cref{sec.evaluation}. 
%Unfortunately, \textit{framework overhead determines the training time on smaller datasets and not the kernel performance, 

%where training runtime comparison on mid-size datasets is scant or inconclusive due to frequent OOM by DGL and PyG, the baselines.



\noindent \textbf{Methodology.}
DGL consumes close to 23.2 GB of memory (Fig.~\ref{exp-mem}) while training the Reddit dataset on GCN, one of the simplest GNN models.
Our initial suspect was that DGL consumes more memory due to storage cost (\cref{sec.spmmt}), and due to their other inefficient design in GCN: \textit{a)} Cusparse provides only SpMMve API which is not suited directly as {GCN} needs SpMMv API. Hence, DGL uses a \textit{dummy edge-level tensor} with each value as 1.0 to use Cusparse API, consuming an additional $|E|$ memory. 
%A few GCN systems~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} are still focused on optimizing SpMMve despite the focus on GCN. 
%Moreover, DGL unifies the storage format for all GNN, therefore it still keeps separate copies of CSR, CSC, and the edge ID array.
\textit{b)} DGL does \textit{degree-norm} out-of-place. This not only allocates $|V|*|K|$ sized additional memory(K is feature-length) but the division also becomes a node in the computation graph of GNN. Therefore, gradients are also generated and materialized between SpMM and degree-norm kernel.
\textit{c)} DGL processes the degree array before each call to degree-norm due to the presence of empty rows in the sparse matrix. In this case, DGL calls (\textit{clamp}()) API which sets the degree to 1.0 for empty rows for each iteration, introducing further slowdown and additional $|V|$ sized memory.


%is also due to its framework memory overhead, which does not originate from kernel operations or graph storage. For instance, 
However, our direct evaluation of DGL's SpMMv kernel (used by GCN) on Reddit ($|K|$=32) shows a whopping 12,982 MB of memory consumed (on top of graph storage).
Our back-of-envelope calculation shows not more than 936 MB for two vertex-level tensors of size $|V|\times|K|$, and one edge tensor of size $|E|$ which are used in SpMM. The scratchpad memory consumed by Cuspasre SpMM is very small. Indeed, our direct evaluation of Cusparse SpMM shows only around 936 MB of additional memory consumption.

\textit{Thus, we note that DGL introduces a framework memory overhead of around 12,046 MB memory in this case as the memory requirement of known sources cannot account for it.}
We also measured in an older version of DGL which still introduced a memory overhead of 6,340 MB memory, thus confirming that it is not a version-specific problem. %7,276MB 

Our analysis points to DGL's complex system-building approach. At the Python level, it uses a DLPack tensor that converts tensors to a framework neural data structure, and hence its back-end cannot use any PyTorch-specific API. However, its system module brings PyTorch through non-standard integration for its internal memory allocation, which is needed for Cusparse SpMM’s scratchpad buffer allocation. 
We suspect this non-standard integration of PyTorch to be a reason for the memory overhead, as its SDDMM, which does not do any internal allocation, did not show memory overhead.

%\td \red{add dgNN memory leak}

% they say they have 5 times speed up. But when we integrated them use the Cusparse. we find the memory saving is only 30. Or our reference system shows that is only 16.Huge memory consumption also leads to system design to solve memory pitfalls. But it proposed design is not solving the memory saving because the baseline is bad. GraphPy here if we have.


\subsection{Discussion: Hypothesis and Impact}

\noindent \textbf{Hypothesis:}
Understanding DL frameworks presents newer challenges, specifically in the era of heterogeneous hardware, e.g., CPU and GPU. Indeed, the DL framework is  more like an Operating System whose job is to allow access to hardware without introducing much overhead. The Python and CPU code in DL becomes the equivalent of system call implementation (overhead), while the GPU kernel time is equivalent to device/hardware response time. 
To this end, we hypothesize that prior works think DL models from kernel perspective, hence they miss the overheads associated with the framework. 

% %Framework overhead is presented first time by us, and hence prior works were not aware of its impact. However, beyond that, another fundamental matter about system design is lacking in us.
% For EVAL-P2, we believe \red{OOM condition by DGL and PyG} did not allow conclusive comparison on mid-size labeled datasets, thereby many prior works rely on smaller datasets. 
% % The framework overhead pitfall makes the evaluation unreliable. 
% Further, earlier versions of GPUs had less memory on which prior works had to rely leading to OOM by baselines. 
% Moreover, access to limited choices of labeled datasets and no significant precedent of using synthetic datasets forced us to rely excessively on smaller datasets, thereby leading to a possible compromise on system evaluation. 

%natively written SpMMv gains automatic memory saving and speedup compared to DGL. 

%Though it is possible to conduct such an experiment, which we do in \cref{sec.exp}.
%We now discuss the impact and present a fundamental insight into the pitfalls, hypothesis, and recommendation.


%In this subsection, we discuss two important points on whether the new insight from the framework overhead perspective affects the fundamental understanding of the system. 
%Like the previous pitfalls, a straightforward question can be posed on whether these evaluation pitfalls led to a fundamental problem or an evaluation oversight. 

%However, as we mentioned earlier, framework overhead was not known to the community so it is not a case of evaluation oversight. 


%We should not remain trapped in such errors in the future which compromises the optimization process.

\noindent
\textbf{Impact: Generality.}
DGL and PyG being two widely used systems as baseline and even for system integration~\cite{gespmmsc2020,featgraphsc20,wu2021seastar,p3gandhi2021} have impacted almost every GNN systems. These pitfalls %But as we discussed, framework overhead (EVAL-P2) and memory consumption both 
have questioned our understanding of the role of framework in GNN system design and evaluation where runtime and memory consumption are the two most important metrics.

%\textbf{Generality and Fundamental Flaw in Evaluation.}
%\blue{This is an important question because an academic prototype does not go through the rigorous evaluation as a commercially developed code. However,} 
Presence of \textit{framework-runtime overhead} highlights the fundamental flaws in evaluation process that the community lacks. Indeed, the whole class of sampling-based GNN system are affected. 
We show that many current systems have performance regression when evaluated on mid-size datasets (\cref{sec.exp.kernel}). 
We also suspect that other DL systems may be impacted requiring more evaluations to confirm the observation. 
%It also has huge repercussions for future systems research as outlined in \cref{sec.analyze} (first bullet).

The presence of \textit{framework-memory overhead} in DGL has affected all systems whether integrated with DGL or not. While the former is likely to have same memory overhead, the latter have shown inflated memory saving due to simply not integrating their work to DGL.
For instance, our measurement on a memory-saving GNN system, dgNN~\cite{zhang2022understanding} %claimed less than $3.5\times$ memory consumption 
for Reddit dataset show 3.22$\times$ less memory consumption than DGL, similar to what dgNN paper claims. However, whether all the memory saving is due to their techniques remains an open question (\cref{sec.exp}).
Indeed, it has deprived the community of baseline information about memory consumption in GNN systems, and impedes comparisons with prior works on GPUs with smaller memory capacities due to frequent OOM.
\textit{Thus due to out-sized impact of the baseline, the pitfalls have created critical impact to the community. }

%\blue{Further, popular baselines affect research in other ways, e.g., a few GCN systems~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} are still focused on optimizing SpMMve despite their focus on GCN. Thereby they need a \textit{dummy edge-level tensor} with each value as 1.0 to use these APIs, consuming an additional $|E|$ memory like DGL.}


%Our measurement shows that dgNN achieves only 30\% memory savings compared to the proposed reference system {\graphpy} (\cref{sec.baseline}) for Reddit dataset (\cref{sec.exp}).
%Our measurement shows that dgNN achieves only 16\% memory savings compared to the proposed reference system {\graphpy} .}


%\textit{a)} Cusparse provides only SpMMve API which is not suited directly as {GCN} needs SpMMv API. Hence, DGL uses a \textit{dummy edge-level tensor} with each value as 1.0 to use Cusparse API, consuming an additional $|E|$ memory. 



%\blue{Hence, we cannot term these pitfalls as evaluation oversight.} 
%Kindly note that our discovery of framework overhead exposed the issue, otherwise, there was no question of inadequate benchmarking practice. To this end, a fundamental gap in the evaluation process has been shown, thanks to framework overhead discovery, which becomes severe due to the scant and inconclusive evaluation of mid-size datasets, sampling, and training accuracy issues that are prevalent. 


% \noindent
% \textbf{Impact: Applicability of Optimization Techniques.}
% Pitfalls do impact performance, contradicting the published results thereby questioning the applicability of some of the optimization techniques proposed earlier (\cref{sec.exp.kernel}). For example, we show that the proposed reference system ({\graphpy}) has slower end-to-end training time than a pitfall-manifested system on smaller datasets despite having better runtime for underlying kernels. Such results are unlikely to impress authors themselves and reviewers in a conference or journal unless pitfalls are known.
% %It should be noted that many optimizations are due to better insights into the fundamental trade-offs. Hence, when they are not evaluated on mid-size datasets, the result could be misleading, at least the speedup attained. 


% \noindent 
% \blue{\textbf{Impact: Broken GNN Workflow.} 
% The study suggests that we have masked the true comparison of underlying optimization techniques while measuring training time as evaluation on smaller datasets can not be relied upon due to framework overhead. Indeed, we along with others~\cite{fu2022tlpgnn} have noticed that GNNAdvisor cannot be executed for mid-size datasets at all for GCN, showing the broken GNN workflow.
% Further, scant or inconclusive results on mid-size datasets coupled with accuracy issues together question the whole GNN workflow: the benchmarking practices, the drawn conclusions, and lessons learned in many prior works.}

% In systems, many optimizations are due to better insights into the fundamental trade-offs. Hence, when they are not evaluated on mid-size datasets, the result could be misleading, at least the speedup attained. We indeed show that a few papers with kernel optimization goal are slower than Cusparse in mid-size datasets (\cref{sec.exp.kernel}) due to focus on smaller datasets.
 
% In the absence of inadequate performance benchmarks, one cannot conclude whether the proposed optimization is applicable.  
%But the absence of truly peer comparison such as OOM by DGL and PyG in those papers does not allow us to conclude whether those systems are faster or not. 
%Many systems exclusively rely on smaller datasets,  we do not know if it is really faster than others or not, as we explained earlier. Rather, as we measured a couple of them manually, they are slower than DGL, though we used the latest version of DGL. Other systems majorly rely on smaller datasets with just one or two mid-level datasets. 
%Hence, it questions the advancement of the state-of-the-art and lessons learned.

% GNNAdvisor relies exclusively on smaller datasets. However, when we tried to run it on mid-size datasets of Reddit and Ogb-product, the program crashed due to an invalid memory access error, which has also been observed by prior works~\cite{fu2022tlpgnn}.   
% FuseGNN~\cite{chen2020fusegnn} which is not integrated into DGL, performs better than DGL for smaller datasets. However, its result on Reddit (the only large dataset) shows that it remains inferior to DGL. Our measurements confirm that its overhead is smaller than DGL for smaller datasets. Hence, the lower overhead due to the new system is responsible for the better performance of FuseGNN. But once overhead is not a factor for mid-size datasets like Reddit, FuseGNN performs slower than DGL.



% However, looking at the impact of the evaluation pitfall, one can definitely claim that the pitfall has exposed a fundamental limitation in the evaluation methodology as end-to-end evaluation on the smaller dataset is not sufficient to claim a system is faster due to the proposed kernel optimization, while the scant coverage on mid-size datasets does not provide a decisive verdict. Coupled with the wrong accuracy with many prior works, a fundamental gap in evaluation has definitely emerged.   

%If memory consumption or out-of-memory is not allowing us to measure effectiveness on mid-size datasets, we need to come up with a different set of evaluation methodologies. We discuss them in the recommendation.

%However, the community agrees that the purpose of the evaluation is to understand the trade-offs in the system design, and an optimization technique that argues for better performance but performs slower in evaluation is unlikely to be useful.   [\td may cite the system paper writing paper]. 
%We explain this point in detail after we pose one more question next.


% When almost all the prior works use the smaller datasets exclusively or partially, it impacts our understanding of the proposed techniques. \textit{Firstly,} if a work exclusively used smaller datasets only, we are not sure if their proposed optimization techniques are actually better or not compared to the prior work at that time. Indeed we will show that at least one GNN system performs slower compared to the baseline against which it claimed to perform better on larger datasets, which it did not evaluate [\td].
% \textit{Secondly,} a few works reported speedup when evaluating smaller datasets, but reports slowdown on larger dataset(s). This directly proves that their optimization techniques are not at all useful as the optimization on smaller datasets is due to lower framework overhead. 
% \textit{Thirdly,} as the evaluation on smaller datasets does not tell whether the proposed optimization works or not,  then the rest of the evaluation becomes very selective as it may only be picking very few additional datasets, such as 1 or 2, and hence the evaluation strategy can not be called a representative. 



%\subsubsection{Hypothesis and Recommendations}
%We first discuss the hypothesis, followed by our recommendation.


%As we discussed earlier, the complex relationship among pitfalls has led to more pitfalls, but all point to the same root cause: we have not understood the GNN completely yet.

%The GNN system design is a complex process due to the involvement of backward computation. However, once the required kernel functionality is identified, it needs to look for those APIs if using vendor libraries before deciding to rely on additional design. While many works could not identify the required kernel, specifically those that suffer from SYS-P2, DGL decided to solve it despite Cusparse offering such native API, which ultimately led to huge memory consumption and slowdown (\cref{sec.mem}).
%that goes beyond the development and usage of sparse kernels. It is this complex relationship that DGL has solved using memory-intensive solutions, which we analyze in-depth in \cref{sec.mem}, to take care of the design pitfalls. 



% which indirectly influenced the inconclusive training runtime comparison in later works because DGL is frequently shown out-of-memory.
%Hence, a broken system evaluation, specifically the absence of training accuracy measurement, has masked those higher-level issues of the system design. So. when baseline systems, specifically DGL, show OOM and not our own system, we never look at the proposed systems with a critical eye. 

%And even when the prior works did measure the accuracy of their system, they never were aware of the framework overhead, which we presented the first time.


% on those earlier GPUs. Unfortunately, DGL consumes memory in access of 20GB for GCN, while GAT requires even more memory for the Reddit dataset, a popular mid-size dataset as listed in Table~\ref{table-obs-memory}.
% On the other hand, PyG always runs out of memory on A100, which has 40GB of memory. 






% \begin{table}[h]
% \small
% %\vspace{-6pt}
% \caption{\small Memory Consumption (in MB) when running GNN training on DGL. PyG always runs out of memory (Lower is better).} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r|r |r|r|r|r|} 
%     \hline\hline 
%     %heading
%   %  \cline{2-7}
%     Graph Dataset & GCN & GIN & GAT-1 & GAT-3 \\
%     \hline % inserts single horizontal line
% %    Cora & 1,719 & 1,349   & 1,719 &1,375 &&\\ 
% %    PubMed & 1,767 & 1,395  &1809& 1,503 && \\
% %    Citeseer& 1,697&1,381   & 1,759 &1,409 &&\\ 
%     Reddit & 23,237& 23,737 & 30,395 & OOM  \\
%     OGB-Product & 15,137 & 19,203 &20,789& 32,285 \\
%     %OGB-Pr & 25,551 &OOM & 20,789 & OOM  &32,285& OOM\\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% %\vspace{-6pt}
% \label{table-obs-memory}
% \end{table}

% Hence even if earlier works may have performed better than DGL on mid-size datasets, they could not verify it. So, a few work when reports result on DGL and PyG, they almost always show them out-of-memory.



%Interestingly, despite the OOM issues in DGL and PyG, no prior GNN works exclusively focused on analyzing memory consumption in prior works and focused on optimizing it. dgNN is possibly the only system that optimized memory consumption though it has accuracy issues, and focused on class A GNN only. It saved memory through recomputation so that it can avoid materializing some state tensors. However, we still do not know why DGL has high memory consumption in class B GNN.   


%result may have discouraged many prior works on exploring evaluations on these datasets.



\section{Future Direction and A Reference System} \label{sec.analyze}
% In the presence of the pitfalls, two questions remain on how to make forward progress:
% 1) whether the community should start from scratch; and 2) and how to make sure that the community makes genuine advances. 
% The latter concern is because DGL, the identified state-of-the-art in this paper, has introduced a big gap (fundamental and system introduced) between it and Cusparse APIs, for which DGL follows many costly workarounds. Hence any spurious optimization may outperform DGL easily if they can avoid those workarounds.

% To this end, we build {\graphpy} from scratch by focusing on identifying and building GNN primitives so that no workarounds are needed. 

% After identifying the pitfalls, the natural progression leads us to the question of how to address and overcome these pitfalls. 
% Otherwise, we suspect that if the current solutions are integrated into existing systems with design pitfalls, they may also run out of memory. 
% The current solutions require in-depth analysis to find out whether it has fundamental limitations or whether a new solution could be found through novel optimization.

% In response, we introduce {\graphpy}, a novel GNN system designed not only to overcome these pitfalls but show that solving pitfalls offers a new category of optimization opportunities that are complementary to the existing sparse kernel optimization approach. 
% %targeted at improving data locality.  but also to incorporate various other innovative designs. Additionally, GraphPy explores and discussed several new optimization aspects for GNNs, a previously unexplored territory. 
% Our pioneering work in this area reveals that these new aspects complement existing GNN optimizations, as demonstrated by our experimental results. Past and future GNN systems can benefit by adapting them in order to make the GNN systems perform training correctly and efficiently amid reduced memory consumption. 



%its \textit{runtime performance} and \textit{memory consumption} of DGL. Though it may seem a very specific discussion, we show that it does capture a generic observation regarding system design that is equally applicable to many other works even if they have requirement misunderstanding or evaluation issues. Based on those analyses, we simultaneously explain the novel design idea of {\graphpy}, which is rooted in an in-depth understanding of the requirements, and system characteristics.


% {\graphpy} exploits symmetry in GNN datasets using a novel edge ID reordering for transpose SpMM, allows both the workload balancing and data reuse in SDDMM, and exploits special kernel requirements for GCN.

Pitfalls presented in \cref{sec.accuracy} and \cref{sec.evaluation} have renewed our understanding of system design and implementation for GNN models and the role of the framework respectively. Thus, this paper questioned every aspect of GNN workflow-- design and implementation, integration, benchmarking practices, drawn conclusions, and lessons learned-- in many prior works.
Hence, the natural progression is overcoming these pitfalls collaboratively. So we present useful recommendations and future research direction in \cref{sec.direction}, and a reference system in \cref{sec.baseline}.

 
\subsection{Recommendations and Future Direction} \label{sec.direction}

\noindent \textbf{Accuracy Related.}
\textit{Measuring training accuracy} is the most important feedback to the correctness, and hence should be enforced ({Recommendation \#1}).

The systems with no backward implementation or with accuracy issues risked being sidelined for evaluations by future works. 
Some pitfalls in them can only be addressed via invasive efforts, e.g., by developing backward computation code, fixing the order in backward computations, including bias and other mistakenly removed operations to model layers, etc.
We believe that a systematic approach by developing a standardized system benchmarking tool may allow us to plug-and-play their kernel for fair and end-to-end benchmarking. Such work remains a work in progress.
Till then, we believe that \textit{directly evaluating their kernel running time} ({Recommendation \#2}) can make sure that we do not discard their advances in basic kernel design, like SpMM and SDDMM. This is impossible if prior works have only fused kernels with pitfalls.

% \noindent 
% \blue{\textbf{Recommendation \#2.}
% For the systems with no backward implementation or with accuracy issues, we believe that directly evaluating their kernel can be another methodology to make sure that we do not discard their advances in basic kernel design, like SpMM and SDDMM. This may not be possible if prior works have only fused kernels with pitfalls, and hence they risked being sidelined for evaluations by future works. }
% %As part of this work, we have developed scripts including modifying their back-ends to allow evaluation of basic kernels, such as SpMM and SDDMM, if present in prior works.



\noindent \textbf{Performance Runtime Related.}
Smaller datasets alone cannot be used to conclude better runtime due to the framework overhead. 
To negate it, end-to-end performance measurements should \textit{evaluate on mid-size datasets} (Recommendation \#3). Once system accuracy measurement confirms the correctness of the system design, but limited labeled datasets are not of mid-size, we recommend relying on datasets through generation tools~\cite{graph500,gt_graph} and other graph repositories~\cite{matrix_market,snap} for training runtime comparison only.



%redefine the optimization direction and evaluation metrics to ensure that the correct optimizations are implemented.  For instance, optimization techniques for small graphs should prioritize reducing overhead rather than improving GPU utilization.



In use cases that primarily focus on smaller datasets, such as sampling-based GNNs, it is essential to \textit{identify the right methodology to evaluate} the contribution (Recommendation \#4). Our proposed methodology (\cref{sec.overhead}) to measure the framework-runtime overhead informs the practitioner to identify such cases.
%\noindent %$\bullet$
%\textbf{Framework Overhead Research.} 
%The advent of \textit{framework-runtime overhead}, though can be measured using the proposed methodology (\cref{sec.overhead}), 
However, it also presents the community with a new area of research by thinking of it as an operating system. E.g., when we zoom into one kernel operation, it is becoming faster due to powerful GPUs, better algorithms, and other innovations such as quantization, pruning, {sampling}, etc. At the same time, framework overhead remains constant and understudied, which runs in a single CPU core. 
Hence, we infer that the DL framework is now becoming more like an Operating System whose job is to allow access to hardware without introducing much overhead. 
Thus, the future lies in studying those overheads. 


\noindent \textbf{Memory Consumption Related.}
\textit{Frequent OOM and memory consumption should be analyzed} (Recommendation \#5) like runtime with the same zeal (as we do in \cref{sec.mem}) without any pre-assumption. Otherwise, we will continue to have 
%limited choices for current GNN systems to evaluate training performance on mid-size datasets, and end up with 
highly inflated results. 
For GNN systems with non-standard integration processes, additional verification of memory consumption is needed.
% It also asks us to verify the memory consumption for any non-standard integration process.

% \blue{have proposed several techniques to optimize the framework overhead in another paper, which is currently under review. We  are also working on taking framework overhead out of training time.}




% \red{which allows plugging sparse kernels of prior works to the benchmarking platform to fix the system pitfalls automatically while comparison can be performed amid equal framework overhead.}


 %Further,  \td {Need more motivation}
%\red{This is particularly critical as some compilers are designed with techniques adapted from these GNN systems~\cite{ye2023sparsetir}. Therefore, enhancing the baseline system will not only drive the next wave of systems research but will also influence the broader landscape of compiler design, potentially leading to more efficient and innovative solutions.}
%Relying on kernel runtime is not sufficient for evaluation as we discussed in Recommendation\#2. In the absence of a correct and optimized baseline, the evaluation will continue to be compromised for measuring training time as we show in \cref{sec.exp.kernel}.


% \noindent \textbf{Importance of Memory Efficiency.}
% While performance improvement is a well-understood metric, the deep-learning field also requires understanding the memory consumption of the proposed design.
% For example, as Table~\ref{table-gpt} shows, the number of parameters and dataset size in GPT-2 is 1.5 billion and 40GB but jumps to 175 billion and 570 GB in GPT-3. This huge parameter and dataset increase will cause huge memory consumption pressure. GPT-4 is estimated to be around a trillion parameters.
% Based on these observations, the trend of the next generation deep learning models will become much larger and more complex, with a huge increasing number of parameters as well as larger training datasets.
% Thus just the memory requirements mandate usage of many GPUs, rather than fully guided by the performance behavior.

% \begin{table}[t]
% \footnotesize
% %\vspace{-6pt}
% \caption{\small parameter and dataset size from GPT-1 to GPT-4.} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| ccc|c|c|} 
%     \hline\hline 
%      & GPT-1 & GPT-2 & GPT-3 & GPT-4\\% & SpMM \\
%     \hline % inserts single horizontal line
%     Parameter Count& 117M  &  1.5 billion & 175 billion  & trillions(estimate)  \\%&  0.000228\\
%     dataset size & 4.5GB  & 40GB  & 570GB  &   no-release \\  
%     \hline
% \end{tabular}
% %\vspace{-6pt}
% \label{table-gpt} % is used to refer to this table in the text
% \end{table}

% GNN also has seen similar trends. Roc~\cite{jia2020improving} shows that larger GNN models can boost the training accuracy, which provides the potential research direction for large GNN models in the future. 
% However,  as we discussed in the previous section, many GNN systems run out of memory on larger datasets. Hence, in this section, we analyze the GNN systems for performance and memory efficiency both. 

%After the release of chat-GPT-4, the power and effectiveness of large deep learning models are realized and accepted by not only academics but also the industry. Many famous big tech companies, such as Meta and Google, decide to buy more GPUs and develop their own large deep-learning models. Based on these observations, the trend of the next generation of deep learning models will become much larger and more complex, with a huge increasing number of parameters as well as larger training datasets. This new trend emphasizes the importance of optimizing memory consumption. Moreover, the increasing speed of the number of parameters and training datasets is linear times for each development cycle. 

%Therefore, DGL is still the best-performing system in GPU despite being one of the oldest systems around. This is a little ironic as years of research have resulted in systems that claimed otherwise. The reasons for the observation that DGL is the best system around can be attributed to three reasons from prior works: memory corruption or out of memory (OOM); missing end-to-end training loop or requirement misunderstanding issues;  and slower than DGL as reported by themselves or through our measurements when they do not measure on any larger datasets, which is presented next. This observation implies that we do not have any baseline system working in training mode on larger datasets except DGL. Yet DGL has a huge memory overhead that allows it to train only basic GCN models while other models run out of memory in those same larger datasets. We present an analysis next.



 
% Further, DGL also consumes significantly higher memory as shown in 
% Table~\ref{table-obs-memory} for Reddit. DGL cannot train a 3-head GAT model even in the A100 GPU with 40 GB of memory.
% High memory consumption does not allow DGL to run Reddit at all on the older generation of GPUs, such as Nvidia GTX 1080 Ti, and Titan V. We explore the reasons behind its memory consumption in \cref{sec.dgl}.
% Table~\ref{table-obs-memory} shows the results.



%\footnote{\url{https://ogb.stanford.edu/docs/leader_nodeprop/##ogbn-products} shows that PyG can run on OGB-product, however, they use data sampling.}. 


%\subsection{Mismatch between Kernel and GNN System}


% \subsubsection{Details.}
% DGL's backend internally uses Cusparse, a library conceived over a decade ago that offers SpMMve as a general-purpose library that is used by DGL. We discuss the gap between DGL system and Cusparse API.
% %instead of SpMMv and SpMMveid. However, Cusparse is not designed for GNNs only, it is a general library that supports general SpMMve for matrices with non-zeros element in irregular problems. 

% \noindent \textbf{GAT.}
% For {GAT}, we need many SpMM and SDDMM variants.
% For SpMM, DGL first re-arranges the edge-level tensors using the edge ID, called \textit{eShuffle}, before calling Cusparse's SpMMve. These additional kernels and intermediate results \textit{increase memory consumption} by $|E|$.

% For SDDMM, DGL relies on its own implementation using the COO format as Cusparse has only provided SDDMM with the latest version of Cusparse, though it is still slower than DGL's SDDMMvv. Choosing the COO format allows edge-parallel implementation of SDDMM as it is naturally suited for it. However, this speedup is at the cost of additional memory allocation for storing the COO format.  
% Further, there are many non-standard APIs that DGL has to implement itself, such as SpMMe, and SDDMMve which use CSR and COO respectively.


% For transpose needs, the SpMM variant requires the transpose of the sparse matrix along with the edge-level tensor during the backward computation. Even though in GNN datasets each edge is stored in both directions, the presence of the edge-level features in SpMM mandates transposition as it is not symmetric. In another way, the topology does not require an explicit transpose, but the edge-level feature needs one. However, DGL explicitly stores the topology using both the CSR and CSC, while explicit edge ID is used to transpose the edge-level tensors using the eShuffle operation, discussed above. Since eShuffle is an internal operation, it is not part of the DAG, however, DGL internally needs to allocate additional memory for eShuffle. 


% We never need any transpose of the sparse matrix for SDDMM variants. 

% \noindent \textbf{GCN.}
% Cusparse kernel is not suited directly for \textbf{GCN} use. 
% GCN computation never involves any edge-level features, as it only requires SpMM\textbf{v} and not SpMM\textbf{ve}. DGL uses a \textit{dummy edge-level tensor} with each value as 1.0 to implement SpMMv using Cusparse's SpMMve. This leads to an additional memory allocation of size proportional to $|E|$ to keep the dummy edge-leve tensor and computation which is not needed in GCN at all. Further, another kernel needed in GCN is \textit{degree-norm}, which is not offered by Cusparse. DGL uses Pytorch API, which is computed out-of-place. Hence, it consumes another additional memory allocation proportional to $|VxK|$ where K is feature-length.  

% For backward computation, GCN never requires the transpose of the sparse matrix because there is no edge-level tensor present in GCN while GNN datasets are symmetric as it stores each edge in both directions. Moreover, due to the usage of Pytorch API for degree-norm operation, the API becomes a node in the computation graph (DAG) of GNN. Therefore, gradients are also generated and materialized between the operators SpMM and degree-norm kernel, leading to more memory consumption.


%the code study finds that DGL has to implement several extra ad hoc techniques to bridge this gap: 

%DGL first re-arranges the edge-level tensors using the edge ID, called \textbf{eShuffle}, before calling Cusparse's SpMMve; (c) DGL does \textit{additional transpose} using CuBLAS library when using the older Cusparse version, but since CUDA 11 version, it switched to using a new API without needing any such transpose.
%(b) DGL uses a \textit{dummy edge-level tensor} with each value as 1.0 to implement SpMMv using Cusparse's SpMMve. 

%These additional kernels and intermediate results \textit{increase memory consumption} as shown earlier in Table~\ref{table-obs-memory}. 



% \subsection{System Design Analysis} 
% In this section, we analyze the basic building blocks of GNN and show to find out the reason for huge memory consumption and possibly slower performance.
%is a \textit{functionality mismatch} between Kernel API specification and corresponding GNN systems.
%Some works design and optimize the kernel based on the general purpose instead of considering the GNN use cases specifically.  
%These mismatches have forced the GNN system designer to introduce extra steps in the form of workarounds that cause \textit{large memory overead} and \textit{slow down} the overall performance as we show next for DGL before generalization it to other systems.

%The above section explained many mismatches between DGL and the Cusparse API, which is responsible for workarounds that led to a slowdown and huge memory consumption. None of the prior works have highlighted such issues. We now discuss whether these workarounds are due to inefficient system design which is rooted in an inadequate understanding of the domain requirements or not. And whether other works, despite having issues discussed in previous sections, try to solve these fundamental problems or still suffer from these issues.

 
% \begin{figure}[t]
%   \centering
%   \includegraphics[scale= 0.345,left]{result/dgl-format.pdf}
%    \vspace{-18pt}
%   \caption{\small Sample graph and the data layout of COO, CSR, and CSC in DGL.}
%   \label{fig-dgl-format}
 
% \end{figure}




% \noindent $\bullet$ 
% \textbf{Invasive Effort or GNN Benchmarking Tool?} 
% Some pitfalls can be addressed via invasive efforts by prior works themselves, e.g., by developing backward computation code, fixing the order in backward computations, including bias and other mistakenly removed operations to model layers, etc.
% We believe that a more systematic approach by developing a standardized benchmarking tool may allow us to plug their kernel for fair and end-to-end benchmarking. Such work remains a work in progress.

\subsection{{\graphpy}: A Reference System} \label{sec.baseline}

Pitfall-manifested systems cannot be used as a good end-to-end baseline, hence future works would continue to use DGL or PyG as their baseline, leading to inflated results for both the runtime(\cref{sec.spmmt}, and \cref{sec.overhead}) and the memory consumption (\cref{sec.mem}). 
This motivates the need for a new reference system, {\graphpy}, as a baseline for promoting healthy systems research. 
The goal here is to \textit{remove inefficiency} from current baselines based on clear requirement understanding. 
This will allow us to establish a baseline for memory consumption so that memory-saving techniques can be fairly benchmarked, and allow runtime speedup to be fairly reported without taking advantage of the performance degradation of the current baselines due to their inefficient system design. 


Another goal is \textit{practicality} so that some of those ideas can be integrated into prior works productively to solve a few pitfalls.
Moreover, a reference system would show that pitfalls do stifle innovations, and empirically identify wrong conclusions made earlier. Finally, {\graphpy} would establish a new line of optimizations rooted in solving system design pitfalls.  Kindly note that forward SpMM optimization, such as workload balancing, is not an explicit goal here.






%To this end, the reference system, {\graphpy}, is rooted in clear \textit{requirement understanding}. The goal is \textit{practicality} so that some of those ideas can be integrated into prior works productively to solve a few pitfalls; and \textit{efficiency} to save memory and not slow down performance to establish baseline memory consumption and performance. Kindly note that forward SpMM optimization, such as workload balancing, is not an explicit goal here.




%This also means that we cannot use the DGL or PyG as solution.
%inspiring 
%The proposed solution then provides optimization as the transpose design's natural extensions. 
%subsequent optimizations as their natural extension. 
%inspired by an in-depth study of these pitfalls. {\graphpy} includes several optimization techniques tailored to solve these pitfalls, while inspiring the subsequent optimizations as their natural extension. 

% For example, the long-term solution is to develop a native transposed SpMM without using the eShuffle mechanism as in Cusparse. %However, Cusparse does not offer other variants of SpMM, such as SpMMe as its tranposed version is needed during backward computation. 
% However, %while DGL can use native support for SpMMve$^T$ in Cusparse, 
% other systems do not use Cusparse at all, as their custom kernel brings them optimization, and often rely on custom sparse storage formats and are yet to see an efficient open-source solution for SpMMve$^T$. 
% Hence, each such prior work has to develop a transposed SpMM variant, which seems not a practical approach. 
%Unfortunately, we are not aware of any prior works that have focused on native support for transposed {SpMM} variants, and it is not trivial to develop such a native solution. 
%Hence, a more \textit{practical} approach seems similar to DGL but should avoid its extreme memory consumption and slowdown, and allow future integration of native API to handle transposition. 

%therefore serving as a perfect baseline.

%Hence, the \textit{practical} solution should avoid the memory and runtime overhead of the DGL approach or CusparseCsr2csEx2() API. 


% We now focus on {\graphpy} design and show how our proposed technique can complement all the prior works to fix the transpose pitfall efficiently and save huge memory while serving as a reference system.



% \noindent \textbf{Motivation}.
% The question remains open on \textit{the need for edge ID} when 
%Hence, if any GNN system is relying on Cuspasre, there is no reason to not use its full power. 
%\textit{Therefore DGL has first introduced an artificial gap between its system and Cusparse, and then fixes the design pitfall (SYS-P2), which is also responsible for additional memory consumption (M-P1), and also leads to a huge slowdown.} 
%Native support of transpose SpMM equivalent to Cusparse SpMM, which directly acts on CSR format, will be a natural solution as it will avoid the additional need for CSC, and the costly edge ID + eShuffle or CusparseCsr2cscEx() like API invocation. 
%While techniques are available that make forward SpMM faster than Cusparse, we did not find any work that discusses transposed SpMM implementation. 

% No prior works have discussed algorithms for native transposed SpMM, while plenty of works optimize the forward SpMM. Our initial prototype also did not yield good performance, and hence we proceed with another approach and left it as a future work, which we believe is worth exploring. 

%indeed supports transposed SpMM natively by passing some special flag to its \textit{CusparseSpMM()} API that would avoid even the CSC storage, the edge ID indirection, and the eShuffle operation completely.

\begin{figure}[b]
  \centering
  \includegraphics[scale= 0.35,left]{result/graphpy-format.pdf}
  \vspace{-18pt}
  \caption{\small {\graphpy} storage format for sample graph (Fig.~\ref{fig-format}b): There is only one copy of the grayed array representing Column ID array which is shared among COO, CSR, and CSC. The Offset array is shared between CSR and CSC. Edge ID array is for CSC only.}
  \label{fig-graphpy-format}
 %\vspace{-12pt}
\end{figure}


\subsubsection{Storage Format: Edge ID Order}

%Kindly note that GNN 
Our COO format is arranged in CSR-style (i.e., rows are laid out sequentially) as shown in Fig.~\ref{fig-graphpy-format}. This means that the COO and CSR share their column ID array (grayed part in Fig.~\ref{fig-graphpy-format}), and the edge ID arrays. 
% However, the edge-level features are generated individually for each edge using trainable parameters and are not symmetric. %\textit{So, this symmetry should not be misconstrued for symmetry in edge-level tensors.} 
% Hence, edge IDs may still be required to be stored for both storage formats.
We then propose a \textit{novel edge ID reordering}, where CSR and COO (both stored in CSR-style) are allocated consecutive edge IDs, hence we never keep an explicit edge ID array.
However, an explicit edge ID array is kept for CSC.

Further, widely used GNN datasets are symmetric, where each edge is stored in both directions.
% Further, in GNN system, datasets are made symmetric, where each edge is stored in both directions.
We \textit{exploit the symmetry} where we keep one copy of the topology that serves both CSR and CSC. However, symmetry in topology does not imply symmetry in edge ID. So, CSC in {\graphpy} means CSR + edge ID arary. This does introduce heterogeneity in the graph storage. Off course, when symmetry is not there in dataset, CSC topology is also stored separately. 

%and SpMM: \textit{SpMMve} needs just the graph topology, while \textit{$SpMMve^T$} needs both, the same topology and edge ID array.





In total, the format costs in {\graphpy} is only $|V| + 3|E|$ where CSR/CSC needs $(|V| + |E|)$ + COO ($|E|$) + Edge ID array ($|E|$) in CSC  for class A GNN. For GCN, {\graphpy} need only $(|V| + |E|)$. 

%Further, no separate memory allocation for eShuffle-like operation or degree-norm. 

% This simple but fundamental change enables both workload balancing and data reuse. While the former is purely due to the COO format, the latter is enabled by reusing the features of rows across many non-zero elements.
 \subsubsection{Kernel Design.}
In this sub-section, we outline how the simple change in storage format layout along with some other changes allow optimizations in {\graphpy}.

\textbf{{SpMMve$^T$}.}
{\graphpy} implements $SpMMve^T$ natively as one single operation without a separate eShuffle kernel (\cref{sec.spmmt}). It uses edge ID to fetch the correct edge-tensor values while keeping the rest of the SpMMve code the same. 
This also avoids the additional memory that a separate eShuffle requires in DGL. Kindly note that optimizing SpMMve is not within the scope of this work, yet removing eShuffle in the forward, as opposed to DGL, due to format layout changes allows additional benefits.

Other works can easily implement such an approach, even if they rely on a custom storage format as the sequential edge ID will still be applicable for forward SpMMve without requiring any change, while format-specific but explicit edge ID array needs to be generated for $SpMMve^T$. 



\noindent \textbf{SpMMv$^T$.}
For backward computation, GCN requires transpose of the topology only, as there is no edge-level tensor present in GCN. Hence, when the datasets are not symmetric, we only require the transpose of the topology while same API remains usable. 
%it does not require any additional operation as  SpMMv$^T$ is equivalent to SpMMv.
{\graphpy} supports \textit{SpMMv} API natively where the edge-level tensor is not an input.
The API also accepts an optional boolean flag to indicate degree-norm flag. When the flag is true, it only normalizes the result of SpMM as part of the same kernel. However, in the backward computation, a separate \textit{in-place} normalization kernel is called before calling backward SpMMv.
% Clearly, \textit{the community is not designing GNN systems and kernels suited for GNN use cases}, and is relying on workarounds. Hence we are still paying additional costs or not exploring the native benefits that the basic building block offers.
This kernel definition, though very intuitive 
%differs from prior works. Cusparse, FeatGraph, Huang et al offer SpMMve. GNNAdvisor does not make normalization optional and ends up with the wrong fusion during backward. GE-SpMM has mostly focused on SpMMve, and silently implements SpMMv without the normalization option. 
provides substantial memory saving to {\graphpy} on two accounts. (1) Compared to Cusparse compliant SpMMve, {\graphpy} never need to allocate dummy edge-level tensor; saving O($|E|$) memory. This also results in a substantial performance gain. 
(2) Even in the case of a separate degree-norm, {\graphpy} uses the same tensor as input and output both by using in-place degree-norm inside {\graphpy}. 

%On the other hand, DGL performs normalization at the Python level using  PyTorch's CUDA API that can only perform out-of-place normalization, Thus increasing the memory consumption by O($|V|$*feature-length). Hence, DGL-integrated systems, such as GE-SpMM and FeatGraph likely to consume additional memory as well.

\noindent \textbf{SDDMM and Automatic Data Locality.} 
%This kernel operates on the vertex-level features of rows and columns for each edge, and generates output at edge-level. 
The COO format stored in CSR-style leads to a new avenue of data locality in SDDMM, which is purely enabled due to the proposed edge ID reordering while providing a fully workload-balanced SDDMM solution. Specifically, we first divide the COO format equally among warps of the GPU to achieve workload balance. Then within a warp, many edges have the same row ID as COO is laid out in CSR-style.
Hence, the vertex-level features of the same row ID across edges can be fetched once and \textit{reused} multiple times within the warp. 

In contrast, prior SDDMM solutions can either achieve workload balance or data reuse, but not both.
For example, DGL, which uses COO, can achieve workload balance, but can not reuse the features of row ID as its COO is not laid out in CSR-style.  
On the other hand, a CSR-based SDDMM offers data locality for vertex-features of rows, but cannot offer workload balancing. Hence, \textit{all prior systems have introduced a  trade-off: the workload-balanced COO-SDDMM or data-locality based CSR-SDDMM.}

%As neither a row nor a column is laid out consecutively, its SDDMM cannot reuse either the row features or column features while processing the successive non-zero element.

%DGL cannot exploit data locality for vertex features of rows or columns due to its COO format.

% \noindent \textbf{Motivation and Discussion.}
% DGL's COO is neither stored in CSR-style (rows are laid out consecutively) nor in CSC-style (columns are laid-out consecutively).  The order of edges is determined by the dataset file or parsing module which is often performed by the user. Hence, edge ID allocation in DGL is determined by external factors.


%Interestingly, many other works have not implemented explicit SDDMM. They have fused SDDMM with SpMM, and hence their SDDMM remains vertex-parallel using CSR format.


%We now show that edge ID reordering enables excellent data locality in another sparse kernel, namely SDDMM without compromising on its workload balancing. 
%To understand this, we need to focus on the edge ID allocation algorithm in DGL.

% %\subsubsection{Existing Solution.}

% It should be noted that the COO is neither stored in CSR-style (rows are laid out consecutively) nor in CSC-style (columns are laid-out consecutively), but rather its edges are randomly ordered which is determined by the order of edges in the dataset file or parsing module which is often performed by the user.
% Hence, edge ID allocation in DGL is determined by external factors.
% %On the other hand, CSR and CSC have an explicit edge ID as we discussed earlier. 
% %Due to this design choice, COO storage of DGL consumes an additional $|2E|$ memory. Thus total memory requirement for DGL is 2*($|V|$ + $|E|$ + $|E|$) + $|2E|$ just for storage format handling.


% \textbf{Trade-Off.}
% %The above solution brings one trade-off. 
% %As the workload imbalance can slow down the SDDMM kernel, the design decision of DGL is very clear: 
% %introduce memory overhead (extra storage for COO) to impart workload balance to the SDDMM kernel.
% Kindly note that SDDMM operates on the vertex-level features of rows and columns for each non-zero element. Hence, when COO is laid out randomly the vertex-features of neither row nor columns offer data locality.
% %Hence within a row, the vertex-level features of the row can be \textit{reused} if performed using CSR format. This is not exploited in SDDMM due to the way COO is constructed and stored. 
% %As neither a row nor a column is laid out consecutively, its SDDMM cannot reuse either the row features or column features while processing the successive non-zero element.
% On the other hand, a CSR-based SDDMM offers data locality for vertex-features of rows, but cannot offer workload balancing. Hence, \textit{all prior systems have introduced a  trade-off: the workload-balanced COO-SDDMM or data-locality based CSR-SDDMM design.}
% Interestingly, many other works have not implemented explicit SDDMM. They have fused SDDMM with SpMM, and hence their SDDMM remains vertex-parallel using CSR format.


%\subsubsection{{Novel Optimization}: COO stored in CSR-style}

% \noindent \textbf{Implementation Notes and Memory Analysis.}
% We use CSR with vertex-level parallelism for SpMM variants. We incorporated feature-level parallelism~\cite{yang2018design} when the features are vector while using shared memory to cache non-zero element. 
% For reduction, we use a tree reduction~\cite{wang2016gunrock} wherever applicable. These techniques are used by most prior SpMM works. We did not do any specific workload balancing.
% We perform edge-parallel SDDMM by using the COO format but introduce data reuse due to COO being stored as CSR. We do not optimize the resultant kernels or fuse them any further.


%Thus reducing the memory consumption by almost 3$\times$ due to storage design alone compared to DGL without introducing any trade-off.

%%%%%%---------------------



% \subsection{Restrictive Interface for Graph Exchange.}
% \vspace{2pt}
% \noindent
% \noindent \textbf{Description and Implications.}
% The plugin interfaces for GNN systems are limited to accept only tensor type, a specific smart pointer (c10::intrusive$\_$ptr), and built-in scalar types. \textit{This means that we cannot pass a custom class such as graph object through it}.
% Hence, prior works follow many workarounds.
% Earlier systems~\cite{pytorchg2019,spektral,battaglia2018relational,grattarola2021graph} rely on COO format using one or two tensor array(s) of source and destination vertex ID to pass graph.
% %Examples include PyTorch Geometric~\cite{pytorchg2019}, Spektral~\cite{spektral}, Graph Nets developed by Deep Mind~\cite{graphnets}, and others~\cite{battaglia2018relational, grattarola2021graph}. 
% %Clearly, such works leave behind decades of work in graph analytics and sparse linear algebra.
% %Achieving good parallelism is hard when using COO formatted graphs and is slower than CSR/CSC, a well-known fact, and is confirmed in \cref{sec.exp}. 
% %as well as by prior work~\cite{dgl2019}.  
% TLPGNN~\cite{fu2022tlpgnn} and GE-SpMM~\cite{gespmmsc2020} use two tensors to represent the offset array and neighbor array (Fig.~\ref{fig-format}) of CSR.
% %But this hard-coded interface design restricts its kernel to work only on unweighted GNN models, such as GCN using Vanilla CSR/CSC format.
% GNNAdviosr, on the other hand, relies on multiple tensors to pass the graph objects as its neighbor grouping requires two more tensors. 
% Such limitations force researchers to define new APIs for any change in graph storage, hence a stable system API can never be developed leading to productivity loss if one wishes to optimize graph storage format. 
% We did not find any prior works that use the smart pointer approach. But we found it complex to implement as it took us 6 months due to complex and unclear documentation (see appendix for timeline).


% \noindent
% \textbf{Compatibility Loss.} Systems written using a plugin cannot be shared with other DL Frameworks.
% %and hence causes a huge drop in productivity and needs huge investment. 
% For example, Meta first implemented submanifold sparse convolution~\cite{graham20183d} using PyTorch plugin followed by Google~\cite{najibi2020dops} which used the TensorFlow plugin. Google could not reuse the system code-base of Meta because of this framework dependency, resulting in a huge investment.
% Even within the PyTorch family, every version hosts its plugin code and binaries, hence systems like PyG  hosts one version for each major PyTorch release to make the installation job easy, but not the maintainers' job.



% % \subsection{Implementation environment}


% %The conclusion is that relying exclusively on smaller datasets misleads performance results. Further, the absence of training accuracy measurement or forward-only systems cannot fully justify the proposed system optimizations till training accuracy is shown. However, we have fewer baselines for future comparisons on larger datasets for Class A and B end-to-end GNN models. 


% % \begin{table}[h]
% % \footnotesize
% % %\vspace{-6pt}
% % \caption{\small Framework Overhead of both DGL and PyG for GCN model (in Seconds)} % title of Table
% % \vspace{-6pt}
% % \centering % used for centering table
% % \begin{tabular}{|l| r|r |r|r|r|r|} 
% %     \hline\hline 
% %     Graph  & \multicolumn{3}{|c|}{DGL} & \multicolumn{3}{c|}{PyG} \\ % inserts table
% %     %heading
% %     \cline{2-7}    
% %     Dataset & Traning & Total & Percentage & Traning & Total & Percentage\\
% %       & Time & Overhead & (\%) & Time & Overhead & (\%)\\
% %     \hline % inserts single horizontal line
% % %    Cora & 1,719 & 1,349   & 1,719 &1,375 &&\\ 
% % %    PubMed & 1,767 & 1,395  &1809& 1,503 && \\
% % %    Citeseer& 1,697&1,381   & 1,759 &1,409 &&\\ 
% %     Cora & 1.35 &0  & 99.48 & 0.98  & 0&99.28\\
% %     Citeseer & 1.51 &0 & 99.27 & 1.05  &0& 99.23\\
% %     PubMed & 1.48 &0 & 99.32 & 1.20  &0& 99.33\\
% %     % & 76.47 &  76.52 & & \\
% %     \hline %inserts single line
% % \end{tabular}
% % \vspace{-6pt}
% % \label{table-overhead_merge} % is used to refer this table in the text
% % \end{table}



% % \begin{table}[h]
% % \small
% % \vspace{-6pt}
% % \caption{Framework Overhead of PyG (in Seconds)} % title of Table
% % \vspace{-6pt}
% % \centering % used for centering table
% % \begin{tabular}{|l| c cc|} 
% %     \hline\hline 
% %     Graph & Traning & Total & Percentage \\ [0.5ex] % inserts table
% %     Dataset & Time & Overhead  & (\%)  \\
% %     %heading
% %     \hline % inserts single horizontal line
% %     Cora & 0.976 &  0.969 & 99.283   \\ 
% %     Citeseer & 1.046 & 1.038 & 99.235  \\
% %     PubMed & 1.204 & 1.196 & 99.336  \\
% %     % & 76.47 &  76.52 & & \\
% %     \hline %inserts single line
% % \end{tabular}
% % \vspace{-6pt}
% % \label{table-Pyg} % is used to refer this table in the text
% % \end{table}

% % Interestingly, the huge memory consumption for DGL is introduced due to the requirement mismatch handling (points \#1, \#2, and \#3) when using Cusparse kernels. The additional transpose (\#2) requires huge memory equal to $|V|*feature-length$, while eshuffle requires $|E|$ additional memory for each SpMM kernel. These are huge memory requirements. 
% % For PyG, it expects its graph in COO format, which materializes the intermediate  messages that are passed from one vertex to another. Hence, it consumes a huge amount of memory, and cannot run any large graphs.

% % Moreover, large memory overhead may prohibit researchers to run the GNN training in large datasets or on complex models such as GAT. Such high memory overhead may discourage researchers to evaluate end-to-end GNN training on larger datasets on a single GPU, and hence likely to be misled by the performance gain on smaller datasets or through other means. 

% %We believe that this is also one of the reasons that many researchers focused on smaller dataset evaluation only in a single GPU, which led to the wrong conclusion about performance benefits. However, huge memory consumption still discourages a lot of researchers that have access to slightly older GPUs,   and we need to encourage them as well for the advancement of systems research in this important field.

% %If the researchers want to test the GNN models in large datasets, Researchers need to split the large graph into multiple subgraphs and send them to multiple GPUs to do parallel training (\td citations). This multiple GPU setting makes the problem become more complex, and many concerns needed to be worried, such as how to synchronize the results, how to minimize the overhead, and how to optimize the communication between each split subgraph(Graph Partition is an NP-hard problem).



% % \subsection{Requirement Understanding Issues}
% % It is clear from the examples presented earlier that system optimization becomes invalid if system requirements are not understood correctly. We now present some additional examples tailored toward missed optimization opportunities due to the absence of an in-depth analysis of the system requirements.

% % \noindent \textbf{Requirement Mismatch and Its Overhead.}
% % We take the example of DGL to demonstrate some overheads introduced due to the usage of Cusparse as the underlying library for kernel implementations. Cusparse has been developed more than a decade back when GNN was not known. So, it is obvious that it suffers from the requirement mismatch that we present next. 


% % \noindent
% % \textbf{\#1. Dummy Edge-Level Tensor (GCN Only):} GCN performs unweighted aggregation, and hence DGL has to pass a default edge-level tensor, whose value is 1.0 for each edge, to call SpMM of Cusparse requiring additional memory and computation. 
% % %\noindent
% % \textbf{\#2. Two Additional Transpose}: The vertex-level tensor of Cusparse SpMM expects a column-major layout whereas the PyTorch tensor is row-major. Hence, DGL invokes two additional transposes of the vertex-level tensors (\textit{implicit} kernels) for the input and output, which consumes additional memory and computation.

% % \noindent
% % \textbf{\#3. eShuffle (GAT Only):} The Cusparse SpMMve does not support edge ID in its graph storage, therefore, the edge-level tensor is first shuffled by the edge ID that is stored in DGL before calling SpMMve. 

% % \noindent
% % \textbf{\#4. No Support for edge-level vector features (Multi-head GAT Only).} In multi-head GAT,  the edge features are a vector for each edge, which is not supported by Cusparse SpMMve. Further, it requires eShuffle support. 
% % %hence DGL has to call SpMMve kernel multiple times just to handle different dimensions of edge-level features, with same set of vertex-level tensors. 




% % \noindent \textbf{Performance Implication.}
% % Table~\ref{table-kernel-time} shows SpMM run-time for DGL and Cusparse. DGL introduces a slowdown up to 1.64$\times$ over Cusparse due to requirement mismatch overhead. We also plot the eShuffle time for the scalar edge feature. For Reddit, which has a smaller vertex count and a much larger edge count, the eShuffle time is almost equal to SpMMve time, as the transposition of vertex-level tensor (not measured) is small. For OGB-Product, the eShuffle time is significant.
 
% % Interestingly, many new GNN systems are still focusing on optimizing Cusparse SpMMve equivalent kernel in the garb of GNN use cases rather than designing new kernels that are appropriate for GNNs. This is specifically true for systems that integrate with DGL, such as GE-SpMM~\cite{featgraphsc20} and FeatGraph~\cite{featgraphsc20} whose SpMMve implementations do not support edge ID inside their kernel, and hence eShuffle is still needed as a separate kernel that will materialize one additional edge-level tensor. Hence, optimizing SpMMve alone will have a lesser impact on end-to-end training as the scope of SpMMve improvements are small as this kernel has already been optimized by many works over the last many years.   

% % Such works neither provide vector features for edges in their SpMMve nor even talk about SpMMe kernel. Off-course, such works have proposed a newer SpMMv kernel and avoided transpose, but do not offer degree-norm inside it.


% % % \noindent
% % % \textit{\textbf{Observation\#3:} It is clear that focusing on existing sparse kernels alone brings limited performance optimization, and hence end-to-end understanding is needed to fully optimize the system.}

% % \noindent
% % \textit{\textbf{Observation\#3:} It is clear that optimizing the sparse kernels based on Cusparse definition alone brings limited performance optimization because there is a large gap between the GNN requirements and the kernels offered by Cusparse. }


% %Clearly, if the requirements are not understood exactly, then integration of better kernel design may not be the one contributing to the performance improvements. This is because researchers might just remove the need of mismatch of the requirement that may be the major performance contributing factor. 

% %fuse these two steps together or remove the need for transpose for cusparese library and do not apply any optimization techniques, the end-to-end training time will improve a lot. But if the researchers do not understand these steps correctly, and design some optimized kernel to just replace the Cusparse. Even if the optimized kernel is faster than Cusparse, we lose many other opportunities for optimizations. the end-to-end training time will not be improved. (\td not sure whether this DGL example is overhead or not)


% %The above observation is a general problem because GNN system researchers mainly focus on describing the systems technique for better kernel implementation, while accuracy evaluation as well as evaluation on diverse datasets, such as large datasets are not thoroughly evaluated and understood. This sometimes cannot lead to good end-to-end training performance or performance improvement can only be attributed to factors outside of the systems technique of the paper. 


% % Besides the overhead problem, there are other reasons that make the existing works cannot be used as a baseline.
% % As we mentioned in the above section, GNNadvisor has an accuracy problem in end-to-end training. It does not consider the edge id indirection at all so that it can only support a specific type of GNN model, such as GCN, GIN. It cannot work on another class of GNN, such as GAT.
% % Although zhai’s work supports GAT kernel, its kernel implementation is wrong because of the missing edge Id indirection. Moreover, Zhai’s work does not contain the end-to-end training loop. It is also impossible for researchers to implement a training loop by themselves because zhai’s work does not provide a backward process. 
% % Gespmm does not support edge indirection property either, which means that it cannot support GAT. 
% % PyG meets the OOM problem even for the median size data set. It also has a Large overhead for small datasets.
% % Therefore, none of the existing works can be treated as the baseline. 
% % There is a need for a Baseline in GNN systems, which is better than DGL in end-to-end training but does not include any novel opt techniques so that new optimization techniques can be added.


% % Our measurements in Table \ref{table-exp-memory} show that many current GNN systems show out-of-memory conditions frequently on even slightly larger dataset in  single GPU setup. 
% % Reddit graph, which has less than 230 million edges, can not be trained on A100 GPU which has 40 GB memory by PyG, GNNadvisor on any of their supported models. DGL cannot run a slightly complex GAT model, while it still consumes way more than 16 GB memory for GCN, and a simple GAT model. Hence, it is unsuitable on low- and mid-grade GPUs that has small memory, such as Nvidia GTX 1080 Ti.
% % Hence, many prior GNN systems have only demonstrated smaller dataset for performance, which then are affected due to framework overheads that we discuss shortly. 
% % Moreover, many works that do evaluate larger dataset have only focused on kernel benchmarking, but has many issues. 

 
% % We investigate if end-to-end training performance comparison on smaller dataset can really rank systems based on their kernel performance.
% % Table~\ref{table-motivation-overhead} shows overhead for GCN on two smaller datasets of Cora and Pubmed in an A100 Nvidia GPU that includes the time taken by rest of the  Python and C++ code but not kernel time; as well as total training time. The methodology and dataset are described in \cref{sec.exp-gnn.time}. It is very clear from this table that the total training time for Pubmed actually does not depend on the kernel time, as total training time is almost equal to the overhead time. Hence, any optimization of the SpMM kernel will not show up if using DGL to prototype kernels. However, many systems that use PyTorch's plugin approach to prototype GNN on this dataset shows huge performance improvement compared to DGL. Hence, how can we be sure if the performance improvement is purely due to better kernel implementation and not due to difference in the overhead, when we are not able to evaluate larger dataset. 


% % \textbf{Summary}
 
% % To sum up, wring the kernel alone is not enough. There is a need to provide a platform to let researchers really understand the kernel requirements and related topics.





   

==> tex/others.tex <==
\vspace{1mm}
\noindent \textbf{Proposition.}
However, these graph deep learning system cannot directly read the graph structure from the raw data, instead, they rely on some pre-implemented python graph structure, NetworkX ~\cite{networkx08}, or a list of python objects. This design will make the users need to do more graph preprocessing jobs and lack scalability, performance, and cannot handle big graphs. Moreover, NetworkX cannot support dynamic graph representation, which means even if the graph is updated by a small number of edges, the NetworkX needs to re-create the whole graph representation instead of increment updating. This triggered us to design an end-to-end graph deep learning system with a high-performance graph creation modular which can support dynamic graph. 
 
As we mentioned in the introduction, the GNN research area is young, which means many new GNN frameworks with different variant tensor operations or some customized message-passing paradigms maybe proposed in the future. Therefore, the extensibility of graph deep learning systems become important. A good graph deep learning system should be flexible enough to extend to new GNN operations and should be able to add in new customized message passing kernels easily without worry about the code dependency. 
 
Although DGL does provide some extensibility by providing 4 scatter choice ‘sum, sub, multiple, divide’ and 3 gather options ‘max and min, sum’ for users to choose, the message passing paradigms is fixed. If users want to apply a customized message passing paradigms, they need to modify the whole message-passing paradigms as well as the dependent codes in other submodules. This design pattern may limit its usage because graph neural networks are more familiar with machine learning operations and it is hard for them to handle system code dependency.  From the above observation, we put all message-passing paradigms in a pluggable, neural kernels modular and minimize code dependency between different modular. 
 
For some knowledge bases graph GNNs[NEED ADD SOME CITATIONS], the edge information is also captured when applying the graph deep learning. Unlike the traditional edge information which normally treated as the edge weight or a float number, the edge information in the knowledge bases graph can be extended to a vector.[Not sure whether  I understand it correctly or not] Therefore, there is a need for a graph deep learning system to support the customized edge. 


Moreover, different GNNs have different aggregations. GCN uses the unweighted sum as the aggregation. But GAT uses the weighted sum version to assign a weight for each corresponding edge. In other words, edge ID is not necessary for GCN but necessary for GAT. It is unnecessary to always create the edge ID for GNNs. Moreover, the backward procedure of message passing paradigm need to integrate more computation than the forward. If the edge Id can be stored based on the backward procedure, the performance will be improved. Therefore, it is necessary for a graph deep learning system to provide flexible edge choice to users, such as whether creating the edge ID and which procedure the edge ID should be stored. 




\noindent 
$\bullet$ \textbf{New Sparse Formats and Data Sharing}
While we discussed that Numpy arrays will be used to allow zero-copy sharing of graph structured data, and hence it becomes very easy to share CSR/CSC format. However, once a system researcher comes up with an entirely different format~\cite{gstore,mosiacEuroSys17,hicoosc18}, one can think that {\graphpy-DE} as well as the data sharing APIs become non-usable. 
It should be noted that G-Store~\cite{gstore} calls the format Smallest-number-of-bits (SNB), and Mosaic~\cite{mosiacEuroSys17} calls it tile format. HiCoo~\cite{hicoosc18} reduces to the same format when dealing with sparse matrices, but it also extends this to higher dimension sparse data. We use SNB format as it was published first, and explain how the same set of API can be used for graph preparation and data exchange.

\begin{figure}[h]
  \includegraphics[scale= 0.22]{result/zero_tile.pdf}
  \caption{{\graphpy} SNB format.}
  \label{fig-snb}
\end{figure}

 \textbf{Solution: CSR as an Indexing Structure.}
To solve it, we came up with a generalized theory about graph data preparation and sharing that can capture graph in various formats. 
Fig.\td shows the SNB format, which we have re-arranged to make it look like CSR structure. This established the fact that CSR can be used as a general purpose indexing structure, wherever we have one-to-many relationship. 
Clearly, all the data exchange format remains same as it is, e.g. we can still use the 4 Numpy arrays with slightly different dtype to share the graph between {\graphpy-DE}, and {\graphpy-Kernel}, as shown in Listing \ref{list-snb}. It only required one cosmetic change at both the line number 6 and 10. 
%We also needed to modify the $get\_graph$() API that also returned vertex count as we cannot rely on offset array for the vertex count. This also require that we pass vertex count in the $init\_graph$() API. However, all these changes are cosmetic from the user point of view as we provide different version of $prep\_graph$() API.


%Python code highlighting
\begin{lstlisting}[language=Python, caption= Illustration of graph creation in SNB format, label={list-snb}]
import numpy as np
import graphpy as gp
def prep_graph():
  edge_dt=np.dtype([('src', np.int32), ('dst', np.int32), ('wt1', np.float), ('wt2', np.int32)]
  #Directed and SNB graph. 
  G=gp.create_graph(gp.eDdir|gp.eSNB, edge_dt) #Changed code 
  #space is delimiter
  G.add_edges_from_dir('./input_dir/', ' ')
  #Get graph as numpy array using SNB dtype.
  snb_dt=np.dtype([('src', np.int16), ('src', np.int16), ('wt1', np.float), ('wt2', np.int32)]) #Changed code
  csr_offset, csr_neighbor, csc_offset, csc_neighbor = G.get_graph(csr_dt)
\end{lstlisting}

To implement it in {\graphpy-DE}, we still utilized the same infrastructure, but had to adjust the \textit{CSR creation routine} in Fig.~\ref{fig-parallel_pa} to offer graph in SNB formats without changing its APIs.

Off-course, {\graphpy-Kernel} has to implement all the GNN kernel code, but it can still utilize the boiler-plate code. For the proof-of-concept, we integrated G-Store code which also had in-memory processing routine. We also implemented the spmm kernel for GCN. It should be noted that we did not require any changes to the {\graphpy-Workflow}.
%Should this format result into better GNN performance, but we leave it to the respective authors to implement the kernel and find out the details.





\subsubsection{\#2: Integrating Graph Analytics System Research with GNN}

Since existing graph analytics systems usually include optimized high-performance graph computation engine. A straightforward way to test their innovating ideas is to integrate these graph analytics systems with Graph neural networks by simply implementing the new GNN kernels on top of them.

\noindent \textbf{Gap between Kernel and DL Framework.}
One approach to integrate newly written kernel code to current DL framework is to port them to DL Frameworks. However, current DL frameworks does not have support for sparse linear algebra, and hence it is not easy to integrate these system enhancements to improve GNN performance, as it will involve huge efforts not only in integrating into the back-end but also require python binding as per the limitation of these frameworks. Such frameworks allow python binding of limited types.

%To this, end, we list down some basic building blocks, that can guide researchers from graph analytics field to quickly prototype additional functionality on top of the existing code base to test whether those techniques are beneficial or not, before we jump to brand new implementation.
One can try to integrate those code-bases to existing GNN frameworks by porting the existing design and code to them. However, such porting generally requires huge effort to understand the existing development environment and framework. Moreover, their code-base is still nascent, does not have documentation on how one can integrate the code in the back-end, and their code base is constantly changing. Without active involvement of the system maintainer, it seems not possible to integrate new ideas to current GNN frameworks~\cite{featgraphsc20}.
%and as well as  E.g. \td. what are the problems if we integrate in C++ way with Pytorch?  

Hence a more lightweight approach is required, where the job of system researcher should remain limited to implement the required kernels using their design without being restricted to follow a specific development style or any changes to the framework. Yet, it should immediately become part of the whole deep learning workflow. 
This will lead us to a flexible and generic infrastructure that will allow an independently developed pluggable modules, yet taking care of managing computation graph and tensors.


\subsection{Opportunities and Challenges}

The forgone decade saw incredible performance improvement to graph analytics tasks, such as Breadth First Search (BFS) or Page Rank due to various novel system designs, such as better data layout, improved utilization of hardware caches, NUMA-aware data partitioning, structure-aware compression, re-ordering to introduce data locality, integration with various hardware platforms, such as GPUs, FPGAs, customized hardware, etc. 
They improved the performance of graph analytics by orders of magnitude. Many of the techniques are highly graph-aware to take care of its irregularity in the structure and computation both.

On the other hand, GNN computations are very new with the first system level framework appearing recently~\cite{dgl2019}. So, there are plenty of opportunities to improve the performance, and is already being tried~\cite{featgraphsc20}. This is now even more important as deep learning training procedures are  more compute intensive than the tradition graph analysis. So, we are likely to see a number of research direction to optimize the GNN training time including using the techniques mentioned above.

% not all the techniques are possibly applicable to GNN eco-systems due to differences in the requirement between graph analysis and GNN.Graph analytics system researchers were highly influenced by Graph500~\cite{graph500} ranking, which benchmarked BFS or other graph traverse algorithms only. Each iteration of graph traverse algorithms operates on an active vertex set only and contains scalar vertex-level metadata only. However, 

However, trying system system techniques in the context of deep learning is not so easy.
These graph traverse algorithm workloads are very different from the GNNs as GNN have 2 procedures, \textit{forward procedure}, \textit{backward procedure} in each epoch of the training. 
Further, the GNN kernel uses vector metadata and trainable parameters for each vertex and edge in forward procedure and calculate the loss based on the prediction result. In backward procedure, GNN kernel computes the gradient and updated the training parameters based on the loss we calculated before. 
In other words, we can view traditional Graph Analytic works as performing the forward procedure only.
% but do not need the backward procedure.
% \td maybe backward also need to store the gradient information? 
As we discussed in Figure~\ref{fig-forward}, backward procedure has additional requirements, including saving and operating on the tensors produced by forward computation, referred as tensor \textit{states}, and many times operating on the inverse of the graph.

%Nonetheless, considering the variety of work it is natural that  we must test the efficacy of such techniques before putting the verdict out. 

So, if one wants to develop GNN on top of prior graph analytics systems, he or she has to take care of data engineering tasks, implementation of GNN kernels on top of their GAS framework, and the deep learning specific workflow including computation graph and gradient calculations. These tasks have system challenges and involves huge efforts as we discuss next.

% Specifically, many of the techniques focused purely on optimizing the BFS due to benchmarking established by Graph500. BFS is very different than GNN kernels. The former is very compute light, and only a few vertices participate in each iteration. Apart from that the computation only happens in the forward direction in graph analytics as it does not involve gradient computation.



%system which can support graph deep learning features. To be more specific, given the raw input data, such as the CSV, Jason, text or binary data, the graph deep learning system should build the dynamic graph representation data structure automatically and also provides python APIs for users to perform traditional graph topology analysis as well as the graph deep learning operations. 
 
%All the previous works cannot support these requirements, this trigger our work {\graphpy}, which unify the graph data engineering with graph deep learning leads to one integrated graph neural network system and provides end-to-end control over data engineering and machine learning operations resulting in greater synergy and performance.





\subsubsection{Traditional Graph Data Science}


With the advent of data-science as a field, people from many fields are attracted to it. One of the important reason of is easy to program using Python programming language, and the ease with which DL frameworks can be programmed at least in a single node/GPU setup.




==> tex/overhead.tex <==

\section{Framework Overhead + Evaluation Pitfalls} \label{sec.evaluation}
%In this section, we discuss the evaluation.
%Evaluation is the process that makes sure that the hypothesis of the research work stands correct empirically. Hence, any fundamental flaw in the measurement can undermine the hypothesis, which when corrected can prove the hypothesis wrong.
%the semantic gaps in requirement understanding but also the performance misunderstanding.

 
 %and we cannot blame these excellent baselines for relying on memory-intensive solutions. However, it has indirectly influenced the evaluation process as we present the prevalence study next.  

%\subsection{Runtime Evaluation Pitfall} \label{sec.overhead}

% The system design pitfalls indirectly have led to another pitfall related to runtime evaluation. 
% Specifically, The solution implemented by DGL to overcome the design pitfalls is the main reason for the huge memory consumption in DGL (\cref{sec.analyze}).
% Hence, prior works have repeatedly shown DGL as out-of-memory on mid-size datasets that have forced them to excessively or even exclusively rely on smaller datasets for training runtime comparison. 

% Moreover, we suspect that if the same solution is integrated into existing systems, they may also run out of memory. Though at present, this excessive memory consumption has compromised the performance evaluation process.
%In this section, we discuss two pitfalls-- \textit{unawareness of framework overhead}, and \textit{scant or inconclusive evaluation of mid-size datasets}, through a prevalence study and then 


\noindent \textbf{Introduction and Prevalence Study.}
%In this section, we analyze the role of the framework-- the runtime and memory overhead, to show that we have not fully understood the role of the framework in GNN.
We now discuss the role of the framework on GNN performance as many prior works have shown frequent OOM on popular baselines (DGL and PyG) thereby almost all single-GPU GNN training systems~\cite{wang2021gnnadvisor,fu2022tlpgnn,chen2020fusegnn,gespmmsc2020,dgl2019,wu2021seastar,tian2020pcgcn,zhang2022understanding,hu2021efficient,wang2023tc,kim2022analyzing, yan2020characterizing, tian2020pcgcn,baruah2021gnnmark,ye2023sparsetir} %architecture~\cite{liang2020engn,zhang2021boostgcn}
have exclusively or majorly relied on smaller datasets to conclude better training runtime. 
%On the other hand, the results on mid-size datasets are scant, or inconclusive as DGL and/or PyG show OOM, such as Reddit, a widely used labeled mid-size dataset. 
E.g.,
GNNAdvisor, Ge-SpMM, TC-GNN, and others~\cite{hu2021efficient,baruah2021gnnmark} have relied exclusively on smaller datasets for training runtime comparison.
FuseGNN~\cite{chen2020fusegnn}, dgNN, and Seastar used only one mid-size dataset (Reddit), while the remainder are smaller datasets. Additionally, FuseGNN even reports that its GCN is slower than DGL for its only mid-size dataset. However, there is no information on whether FuseGNN's GAT is faster than DGL's GAT, as DGL shows OOM. Seastar also reports OOM in DGL on GAT. 

Though sampling in GNN~\cite{kaler2022accelerating, yang2022gnnlab, waleffe2023mariusgnn, liu2021bgl,lin2020pagraph,song2022rethinking,jangda2021accelerating,ye2023sparsetir} uses large datasets to evaluate runtime, it should be noted that they {sample} the dataset in each iteration to generate a smaller graph to run training/inference. E.g., such works only pick 256 vertices to {sample} the graph, while picking only 10 (for example) neighbors, if those vertices have more than those neighbors. Hence, the resultant {sampled} graph is small. 
%to be impacted by the framework overhead pitfall. 
%We next show measurements to back up the claim.
%\red{Many multi-GPU GNN systems are designed based on single-GPU, which are also impacted by the pitfall of framework overhead.}


%We would like to discuss two more aspects of sampled GNN systems. Firstly, we do not analyze multi-GPU GNN systems as we kept out of the scope of this paper (\cref{sec.prevalence}) as we wanted to avoid the impact of multi-GPU communication on runtime. However, it becomes very logical that if the sampled dataset is small enough in a one-GPU system, it will become even smaller in multi-GPU systems. Secondly, the sample-based GNN performs sampling plus kernel computation in each iteration. 
%Sampling takes the whole dataset as input, while kernel takes the sampled graph as input. In this paper, we have only analyzed kernels and not sampling.



% This section discusses two performance evaluation pitfalls that have undermined our ability to conclude: \textit{Unawareness of framework overhead}, and \textit{Scant evaluation of mid-size datasets}.  

%\subsection{Pitfalls}

% \noindent \textbf{Introduction and Prevalence Study.}
% Almost all singe-GPU GNN systems~\cite{wang2021gnnadvisor,fu2022tlpgnn,chen2020fusegnn,gespmmsc2020,dgl2019,wu2021seastar,tian2020pcgcn,zhang2022understanding,hu2021efficient,wang2023tc} %architecture~\cite{liang2020engn,zhang2021boostgcn}
% are impacted by these two pitfalls together, as they exclusively or majorly relied on smaller datasets, which is due to lower framework overhead and not due to better kernel performance. Evaluations on mid-level datasets were scant, inconclusive, or slower or suffer from the accuracy issue described earlier. 
% These two pitfalls together question the validity of the evaluation process as it does not indicate superiority as we explain in this sub-section.


%\subsection{EVAL-P2: Framework Overhead Pitfall} \label{sec.overhead}

%

%We discover a fundamental pitfall in the evaluation process. %of prior works that exclusively and majorly rely on smaller datasets for showing performance gain. 


%This observation is critical because many prior works have exclusively relied on smaller datasets for performance evaluation. On the other hand, almost all prior works have majorly relied on smaller datasets, out of which some works have reported inferior performance on mid-size datasets, while others may have relied on just one additional mid-size dataset. This suggests an inadequate evaluation that either does not allow to draw conclusions. 
%or may have masked the inefficiency of their underlying optimization techniques.

\subsection{EVAL-P2: Framework Runtime Overhead} \label{sec.overhead}
The end-to-end training time in small datasets is dominated by framework overhead instead of kernel runtime. So, the training speedup in such cases is due to the lower framework overhead (unknowingly) instead of better kernel runtime (claimed). 
%We measure the training time of a few prior works on two popular mid-size datasets of Reddit and OGB-product. 
% The \textit{aim} of this survey is to understand the behavior of prior systems on mid-size datasets.
To clarify, we first present our proposed methodology, simple yet effective, to measure the framework overhead. We also evaluate to understand the overhead when graph size is varied. We reason for the differences in framework overhead. We finally discuss {sampling} in GNN.



\noindent \textbf{A Novel Methodology.}
%We are the first ones to propose such a new methodology to assess the framework overhead in GPU-based GNN systems. 
Eq.~\eqref{eq-overhead} defines the overall framework overhead, which is a sum of the time consumed by the CPU for each training epoch ($k$) in a single-GPU system. %The $k$ represents the number of epochs in the training procedure. 
Kindly note that GPU kernel invocation is asynchronous to the CPU, and it does not wait for the kernel execution to finish-- a well known practice. Hence, measuring the time taken by each epoch without waiting for the kernels to finish execution roughly measures Python and C++ code runtime executed in the CPU. We can use this time to calculate the overhead. 
In this measurement, $k$ is set to [0, 200). %Listing~\ref{list-overhead} shows how simple it could be to compute the overhead time.


\vspace{-12pt}
\begin{equation}\label{eq-overhead}
\textit{Framework$\_$Overhead} = \sum_{k}\textit{$CPU$\_$Runtime$}
\end{equation}
\vspace{-12pt}


\noindent \textbf{Measurements.}
%To make sure this framework overhead is a general pitfall instead of a cherry-pick case. 
We first plot the overhead ratio for DGL in Fig.~\ref{exp-dgl-overhead} for different edge counts in the graph. Indeed, the overhead is close to 100\% for graphs with an edge count of up to 4 million edges before dropping slowly. For Reddit, DGL has only 5.42\% overhead for GCN showing that framework overhead has less impact on mid-size datasets.  
%Table~\ref{table-exp-overhead} shows the DGL framework overhead for Pubmed and Reddit datasets on GCN compared to training time, where overhead is almost 100\% of training time in Pubmed. 
% \blue{This overhead difference \textit{proves that the proposed methodology to measure framework overhead is valid}}. 
We also verified it with other GNN models.  


\begin{figure}[t]
  \includegraphics[scale= 0.51]{exp/overhead_size.pdf}
  \vspace{-18pt}
  \caption{\small DGL framework-runtime overhead when training GCN for 200 epochs on graphs ($|V|$=32,768). {The left figure shows that framework overhead is 100\% of the training time when edge-count is $<$ 4 Million. The right figure shows the framework overhead remains similar irrespective of the edge count.}}
  \label{exp-dgl-overhead}
  % \vspace{-12pt}
\end{figure}



% \begin{lstlisting}[language=c++, caption= {\small Showing overhead time and training time collection}, label={list-overhead}]
% def GNN_Training ():
%   ...
%   #Training Stage
%   start = datetime.datetime.now()
%   for epoch in range(200):
%     start1 = datetime.datetime.now()
%     loss = model(graph, feature)
%     loss.backward()
%     optimizer.step()
%     end1 = datetime.datetime.now()
%     overhead += datetime.datetime.now() - start1
%   torch.cuda.sync()
%   training_time = datetime.datetime.now() - start
% \end{lstlisting}

% Here we separate the total framework overhead into two detailed categories, \textit{start-up cost} (first epoch) and \textit{runtime cost} (rest 199 epochs). We use the time for the first training epoch in CPU to represent the start-up cost and the sum of the remaining epochs as the runtime cost. (\td add a pseudo code to explain it) 

% \begin{table}[h]
% \footnotesize
% %\vspace{-6pt}
% \caption{\small Framework overhead in Seconds for GCN on Pubmed. Overhead on Reddit is also shown for comparison.}
% \vspace{-6pt}
% \centering 
% \begin{tabular}{|l|r|r|r|} 
%     \hline\hline 
%     Graph & Overhead Time & Training Time & Overhead (\%)\\% & gSpMM \\
%     \hline % inserts single horizontal line
%     Pubmed & 1.470 &1.480 & 99.32\% \\%&  0.000228\\
%     \hline
%     Reddit &  1.402 &  25.839 & 5.42\% \\%& 0.031 \\ 
%     \hline %inserts single line
% \end{tabular}
% %\vspace{-6pt}
% \label{table-exp-overhead} % is used to refer this table in the text
% \end{table}



%and 50\% for graphs with an edge count of up to 16 million.

% It is clear that for the small dataset--Pubmed, the total framework overhead (start-up cost + runtime cost) is almost the same as training time. 
% On the other hand, for large datasets-- Reddit, the framework overhead time for DGL is 1.402 seconds only, much smaller than the 25.839 seconds training time. 
%  For Reddit, we were able to run only DGL, while others show out-of-memory (PyG) or memory corruption (GNNAdvisor). 


We evaluate the overhead for multiple GNN models across three widely used small datasets: Cora, Pubmed, and Citeseer. Fig.~\ref{fig-obs-overhead} shows that the overall training time is dominated by the framework overhead, and not by the kernel performance. The source of overhead varies in different systems. 

% \blue{Kindly note that the training loop and model layer (written in Python) remain almost identical between DGL and PyG while the Kernel module is different. Hence they produce slightly different overhead.} 


\begin{figure}[t]
  \includegraphics[scale= 0.42]{exp/overhead_obs.pdf}
  \vspace{-24pt}
  \caption{\small Training and framework runtime overhead for DGL, PyG, GNNAdvisor (GNNA), and dgNN for GNN models training for 200 epochs. Seastar also has almost 100\% overhead for these datasets.}
  \label{fig-obs-overhead}
%\vspace{-8pt}
\end{figure}

%DGL white paper also explains that it has a higher framework overhead than PyG. 

%For the impact of the dominant framework overhead in small datasets, it may misguide the direction of the GNN optimizations. That is because moving GNN layers and other integration code to C++ instead of optimizing kernels or other computations will actually affect the overall training time in small datasets. For example, GNNAdvisor exclusively relied on smaller datasets for performance evaluations. But it uses the PyTorch plugin and moved GNN layer code from Python to C++, resulting in less overhead compared to DGL. 

In GNNAdvisor,  two changes allow it to have a lower overhead than DGL: removal of bias parameter in its GCN layers, and use of C++ to write GNN layers instead of Python. Though GNNAdvisor also suffers from accuracy issues.
%Removing the bias parameter also contributes to its lower accuracy, which we discuss under different headings. 
%Thus, it avoids executing Python code and framework overhead of DGL. 
Indeed, many systems develop GNN from scratch and hardly rely on integration to DGL, and can easily outperform it. A new specialized system never suffers the overhead of DGL, which is due to the generality that it offers: a generic message passing infrastructure that can model almost any sparse kernel, conversion of Pytorch tensor to DLPack tensor to DGL-specific tensor are a few things that allow DGL to support newer GNN models, and many general-purpose DL frameworks, such as Pytorch, Tensorflow, MxNet, etc. but also introduces overhead.

On the other hand, systems integrated into DGL, such as GE-SpMM~\cite{gespmmsc2020} (not shown in Fig.~\ref{fig-obs-overhead}), show hardly any performance improvement in their paper for GCN for smaller datasets on which it relied exclusively in its paper despite showing better SpMM kernel time than Cusparse. This is because the overhead remained the same as DGL.
However, it wrongly attributes this observation to the number of prediction classes not being a multiple of 32. 

%Since GE-SpMM used DGL for integration, which merely replaced the Cuspasre kernel with itself, 


%Kindly note that the feature-length in the last layer depends on the prediction classes, such as 6 in Citeseer, 7 in Cora, and 3 in Pubmed. %which is not optimized by GE-SpMM.

%Though we do not plot the overhead for other systems, such as dgNN, and dgNN because they suffer from accuracy issues. Even then we observe the same behavior.

\noindent \textbf{Sampling.}
In Reddit and Ogb-product datasets, our measurements for GraphSage sampling using DGL show that the maximum edge count is always less than 0.45 million which is very small (see Fig.~\ref{exp-dgl-overhead}). Hence, further measurements show close to 100\% overhead for training on these two datasets. For example, 
%sampling took around 19 seconds, while 
the actual training procedure took around 48 seconds in the OGB-Product dataset, which is also the total overhead during backward and forward computation. %showing that overhead during training is close to 100\%. 
When doing the same measurement in MariusGNN~\cite{waleffe2023mariusgnn}, the training time improved to around 22 seconds but still had close to 100\% overhead. In summary, GPU kernels play no role in training time in this case.

Even for the paper100M dataset, one of the largest used in sampled GNN training, the generated sampled graph has between 13k--2M edges~\cite{waleffe2023mariusgnn}.
Fig.~\ref{exp-dgl-overhead} shows 100\% overhead for GCN if the edge count is less than 4 million in the sampled graph. 
As GraphSage uses GCN for training after sampling, we conclude that the framework overhead is around 100\% of training time in a sample-based GNN system. 


%It should be noted that the methodology is slightly different while measuring the overhead he
%This measurement also highlights that if sampling produces smaller than 4 million edges, the training time is not determined by the kernel run-time taken by GPUs in DGL. 



==> tex/prevalence.tex <==

% \begin{figure}[t]
%   \centering
%   \includegraphics[scale= 0.66,right]{result/gnn-crop.pdf}
%   \vspace{-6pt}
%   \caption{\small todo.}
%   \label{fig-training}
%  %\vspace{-12pt}
% \end{figure}


\section{Prevalence Analysis and Scope} \label{sec.prevalence}

This paper focuses on \textit{single-GPU GNN systems}, and analyze in-depth over 20 systems~\cite{wang2021gnnadvisor, fu2022tlpgnn, huang2021understanding, gespmmsc2020, zhang2022understanding, featgraphsc20, dgl2019, jangda2021accelerating, liang2020engn, yan2020hygcn, pytorchg2019, chen2020fusegnn,tian2020pcgcn,wu2021seastar,wang2023tc,kim2022analyzing, yan2020characterizing, tian2020pcgcn,baruah2021gnnmark, ye2023sparsetir, waleffe2023mariusgnn} in the last 5 years, and are from the top systems and HPC conferences, such as EuroSys, OSDI, ASPLOS, ATC, MLSys, SC, IPDPS, HPDC, and PPoPP among others; hence should not be termed as cherry-picking. 
%Sampling in GNN picks only a few labeled vertices and their fixed neighborhood count, such as only 10 neighbors per vertex. Hence, sampling produces a smaller graph in each training iteration, and the framework overhead pitfall (EVAL-P2) applies to such works. Here, we only present a study on training and not on sampling. 
% We analyze and comment on the %training process as a whole, which automatically focuses on 
% system building, of which individual kernel optimizations play a big part. 
%It is backed by a detailed code study and evaluation of many open-sourced works.
We note the following important points: 




% GNN systems fall into two categories of non-sampling and sampling-based GNN; each of which can be
% single-GPU, multi-GPU, CPU-GPU systems, etc. In this work, we pick \textit{single-GPU non-sampled GNN systems for our in-depth analysis} and analyze roughly 20 systems~\cite{wang2021gnnadvisor, fu2022tlpgnn, huang2021understanding, gespmmsc2020, zhang2022understanding, featgraphsc20, dgl2019, jangda2021accelerating, liang2020engn, yan2020hygcn, pytorchg2019, chen2020fusegnn,tian2020pcgcn,wu2021seastar,wang2023tc,kim2022analyzing, yan2020characterizing, tian2020pcgcn,baruah2021gnnmark,ye2023sparsetir} in the last 4 years, and are from the top systems and HPC conferences, such as OSDI, ASPLOS, EuroSys, ATC, MLSys, SC, IPDPS, HPDC, and PPoPP among others.
% Similarly, sampling in GNN picks two levels of sampling: a) only a mini-batch of labeled vertices is picked followed by b) selecting a fixed neighborhood count of the vertices of the mini-batch, such as only 10 neighbors. 
% %We are rather inspired by this line of work, as papers have to show the impact of sampling by measuring overall accuracy. 
% %many pitfalls are applicable in this case, specifically, 
% Hence, sampling produces a very small graph in each training iteration, and the \textit{framework overhead pitfall} (EVAL-P2) applies to single-GPU works. 
% Here, we only present a study on training and not on sampling. Considering such diverse works should not be termed as
% cherry-picking.  
% In addition, we would like to make the following important points:


%These papers can represent the prevalent current state-of-art research studies for system-level GNN optimizations and should not be termed as cherry-picking.
% Excluding some works focus on accelerator and hardware architecture.
%This should not be thought of as a finger-pointing exercise against the papers we analyze in-depth as without in-depth analysis we cannot conclude.

%~\cite{wang2021gnnadvisor, fu2022tlpgnn, huang2021understanding, gespmmsc2020, zhang2022understanding, featgraphsc20,wu2021seastar,tian2020pcgcn,dgl2019,pytorchg2019,wang2023tc}, 

%\noindent \textbf{Scope.}
%However, its sampling and training procedures are done together during training, hence it requires a more complex analysis, and
%These works verify the correctness of their optimization by testing its accuracy among different datasets. We do not focus on this class, as measuring accuracy is a prerequisite that also avoids many issues that we discuss in the other two classes. 
%\noindent \textbf{Scope and Clarification.}
%Our analysis shows that several pitfalls exist among these works, leading to fundamental issues in evaluation and system design that do not allow them to conclude decisively and often bar their deployment directly. 


%\begin{itemize}[noitemsep,topsep=0pt]
% \item 
\noindent $\bullet$
The paper is not related to reproduction issues. \textit{We indeed can observe and reproduce similar results}. The paper is based on our interpretation of those results and doing additional evaluations on accuracy, framework overhead, and kernel run-time through newer evaluation methodologies, and confirming the observations through code study. %that can hinder the advancement of GNN system research, if unaddressed. 
It may be possible that a single-GPU system, in case our extensive search missed them, doesn't have these pitfalls. But that doesn't solve the case that studied pitfalls are prevalent within the current landscape.
It is essential to note that not all papers within the GNN domain succumb to every pitfall, and the paper does not seek to cast blame on all techniques proposed by existing works.

%\item 
\noindent $\bullet$
We have discussed this paper with the authors of GNN systems having pitfalls over email/teleconference/face-to-face to avoid misunderstandings or potential conflicts regarding our paper. Overall, we have received positive and encouraging feedback. Supplementary material shows code analysis and discussion, which would be open-sourced along with {\graphpy} and other artifacts for healthy discussions.

%\item 
\noindent $\bullet$
Single-GPU systems are \textit{foundational} because their performance and memory consumption form the basis for other settings. 
Additionally, with the increase in memory size in modern GPUs and the advent of numerous memory-saving techniques, such as lower precision and quantization~\cite{halfpre,effhalf, dlhalf, QDLhalf}, gradient check-pointing and/or re-computation~\cite{zhang2022understanding}, kernel fusion~\cite{wu2021seastar,zhang2022understanding}, better mini-batching plus sampling~\cite{waleffe2023mariusgnn} have allowed a GPU to train larger datasets. 
%Indeed, paper100M, one of the largest open-source graph datasets, can be trained in a single-GPU. 
%This enhancement underscores the importance of their analysis in the context of GNN performance.
%\item  
%Hence, we focus on the role of kernel optimizations and their cost of integration with a single-GPU system  without worrying about the costs of CPU-GPU and inter-GPU communication. This establishes a 
Hence, our analysis and corresponding evaluation methodologies, focused on single-GPU systems, establishes the right foundation and methods which can be extended for other settings, such as multi-GPU systems~\cite{wang2021flexgraph,cai2021dgcl, md2021distgnn, zheng2020distdgl, p3gandhi2021,tripathy2020reducing, wang2021flexgraph, jia2020improving, Thorpe2021DorylusAS, ByteGNN22, DSP23, Yang2022WholeGraphAF, yang2022gnnlab,mgg2023}. 
E.g., DistDGL~\cite{distDGL} is built on using DGL~\cite{dgl2019}, while MGG~\cite{mgg2023} is built on GNNAdvisor’s~\cite{wang2021gnnadvisor} idea of neighbor grouping. We leave their analysis as future work.



%\vspace{-6pt}

% This way, we can focus on a single-GPU setup by avoiding the role of CPU-GPU and inter-GPU communication costs in our measurements.
% Also, with increasing memory size in modern GPUs,  and as the performance and memory consumption of a single-GPU system forms the basis for a distributed design, analyzing the former is very important. 


%\end{itemize}




%Sampling~\cite{kaler2022accelerating, yang2022gnnlab, waleffe2023mariusgnn, liu2021bgl,lin2020pagraph,song2022rethinking,jangda2021accelerating}

% \red{distributed + sample ~\cite{ByteGNN22, DSP23, Yang2022WholeGraphAF}}

% \red{just sampling(mul GPUs) ~\cite{yang2022gnnlab, mgg2023}}

% \red{sample(one GPUs and mul GPUs)~\cite{TGL22}} 

% \red{sample (one GPUs)~\cite{waleffe2023mariusgnn}}
% \red{distributed just ~\cite{p3gandhi2021} ~\cite{jia2020improving}, ~\cite{ Thorpe2021DorylusAS}}


%\red{many websites of conference or workshops for Reproducibility Challenge ~\cite{mlre22, rai2020, iclrre2019, neuripsre2019}}

%Our analysis is based on not only their papers but also their code and if it is open-sourced. (Most of these works are open-source) We also add and modify some of their code to make sure we did not omit their work. (The modification of their code will be put in GitHub also to guarantee our analysis)
% Moreover, these pitfalls are fundamental design pitfalls instead of specific engineering flaws. 
% We are the first ones to find and propose/summarize these pitfalls. None of the existing open-source projects do realize and solve them. 

%The two GNN classes capture many variations of graph storage and kernel requirements. Hence we use them to analyze the GNN works and present some critical observations that motivate our work. 


==> tex/requirement.tex <==
% \section{Requirement Misunderstanding Pitfalls} \label{sec.semantic}

% In this section, we discuss many pitfalls related to misunderstanding the GNN requirements.
% The semantics of requirement is the most important criterion for system design and development. Hence, if the requirements are misunderstood, the developed systems are of no use as we cannot rely on their runtime performance, while their proposed optimizations become questionable for deployments. Based on our analysis, we find such misunderstandings have led to wrong system design that unfairly boosts their runtime performance. Lastly, we discuss and provide some recommendations about how to catch such critical issues.

% %Some works are implemented in a simulated environment. Those works implemented the forward kernel only. Their backward procedure implementation is missing and they use the forward kernel to simulate the backward kernel behavior.  

% %\subsubsection{Description and Implication}

% %\noindent\textbf{Description.}
% \subsection{Pitfalls}

% \textbf{Introduction and Prevalence Study.}
% As we highlighted in \cref{sec.intro}, the requirement misunderstanding comes from the fact that deep learning training involves a \textit{forward} and a \textit{backward} computation that involves calling a series of operators, which ultimately calls one or more GPU kernels. 
% In the following pitfalls, we first highlight some of the fundamental knowledge about the GNN requirements, and then point out the corresponding pitfalls. 

% The analysis is theoretical and requires code-study, and debugging techniques to locate the pitfall. Hence, we pick the systems based on systems evaluated in \cref{sec.evaluation} as we are sure that debugging abnormal accuracy may be due to fundamental problems in requirement understanding and system design. Hence we analyze many works~\cite{fu2022tlpgnn,wang2021gnnadvisor,zhang2022understanding,huang2021understanding,wu2021seastar,wang2023tc} that are published in Top-Tier conferences like OSDI, Eurosys, ATC, MLSys, PPoPP, and HPDC, and locate their pitfall.


\section{GNN System Design + Evaluation Pitfalls} \label{sec.accuracy}

In the next few sections, all experiments are run on an Nvidia A100 GPU.
Datasets and other details are presented in \cref{sec.exp}. 


\textbf{Introduction and Prevalence Study.}
In this section, we discuss about our understanding of system design and evaluation for GNN models, specifically because of the fact that  
several GNN systems~\cite{huang2021understanding, wang2021gnnadvisor, zhang2022understanding, wu2021seastar, wang2023tc, gespmmsc2020,fu2022tlpgnn,wang2021flexgraph,hu2021efficient,jangda2021accelerating, liang2020engn, zhang2021boostgcn, kim2022analyzing, yan2020hygcn,ye2023sparsetir} have established a clear trend of not reporting training accuracy in their paper. %Even a few sampling-based GNN systems do not show accuracy.
%We observe that many GNN systems optimizations works do not measure training accuracy in their research papers, 
A few of them rely on emulated version of forward computation due to missing backward computation which cannot fit into any training process. 
%We measure training accuracy if backward computation is present and have not reported accuracy.  



%These works can be classified into two categories: (a) those that do not implement a complete model; and (b) others that do have complete model implementation but do not perform the training accuracy measurements. We present some examples of the mistakes that gain performance at the expense of accuracy. 

%Many optimization works do not measure accuracy. They can be categorized into two: systems that do not have back-propagation of GNN operators; and systems that have the training loop but do not measure the accuracy.

%In this section, we measure the accuracy of the second category of works and show that their accuracy is not the same as DGL. For the second category, we refer them to the semantic discussion.

% FeatGraph reports accuracy.



\subsection{EVAL-P1: No Accuracy Measurement}
%\noindent \textbf{Methodolgy.}


We show that many papers have abnormal accuracy (Fig.~\ref{pitfall-accuracy}) due to requirement misunderstanding that leads to fundamental and engineering issues in their system design and implementation for GNN models. DGL accuracy is for reference. 

%Observation is discussed next.

%It should also be clarified that these works have not reported training accuracy.
%We only picked top-tier conference papers to do the measurements. Also, see \cref{sec.accuracy.discuss} for more discussion.

%reasons such as CUDA compute version dependency where scripts (Pytorch setup tool) automatically pick the latest compute version of the GPU, even when using older Pytorch and CUDA toolkit, but the compiler refuses to compile. Reliance on older versions of DGL on top of which a few works have been developed, or other software that has substantially changed, or their API is deprecated like Networkx, Scipy, Cusparse, etc. that create issues that require manual fixing. 

%Pytorch plugin environment (setup tool) also shows many issues due to the requirement of additional CUDA compute versions and tools that are not needed. 

%Hence, we run these systems for a huge number of epochs and monitor their accuracy at each epoch to make sure that captured results are valid, and are not being affected by random weight initialization. We also run the experiments many times to confirm the abnormal systems, while also being independently reviewed by other co-authors and friends.




%We find that many works~\cite{fu2022tlpgnn,wang2021gnnadvisor,zhang2022understanding,huang2021understanding,wu2021seastar,wang2023tc} that are published in Top-Tier conferences, like OSDI, Eurosys, ATC, MLSys, PPoPP, and HPDC, suffer from wrong accuracy pitfalls.

%Though this work is not focused on setting up the environment, it is indeed a complex exercise even after tools such as virtual environment features of conda or pip3.  
%Hence, we only analyzed works that we were able to run to show their poor accuracy. 



\textbf{Class A GNN.}
Seastar~\cite{wu2021seastar} shows a drop in accuracy by 4.5\% - 26.9\%, while TC-GNN~\cite{wang2023tc} have very very low accuracy on all the datasets for GAT. 
FuseGNN~\cite{chen2020fusegnn} GAT shows NaN during training on Reddit and could achieve only 58\% accuracy, way below DGL's 92.4\%.
%dgNN~\cite{zhang2022understanding} faced a very different problem: its GAT training accuracy for Cora, Citeseer, and Pubmed reaches abnormally high (close to 100\%) within very few epochs of training and stays there. For Reddit and OGB-product, it does not reach the same level of training accuracy, reaching only 47.95\% even after 5,000 epochs for Reddit. 
%In comparison, DGL has a stable accuracy of around 70.48\%. No other works have such high accuracy on vanilla GAT with a single head.
%for the Reddit and Ogb-product datasets is abnormally low, while On the other hand, 
We did not run Huang et al~\cite{huang2021understanding}, and TLPGNN~\cite{fu2022tlpgnn} that have GAT but they do not implement backward computation. 
GNNAdvisor does not provide GAT implementation.
% which cannot fit into any training process due to the absence of backward computation.

%is only 1.83\% and 15\%. But for Cora, PubMed, and Citeseer, the accuracy is 100\%. 100\%, and 98.33\% respectively, which is abnormally higher than the DGL accuracy. It does not implement GCN.

\begin{figure}[t]
  \includegraphics[scale= 0.47]{exp/pitfall-accu.pdf}
  \vspace{-24pt}
  \caption{\small Accuracy comparison: TC-GNN does not provide GAT, hence AGNN is substituted here as both are attention-based(Class A GNN). We also discuss other works in the text. DGL is for reference. } %Missing results are due to out-of-memory conditions.}
  \label{pitfall-accuracy}
% \vspace{-12pt}
\end{figure}

\textbf{Class B GNN.}
GCN training accuracy in TC-GNN is abnormally low. Seastar accuracy drops by 4.5\% - 19.8\%. 
GNNAdvisor~\cite{wang2021gnnadvisor} drops by 14.8\% -- 24\%. Also, GNNAdvisor throws a memory corruption error for Reddit and OGB-product, which is also reported by others~\cite{fu2022tlpgnn}.
Huang et al and TLPGNN do not have backward computation implemented.  
%dgNN does not support GCN.
Ge-SpMM~\cite{gespmmsc2020}, which does not report accuracy, could not be run due to major code reorganization in DGL to which it was integrated. 
Featgraph~\cite{featgraphsc20}, which is integrated into DGL, we could not install it correctly despite help from its authors and trying several GitHub branches though it did report accuracy on Reddit. Except for DGL, only PyG and FuseGNN have normal accuracy on GCN.

%\subsubsection{Impact Analysis and Discussion}

\noindent
\textbf{Fundamental Problem or Evaluation Oversight?}
Academic prototypes usually do not have the same level of evaluation as commercial prototypes. However, one cannot claim that missing or significant drop in accuracy is an evaluation oversight as these systems usually aim for the \textit{semantic-preserving model}, same model as the baseline (DGL in this case) with changes tailored for their system optimizations. 
We next analyze these systems to study the pitfalls in system design.

%the accuracy evaluation is the only simple method that can verify the correctness of the GNN system.
%which forces the GNN system to develop from scratch even though the basic essence of the model remains the same.
%as the model and datasets are the same, with minor changes to the model, such as due to kernel fusion.
%In \cref{sec.semantic}, 
%We have uncovered both fundamental and engineering issues by debugging accuracy errors that can not be ignored as they also contribute to better performance, 

\subsection{Misunderstood Backward Computation} \label{sec.semantic}
Our analysis for drop in accuracy is attributed 
to \textit{insufficient understanding of backward computation and their impact on forward computation}. 
%to errors in  understanding requirements semantically, 
Thus one can find the presence of runtime performance enhancing bugs in their wrongly designed system.  %Hence significant errors in accuracy in those same datasets for which systems are evaluated is not an oversight. 
We also note that correct baselines deploy inefficient designs despite availability of efficient choices. 
%inadequate training to current student researcher, etc.  
Next few sub-sections presents these system design and evaluation pitfalls.


%

%as a reason for abnormal accuracy,  while also highlight other system design design and implementation issues. 
%\red{More detailed code analysis is provided in Appendix \ref{appendix:a}.}

%: (1) during backward, it calls degree-norm after the SpMM in its fused kernel which must be called before; 
% (2) its model does not have a bias parameter compared to DGL evaluation which has the model bias parameter. Thus it unknowingly trades off accuracy for performance without explicitly mentioning it. 


%It is clear that there are some problems in the kernel code of dgNN. (The training and model configuration for all these 5 datasets are fixed to avoid any performance variation)


\subsubsection{SYS-P1: Omitted State Tensor}
Many works fused kernels to optimize the system performance without considering the state tensor requirement for backward computation. 

\noindent\textbf{Definition and Example.}
The backward computation of any operator needs to access the \textit{state tensor}-- the input and/or output tensors of the corresponding forward operator. Whether it needs just the input tensor or output tensor is operator-specific. Such tensors must be saved during forward computation to be used during backward computation.  
Hence, when backward computation is not implemented, their emulated forward computation does not generate and materialize many state tensors. So, kernels could be fused across operators by writing some computations to shared memory or device registers rather than to global memory to gain performance advantage.
Without considering the data write and data read to global memory for the state tensor(s), their performance speedup is over-stated.


% Many GNN systems claim to improve the GNN training performance but do not implement backward of any operator at all. They attempt to fuse multiple operators but do not generate the state tensor at all. These missing state tensors will cause problems for backward procedures.  
% Indeed, without considering the requirement for the backward procedure, many steps and necessary tensors are omitted. 
% %and multiple changes to the data-structure are used 
% which is otherwise not feasible, which we discuss shortly. 


%Since these works do not have backward implementation, they do not consider the requirement for backward procedure. However, compared with forward procedure, the backward procedure may have extra requirements such as the need for edge-level tensor, a trainable model parameter, or extra computation steps, such as edge-level tensor reshuffling. 


%E.g., the backward computation in the GAT model needs both SpMM and SDDMM kernels that depend upon an edge-level tensor and vertex-level tensor(s).  
%(This requirement is mentioned in another paper also.~\cite{wu2021seastar})
Kindly note that state tensors requirement should not be seen from sparse operations only, but many other operations, such as ReLU, Dropout, etc. operations need to store state tensors.  
Huang et al~\cite{huang2021understanding} and TLPGNN~\cite{fu2022tlpgnn} prototyped one giant fused forward kernel that fused many sparse kernels along with other operations, such as ReLU, etc. 
%which are required for the linear layer, dropout layer, etc. 
Hence, their forward-only implementation took advantage of kernel fusion to completely remove the computation and storage of many state tensors. {E.g., TLPGNN did not materialize the attention score in GAT-- an edge-level state tensor, while Huang et al. and TLPGNN did not materialize the state-tensor for the ReLU operation.}
Kindly note these two works claim to optimize GNN training, and not GNN inference, hence, they are not analyzed for the latter. 

%We should also note that the proposed work does not work for inference also due to some other issues, which are not focused on in this work.

\noindent $\bullet$
\textbf{Fundamental Issues or Implementation Issues?}
Clearly, substituting emulated forward computation as a replacement for GNN training is not a good benchmarking practice. 
%But to do that they have tried to substitute the forward computation as a replacement to GNN training, but were unsuccessful at that emulation due to misunderstanding about state tensor.
%Since the academic prototype does not go through the same rigorous quality check as commercially implemented systems have, hence it is always possible to discover some implementation flaws in their code. So, 
Indeed, \textit{kernel fusion}
is a well-studied technique to improve performance in many scientific and graph computations in GPUs. However, in DL training, kernel fusion is not so straightforward where 
%It must fuse them carefully in order to produce intermediate results (tensors) that are needed for backward computation. 
materialization of the state tensor is a fundamental design factor that needs to be considered carefully.
The existing optimizations will not hold if someone decides to fix this pitfall. Further, fixes need critical thinking and design changes, such as the re-computation of state-tensors~\cite{zhang2022understanding} which itself requires saving some other tensors as state-tensors. This saving and re-computation procedure leads to extra slowdown, so the speedup claimed by such works is not practical even if their kernel optimizations are valid.

% \blue{For example, the backward operation of SpMMve in GAT is both the SpMMve(V, E $\rightarrow$ V) and SDDMMvv(V, V $\rightarrow$ E) kernel, where V represents the vertex-level tensor (gradient and state-tensor) and E represents the edge-level state-tensor. 
% However, when the kernels are fused in the forward direction by avoiding the generation of $E$,  every graph-related GNN kernel becomes vertex-centric ($V \rightarrow V$) due to this misunderstanding, and hence the forward computation can fuse many kernels easily as applying vertex-level parallelism faces no challenge whatsoever. 
% Clearly, fixing the issue will introduce a new system-level challenge to fuse kernels that follow different computation paradigms, and yet still generate the state tensor. This may introduce trade-offs that require greater scrutiny during system design. 
% %Hence, such prior works have not discussed the design trade-offs that are needed in order to make kernel fusion work. 
% Such trade-offs are likely to impact the runtime performance and memory consumption both. Hence, this is not a simple bug-fixing exercise. }

%Its backward propagation of fused GAT SpMM kernel, which is missing in these works will be incorrectly abstracted to (V, V $\rightarrow$ V) which falsely avoids the key design problem we mentioned above. 

% %by thinking that it never needs to generate any edge-level tensor, and hence
% %and  computation that are in practice not feasible.  
% When fusing these two operations together, the optimization design needs to consider the data locality for both the vertex-level tensor and edge-level tensor. 
% This part is hard because it is impossible to achieve the coalesce read/write for both the vertex-level tensor and edge-level tensor at the same time. 
% This ununified computation property becomes the key design problem researchers need to take care of for optimization. 
% On the other hand, if the fused kernel falsely drops off the intermediate edge-level tensor. 

%To sum up, this materialization of tensors that are overlooked by prior kernel fusion works does not allow some optimization during kernel fusion, such as it cannot avoid the computation that produces edge-level tensors as those are required to be computed and materialized.  


\subsubsection{SYS-P2:Incorrect Order of Backward Operations}

A few works that attempt kernel fusion do not order their backward operation correctly, which leads to better performance at the expense of wrong training. 

\noindent\textbf{Definition and Example.}
The backward operations, as the name suggests, invoke the kernels in the reverse order to the forward operations. For example, if operator A is called first followed by operator B, then the backward computation first needs to call the backward of operator B followed by the backward of operator A. However when the operators A and B are fused in forward, their backward requires a different custom fused kernel to take care of the ordering.

%A few works that attempted kernel fusion during the forward computation, suffer from a lack of understanding of the same during backward computation as those works did not reverse the order correctly during its backward computation. 
For example, GNNAdvisor~\cite{wang2021gnnadvisor} fuses the SpMM and degree-norm operators during the forward. However, its backward computation did not reverse the order at all. 
%We also suspect that this is the reason for the low accuracy of 
For Seastar~\cite{wu2021seastar} in GCN, the accuracy drop is similar to GNNAdvisor. This is because Seastar relies on a lambda function specification for fused forward SpMM and degree-norm in the forward() API of the GCN layer to generate CUDA code. The generated code always calls degree-norm after SpMM. 
%However, no lambda function specification for backward is visible or controlled by the user. 
We suspect that code-generation logic may not be intelligent enough to generate correct backward fusion.  
%However, as we show in the case of GNNAdvisor, the wrong ordering has only a 14.8\% to 24 \% accuracy drop in GCN. 
%For GAT, the involvement of more operations leads to an even higher drop in accuracy in Seastar.


\noindent
\textbf{Fundamental Issues or Implementation Issues?}
An independent \textit{degree-norm} fetches the degree of every \textit{row}, thus occurring $|V|$ data load. 
It can easily be fused to forward SpMM, as degree-norm happens on the output-tensor of SpMM, which requires fetching the degree of every \textit{row}.  
However, during backward, it should be called on the input-tensor of the SpMM. Hence, a correct fusion during backward computation needs to fetch the degree of column ID of every NZE, thereby fetching $|E|$ data load.   

So when this operation is wrongly performed at the output of the backward SpMM, the fusion wrongly fetches the degree of each row occurring only $|V|$ data load instead of every NZE. Hence the fused kernel gains performance due to less data load and computation. 
%vertex-centric computation performs $|V|$ computation and data-fetch, but an edge-centric operation performs $|E|$ computation and data-fetch. 
%For GAT, the performance benefit is even higher because of more complex operations.
%Indeed, Seastar GAT with 4 layers is actually 2$\times$ faster than their 2-layer GCN on Reddit and Ogb-product datasets, explaining the performance exploitation of such pitfalls. We have never come across this observation where GAT implementation is faster than GCN.
Clearly, fixing such issues is not simple, but requires greater scrutiny of system design. 


% \subsubsection{P4: Removal of Model Parameter}

% \noindent \textbf{Definition and Example.}
% Apart from the above, it goes without saying that model needed to be almost the same in comparison to prior works unless the new proposed model is discussed and evaluated for the changes. For example, We should not be removing bias parameters without explanation, as it is a mistake. 

% We see that GNNAdvisor, Huang, et al, and TLPGNN do not have a bias parameter at all in their GNN model without any explanation. However, they did not remove the bias parameter from DGL when doing the evaluation. In DGL, the bias parameter is enabled by default, but their evaluation scripts do not disable it, resulting in an unfair performance gain.  




\subsubsection{SYS-P3: Regarding Sparse Matrix Transpose}  \label{sec.spmmt}
%\label{sec-P2}

Backward SpMM computation ($\delta X \leftarrow A^T \delta Y$), requires transpose of the edge-level state tensor ($A$, the sparse matrix) in the SpMM operation ($SpMM^T$). 
The sparse matrix (A) itself can be viewed as two parts: the static part(the graph topology) and the dynamic part(the edge-level state tensor $W_e$). While, one can pre-process the graph to keep the transpose of the topology, the generated $W_e$ requires transpose at run-time.
%We discuss whether prior systems perform it and how they perform it.

\noindent
\textbf{Definition and Examples.}
\textit{1)} A few GNN systems did not transpose the edge-level state tensor during backward computation leading to non-practical performance gain.
Many works~\cite{fu2022tlpgnn,huang2021understanding} do not implement backward computation by ignoring this problem, TC-GNN~\cite{wang2023tc} substitute forward SpMM in place of backward SpMM for its attention-based GNN. 
Kindly note that the popular GNN benchmarking datasets are square (sparse matrix), and hence not performing transpose does not lead to dimension mismatch, and cannot be caught during compilation/runtime unless accuracy is measured. 
% However, in GraphSage, sampling produces rectangle matrix, and hence shows the limited range of GNN case for which such systems are designed, albeit wrongly.
%\red{However, in GraphSage, sampling produces a rectangular matrix, which leads to obvious errors when such system designs are applied.}


%Thus,  key baseline of 
%We show that forward SpMM is not a substitute for backward SpMM as their design and performance attributes are very different.  Hence, these works need to add extra steps which require critical thinking, and are time-consuming if they want to integrate with end-to-end GNN training.


%which includes the transpose of the topology and edge-level tensor.
%For SpMM in the forward direction, the backward requires a transpose of the edge-level state tensor. 
%As far as the data structure is concerned, their graphs do not keep edge ID which is needed for GAT training to achieve transposition in the backward procedures. 

%We revisit this again in \cref{sec.spmmt} to show that others have an very inefficient design, despite a native SpMM$^T$ (and faster) is available in Cusparse.
%dgNN even has a code for transposing the edge-level tensor, but is not used in GAT.
%Seastar~\cite{wu2021seastar}, which borrowed DGL's method of transpose implementation suffered from a huge accuracy drop. 
%Rather, except for DGL and PyG, we did not find any other works that actually implement the backward SpMMve correctly. 


%We want to point out we do not know how much corruption these flaws will cause. 
%For example, the flaws of missing an edge-level model training parameter $W$ may have a huge impact on the proposed optimization for SpMM. because this $W$ affects the data read, computation order, and even data locality(\td not sure), which are the fundamental factors when designing the optimization techniques. Since this flaw almost changed the fundamental design factors, the existing optimizations may not be applicable anymore. To solve this problem, there are two ways. The first way is converting the graph CSR to CSC first and then applying the transpose. Another way is creating an extra edge\_id  list and using it in the SpMM backward to avoid the transpose. However, both ways are time-consuming and will slow down the end-to-end performance speed up a lot. (\td should we put some experimental result here?)

\textit{2)} Other systems did develop additional mechanism to take care this requirement, however, they completely ignore the fact that Cusparse natively offer $SpMM^T$ without performing explicit transpose of $A$. 
So, prior GNN systems that rely on Cusparse, never use its native API nor compares against it to show better performance of their additional mechanism.    
Our measurements (Fig.~\ref{exp-gpu-SpMMve}) show that native SpMM$^T$ by Cusparse is still the fastest. 
%Thus, prior works have introduced an inefficient system design against the key baseline kernel of Cusparse, a widely used library for benchmarking other kernels.
%This pitfall discusses the slowdown introduced by many GNN works by unnecessary additional mechanisms.
Thus, this pitfall have allowed many sub-optimal system design to dominate the GNN solutions. Even worse, as we explain next, such additional mechanisms are have introduced additional memory consumption. We first analyze DGL for its memory-intensive SpMM$^T$ approach followed by a discussion of alternate mechanisms. This also serves as an understudy for our reference system (\cref{sec.baseline}).


% There are a few options that require an additional step: 
% 1) Use APIs to explicitly transpose the sparse matrix and the edge-level tensor such as the Csr2cscEx() API of Cusparse. 
% 2) Another option is to rely on a pre-processing step that can save the CSR and CSC formats of the graph to handle the topology part. But for handling the edge-level tensor, another mechanism is needed. DGL uses a novel method. We discuss these methods in \cref{sec.analyze}.
% {Transpose of Sparse Matrix} can be done through these techniques, but have different performance values. Rather both technique incurs huge time-consuming performance cost than forward SpMM. (\td add the experiment result here)

%explicit edge ID is required to be managed. \td explain more. The cost of this eShuffle operation is higher than the forward SpMM itself.

% The disadvantage of this approach is that it transposes both the topology and the edge-level tensor. The topology could be transposed once as a pre-processing step. The cost of these APIs is rather higher than the forward SpMM itself as per our measurement. \td show the number.

%Clearly, existing forward-only SpMM algorithms cannot be substituted for the backward SpMM. 
%Currently known solutions (\cref{sec.spmmt}) are inefficient.


% \subsubsection{EVAL-P1: Ignore a Key Baseline for SpMMve$^T$} \label{sec.spmmt}
% %Our further investigation of the excessive memory consumption issue has led to the discovery of a crucial observation in class A GNN: 
% SpMMve$^T$ ($\delta X \leftarrow A^T \delta Y$) API is natively available in Cusparse, yet prior GNN systems neither rely on it nor have shown better performance than it.    
% Our measurements (Fig.~\ref{exp-gpu-SpMMve}) show that native SpMMve$^T$ by Cusparse is still the fastest. 
% %Thus, prior works have introduced an inefficient system design against the key baseline kernel of Cusparse, a widely used library for benchmarking other kernels.
% %This pitfall discusses the slowdown introduced by many GNN works by unnecessary additional mechanisms.
% Thus this pitfall have allowed many sub-optimal system design to dominate the GNN solutions. Even worse, as we explain next, such additional mechanisms are have introduced additional memory consumption. We first analyze DGL for its memory-intensive SpMMve$^T$ approach followed by a discussion of alternate mechanisms. This also serves as an understudy for our reference system discussed in \cref{sec.baseline}.
% %and also overlook some basic insights that could easily avoid pitfalls (Mem-P1) of huge memory consumption and the slowdown in the popular baseline of DGL. Specifically, the memory-intensive solution was designed to implement SpMMve$^T$ in DGL, which is already available in Cusparse as a native API. Rather than using the native API, DGL designed a solution so that it can use SpMMve to implement SpMMve$^T$.




%Many follow-up works such as Seastar, FeatGraph, and many other systems using DGL back-end infrastructure continue to use the same mechanism without major alteration.  Others have also come up with additional mechanisms. 

%Unfortunately, none has evaluated these additional mechanisms on whether they provide better runtime than the SpMMve$^T$ API of Cusparse. 

%implying that we are yet to fully understand different aspects of the GNN system. %\textit{a unique pitfall}. 

%a system design pitfall by overlooking the obvious solution and introducing slowdown and memory consumption. 

%One can claim that the issue of excessive memory consumption in DGL and PyG itself is not a fundamental pitfall as deep learning, in general, also suffers from high memory consumption due to state tensor materialization.
%However, DGL which uses CSR  does not materialize edge-level tensors in its SpMM, so high memory consumption requires more investigation than what we know before we term it a fundamental pitfall or not. 

%
%These mechanisms are responsible for huge memory consumption and significant slowdown.

%PyG's continued reliance on the materialization of edge-level intermediate results has not solved this issue either.

%which has forced us to have a very poorly designed baseline in terms of performance and memory consumption. 



%However, DGL stores a separate copy of the CSR and CSC topology, which is not needed.  Prior works may have noticed the GNN dataset symmetry as they do not store both the CSR and CSC, however, they misconstrued it for symmetry in both the topology and edge-level tensor. Hence, they neither have an edge ID-like design nor transposed SpMM implementation. Hence, these works substitute backward SpMM with forward SpMM, which is not correct in class A GNN.

%DGL's design falls short of exploiting the dataset symmetry as it keeps CSR and CSC both. Further, 

\noindent $\bullet$ \textbf{DGL.}
To support SpMM$^T$, DGL relies on a separate kernel, termed as \textit{eShuffle}, and \textit{edge ID abstraction} in the graph storage.  Every edge of the graph in DGL is assigned a unique numerical identifier in the range of [0, $|E|$). Its allocation is determined by its COO format (used for SDDMM implementation): the offset of each edge in the COO is its implicit edge ID (see Fig.~\ref{fig-format}c). However, the order of edges in DGL's COO (i.e., storage layout) is determined by the dataset file or parsing module which is often performed by the user (external factor), and hence its COO is neither stored in CSR-style (rows are laid out consecutively) nor in CSC-style (columns are laid out consecutively). 
In such a case, both the CSR and the CSC contain an explicit array of edge IDs (Fig.~\ref{fig-format}(d, e)). 
%Their COO format also with an explicit edge ID
%DGL also keeps the COO format for its SDDMM implementation that relies on implicit edge ID, 


DGL's SpMM and SpMM$^T$ rely on \textit{eShuffle}, an internal GPU kernel, to re-arrange the input edge-level tensors using the edge ID array to generate a new edge-level tensor so that it can use the same SpMM API of Cusparse for both SpMMve and SpMMve$^T$. 
%That is, the \textit{DGL uses the eShuffle operation during both the forward and backward computation}, and the usage of the edge ID array of CSR or CSC determines whether it is SpMMve or SpMMve$^T$ respectively. 
The eShuffle slows down performance by 64\% of Cusparse SpMM on Reddit (\cref{sec.exp}) on both forward and backward, and hence is very costly. 
%Thus, DGL implements transpose (SYS-P2) by additional memory allocation and slowing down both the forward and backward SpMM through eShuffle depspite a native Cusparse API being available. %Due to the eShuffle kernel, DGL also consumes an additional $|E|$ memory per SpMM.
%Further, it always requires an additional memory of size $|E|$ to capture the shuffled edge-tensor output per SpMM.
Hence, any system integrated into DGL suffers from similar issues, but an independently developed system can get additional performance benefits if it suffers from missing transpose pitfalls, while forward-focused systems automatically gain 64\% speedup without any optimization. 
%Seastar uses the same storage design.

Memory consumption in DGL for storage formats is $2|V|+6|E|$ due to CSR $(|V|+|E|+|E|)$, CSC$(|V|+|E|+|E|)$, and COO($|2E|$) irrespective of GNN models. Due to eShuffle, DGL also consumes an additional $|E|$ memory.

% The COO format is used for SDDMM implementation, and explicit edge ID array in CSR and CSC is used for supporting SpMMve and SpMMve$^T$ in DGL. 
%\noindent $\bullet$ \textbf{DGL SpMMve and SpMMve$^T$.}
%Moreover, there is more consumption due to the way kernels are implemented in DGL due to explicit edge ID in both its forward and backward computations as discussed next.



%For example, PyG, which shows OOM on Reddit and OGB-Product as reported by prior works~\cite{chen2020fusegnn,huang2021understanding} as well as observed by us in A100 GPU(40GB memory), 

\noindent 
$\bullet$ \textbf{PyG and MariusGNN.}
PyG implements SpMM and SpMM$^T$ by materializing messages at the edge level using global memory before gathering at the destination vertices in its original design of using the COO format.  
Hence PyG shows OOM more frequently as it cannot run on an A100 GPU with 40GB memory, and has been reported by prior works~\cite{chen2020fusegnn,huang2021understanding}.
However, Cusparse does offer an efficient SpMM on COO, which is ignored.
Lately, PyG uses CSR without materializing edge-level tensors on GCN, however, GAT (which uses SpMMve/SpMMve$^T$) still materializes them.
MariusGNN uses a PyG-like solution, i.e., it materializes the messages at the edge-level on global memory. This mechanism is very slow than using native Cusparse APIs (\cref{sec.exp.kernel}).

%Similarly, PyG also experiences memory overhead from its framework, despite its GCN adopting the CSR/CSC storage format to conserve memory. This issue arises because its Class A type GNNs still utilize the COO format and save edge-level output, which significantly increases memory usage. This additional memory consumption causes PyG to run out of memory on midsize datasets, such as Reddit and Ogb\-Product.

\noindent $\bullet$
\textbf{Other Mechanisms.}
Seastar and FeatGraph also rely on edge ID indirection for GAT in both the forward and backward computations. 
FuseGNN relies on \textit{CusparseCsr2cscEx2}() API (which transposes the topology and edge-level tensor) plus their custom forward SpMM to implement SpMM$^T$. CusparseCsr2cscEx2() API is slower by 130\% of Cusparse SpMM on Reddit, thus this mechanism is even more costly.
Others~\cite{huang2021understanding,fu2022tlpgnn,wang2023tc} have mistakenly avoided transpose. 
%and hence they are not at all aware of the above design trade-offs that we discussed. 


\noindent
\textbf{Fundamental Issues or Implementation Issues?}
Backward SpMM is fundamentally different than forward SpMM because the transpose need introduces a basic trade-off. %cannot be read even read at all if the SpMM algorithm remains the same as proposed by prior works. 
To illustrate, prior works assume the sparse matrix (static + dynamic parts) in a row-major layout, where forward SpMM reads the row using coalesced memory access, though their finer details vary.
In transposed SpMM, if one does not perform an explicit transpose or alter the algorithm, then the sparse matrix must be read in column order sacrificing the coalesced memory access. Even if one keeps the transposed topology, reading the row-major $W_e$ in column order is needed.
\textit{It is not possible to read a row-major sparse matrix in column order without additional metadata or processing.} 

So, dropping the requirement itself, either through missing backward computation or substituting forward SpMM in place of backward SpMM does not present us with those trade-offs in various designs possible, while ignoring the key baseline of Cusparse leads to no progress in state-of-the-art in basic kernel design of $SpMM^T$ (\cref{sec.exp.kernel}).
%Thus, these works have unrealistic and non-practical performance gains. 
%In summary, systems neither utilized native $SpMMve^T$ of Cusparse nor proposed a better solution than it.


% \subsubsection{\red{EVAL-P4}: Requirement Mismatch for SpMMv} \label{sec.mem.gcn}
% The class B GNN, (e.g., GCN), does not involve an edge-level tensor, and hence edge ID, COO format, and eShuffle kernels are not needed. Yet, DGL consumes significant memory as it still keeps the same storage, introduces requirement mismatch,  and uses other inefficient designs as discussed next. 
% %even when GCN does not need edge ID and COO format. 
% %However, there are more reasons for huge memory consumption in this case. 

% \textit{a)} Cusparse provides only SpMMve API which is not suited directly as {GCN} needs SpMMv API. Hence, DGL uses a \textit{dummy edge-level tensor} with each value as 1.0 to use Cusparse API, consuming an additional $|E|$ memory. A few GCN systems~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} are still focused on optimizing SpMMve despite the focus on GCN. 
% %Moreover, DGL unifies the storage format for all GNN, therefore it still keeps separate copies of CSR, CSC, and the edge ID array.
% \textit{b)} DGL does \textit{degree-norm} out-of-place. This not only allocates $|V*K|$ sized additional memory(K is feature-length) but the division also becomes a node in the computation graph (DAG) of GNN. Therefore, gradients are also generated and materialized between SpMM and degree-norm kernel.
% \textit{c)} DGL processes the degree array before each call to degree-norm due to the presence of empty rows in the sparse matrix. In this case, DGL calls (\textit{clamp}()) API which sets the degree to 1.0 for empty rows for each iteration, introducing further slowdown and additional $|V|$ sized memory.




% \noindent \textbf{Overhead.}
% DGL does not exploit the dataset symmetry, further introduction of edge ID increases the memory consumption even more, while an additional intermediate tensor is allocated for the output of the eShuffle operation. 
% Invoking additional kernel \textit{introduces a huge slowdown}. E.g., as shown in Table~\ref{table-kernel-time} a separate eShuffle brings a slowdown of up to 100\% in SpMMve for Huang et al (\cref{sec.exp}), and 64\% over Cusparse on Reddit.

%Hence, it is clear that there is a mismatch between the GNN system (DGL) and Cusparse API. However, without answering the above two design questions, it is not clear who (GNN System or Cusparse) is responsible for this mismatch.




% \textbf{Method 2.}
% For the systems that do have not backward implementation or have accuracy issues, we believe that directly evaluating their kernel can be another methodology to make sure that we do not discard their advance in basic kernel design, like SpMM and SDDMM. This may not be possible if prior works have only implemented fused kernels, and wrongly. 
% %As part of this work, we have developed scripts including modifying their back-ends to allow evaluation of basic kernels, such as SpMM and SDDMM, if present in prior works.

% % case of frequent out-of-memory observation, first, it should be analyzed and presented with the same zeal as the runtime, otherwise, we will continue to have limited choices for baseline systems to evaluate training performance on mid-level datasets. Secondly,
% % Though we will not be able to test the accuracy due to the absence of label information, we can use the smaller labeled dataset to check the accuracy to make sure that the implementation is correct. 


% \noindent \textbf{Summary.}
% As the framework overhead is the main reason for speedup on smaller datasets where total training and overhead time is around 1-2 seconds, observing performance does not present any insight about the techniques invented.
% Hence, observing performance in larger datasets is very critical. 
% The evaluation and discussion clearly state that DGL is still the best-performing system for larger datasets in GPU despite being one of the oldest systems around except for a few closed-source systems which we could not measure. This is a little ironic as years of research have resulted in systems that claimed otherwise. This clearly establishes the deficiency in the evaluation process which has relied excessively on smaller datasets in end-to-end training. 
% %need to have a better understanding of evaluations 

% \noindent \textbf{Overhead Reduction.} %==================
% Though none of the prior works discussed how to reduce the overhead, they unknowingly reduced them. In this part, we understand the technique behind the reduction and comment on those techniques on whether one should follow such a strategy for framework reduction or not.
% One can say that the framework overhead is around 1-2 seconds for 200 epochs, and is definitely not a major performance issue in end-to-end training as it does not impact much when training on larger data (\td not sure what this sentence means). 
% %We argue that it is the not amount of overhead that is important here, but the fundamental question of systems understanding as we explain below.


% GNNAdvisor does not use bias in its GCN, so we compare it with a version of {\graphpy} where bias was commented, and ignored the wrong kernel order in GNNAdvisor.
% This comparison presents a new insight as its layer implementation is in C++. We can clearly see that moving code from Python to C++ leads to less start-up cost because PyTorch spends hardly any time preparing the computation graph, however, that does not reduce the run-time overhead. 
% Though it is slightly faster than {\graphpy} for smaller data sets due to reduced start-up cost, we would not recommend writing layers in C++. 

% 1) Moving code from Python to C++ cannot improve performance in large datasets. 
% 2) GNNAdvisor did not follow the correct approach to writing layers. It merges layer kernels together into one complex operator in C++. However, this fused operator forces us to manually invoke the backward computation of every kernel, such as the linear layer. 
% 3) Our experience shows that writing model layers in C++ correctly is complex and instructions are not clear. When we used the smart pointer approach and wrote layers in C++ it took us almost 6 months to implement GCN (see appendix). 

% % {\textit{An overhead of around a second is not a major issue, but showing performance gains based on smaller datasets alone is not acceptable either. Because of this finding, we do not focus on small datasets and use large datasets for evaluation.}}

%%%%%%%%%%%%========================%%%%%%%%%%%%
% \subsection{EVAL-P3: Scant Evaluation on Mid-Size Datasets}
% We now focus on mid-size datasets as training runtime for smaller datasets depends upon framework overhead.
% We notice that many prior works did not evaluate mid-size datasets at all, while a few that do evaluate have mixed results, such as either slower than DGL, DGL showing OOM, or accuracy issues, which do not indicate superiority. 

% %and hence comparison will not truly compare the performance that was supposed to be there in those papers at that time. 
% \noindent \textbf{Performance Survey.}
% %We measure the training time of a few prior works on two popular mid-size datasets of Reddit and OGB-product. 
% The \textit{aim} of this survey is to understand the behavior of prior systems on mid-size datasets and find out the current state-of-the-art so that they can be analyzed in-depth later.


% \textbf{Class A GNN.}  
% Seastar, dgNN, Haung et al, TLPGNN, and FuseGNN all have accuracy issues (and system design issues), and hence their performance can not be relied upon for GNN training.
% PyG always runs out of memory (OOM) on Reddit and OGB-Prodcuts. This has been reported by prior works~\cite{chen2020fusegnn,huang2021understanding}. 
% Kindly note that our result used its original design of using COO format that implements SpMM by materializing messages at the edge level using global memory before gathering at the destination vertices. This materialization causes out-of-memory. 
% %This whole thing is usually avoided by other works such as by using SpMM directly.
% Its latest release uses the CSR format, however, it continues to rely on materialization to implement GAT, and hence still shows OOM.


% %  shows that DGL GAT runs out of memory for its only mid-size dataset in its paper, but it also has very low accuracy.
% % Seastar~\cite{wu2021seastar} evaluates GAT on Reddit, but it shows out-of-memory conditions on DGL. But it also suffers from low accuracy (see \cref{sec.accuracy}).
% % %and we used end-to-end training for 200 epochs, while they shown for one epoch only.
% % %now uses the latest Cusparse for SpMM, while its SDDMM has adopted best practices from FeatGraph.
% % %Our measurements show 
% % dgNN shows better performance than DGL in the paper but suffers from accuracy issues(\cref{sec.accuracy}). 
% % %while many of its technique has also been merged into DGL as it relies on its own implementation of sparse kernels that are not available in Cusparse.
% % Huang et al, and TLPGNN relied on an emulated forward computation to show better than DGL performance. However, they have fundamental pitfalls (\cref{sec.semantic}) in their system design. 
% % %Further, these three systems also suffer from major design issues that we discuss in \cref{sec.semantic}, 
% % Hence, we cannot rely on their performance as end-to-end systems. 

% Others, such as GNNAdvisor, PCGCN, NeugGraph, and Ge-SpMM do not focus on class A GNN. 
% %\textit{In Summary, DGL is the state-of-the-art system for conducting training correctly.}


% \textbf{Class B GNN.}
% In this class of GNN, more works have been proposed than in the class A GNN. 
% GNNAdvisor which suffers from accuracy issues as discussed in \cref{sec.accuracy} faced illegal CUDA memory access on Reddit and OGB-Product, which is also observed by others~\cite{fu2022tlpgnn}. 
% %of the  Other works suffer from the issues mentioned for class A GNN, such as semantic issues, and hence they are not an end-to-end system for GNN training.
% FuseGNN~\cite{chen2020fusegnn}, which has correct accuracy for GCN reports that it is slower than DGL for its only mid-level dataset of Reddit. 
% PyG ran out of memory on its original design of using the COO format on GCN as discussed above. 
% %Though its newer version supports CSR \td. 
% %Our measurement shows that for the Reddit and Ogb-Product datasets,  Seastar is slower than DGL as per our measurement though the former has accuracy issues. 
% Seastar, Haung et al, and TLPGNN continue to suffer from the same issues that we discussed above. dgNN does not implement GCN or any class B GNN.
% %In this class, which is simpler than class A GNN, we still note that many prior works suffered from the issues of requirement misunderstanding. However, in this class, such as GCN the requirements are simpler as only 

% %We were able to run its SpMMv kernel (after commenting degree-norm and other codes). Table~\ref{table-kernel-time} shows that it performs worse than DGL for both datasets, which we explore in \cref{sec.exp}. Similarly, 
 
% %We have explored many other systems (see \cref{sec.exp} for such systems), though we could not run them end-to-end due to issues mentioned in this section and in \cref{sec.dgl}.

% %This makes DGL and PyG only end-to-end baselines. However, PyG cannot run any GNN model on Reddit which is also shown by prior works~\cite{chen2020fusegnn,huang2021understanding}. Kindly note that our result used its original design of using COO format and torch-scatter as its CUDA kernel that materializes message passing at edge-level resulting in out-of-memory. Its latest release
% %%\footnote{\url{https://pytorch-geometric.readthedocs.io/en/latest/notes/sparse_tensor.html}}  
% %uses CSR format and PyTorch for its back-end, which internally uses Cusparse ({https://github.com/pytorch/pytorch/issues/60854}), 
%  %which we evaluate extensively through DGL and separately.
% %%A natural question is whether we can test various GNN models end-to-end on larger datasets.

% %Previously discussed works continue to see the issues that forbid their reliance due to the requirement misunderstanding and out of memory, such as GNNAdvisor, Haung et al, PyG, etc.,


% We observe more issues in running other works successfully.  
% For example, a lot of other works are not open-source.
% PCGCN~\cite{tian2020pcgcn} does provide an accuracy metric, but the authors have not open-sourced it. Similarly, NeuGraph~\cite{neugraph19atc} is also not open-source.
% GE-SpMM has not shown training time on mid-size datasets. It has been integrated into DGL but is non-functional now due to a major code reorganization in the DGL, which does not allow its compilation and deployment.
% FeatGraph~\cite{featgraphsc20} has shown improvement on top of DGL's old back-end, which was called minigun. Since then, their main design ideas have been integrated with DGL. However, its authors communicated that it is slower than Cusparse-based DGL\footnote{Github URL will be made public for this communication} as we could not run it end-to-end despite help from its authors and trying several Github branches.

% The issues discussed in the last paragraph are not necessarily a problem as such, though it makes \textit{DGL the only system that can be used as a baseline for end-to-end training for future research, and may be termed as the state-of-the-art}.

% %Indeed, many recent papers compare only against DGL if at all they compare; though it keeps showing out-of-memory on many types of GPU. 
% %with the exception of using PyG for smaller datasets.



% \blue{These design choices are responsible for up to 10$\times$ memory consumption (Fig.~\ref{exp-mem}) and a slowdown in DGL, and OOM in PyG. More importantly, the design decisions have introduced a requirement mismatch: a) using SpMMve + a dummy edge-level tensor instead of SpMMv; and b) CusparseSpMM() API supports native SpMMve$^T$, thereby questioning the need for edge ID abstraction and eShuffle design in DGL.}  


\subsubsection{SYS-Others: Other Pitfalls}
The following additional errors have been observed in GCN: no model bias parameter in GNNAdvisor, Huang, et al, and TLPGNN in their GCN; 
%No model bias parameter in dgNN in its GAT; 
and absence of bias and \textit{degree-norm} array in TC-GNN in its GCN. In DGL, the bias parameter is enabled by default, while performing degree-norm operation.
%However, they did not remove the bias parameter from DGL when doing the evaluation. 
In GAT, no dropout layer is there in the fused GAT model of Seastar, TLPGNN, and Huang et al., introducing which requires complex changes to their backend due to the fusion.
%but their evaluation scripts do not disable it, resulting in an unfair performance gain.  
%We indeed measure DGL GCN by commenting bias parameter and notice a drop of 4\%-5\% in \td dataset. This means that these systems may have more hidden but invalid optimizations.
%The discussed pitfalls change the performance characteristic to a large extent, and hence the systems gain performance unfairly compared to baseline systems.
Huang et al use the same allocated memory to keep the attention score for every model layer, which is wrong. 
%TC-GNN evaluation script does not invoke all the kernels that it developed due to an inadequate understanding of CUDA graph capture and replay: GCN does not use the CUDA stream (needed), while AGNN uses it incorrectly. Moreover, 
TC-GNN does not implement SpMM and SDDMM kernels with odd dimensions of feature-length needed in the last layer of GCN and AGNN models, yet its script calls these kernels with those feature lengths. 
%incurring zero runtime. 
These errors indicate serious system design and evaluation issues. 




\subsection{Discussion: Hypothesis and Impact} \label{sec.accuracy.discuss}
The accuracy evaluation is a very time-consuming exercise for systems due to various compilation, installation, and usage issues that are common with academic prototypes. Additional supporting software has since changed substantially, like deprecated APIs. 
Many systems rely on generated features and labels, while each system has its own way of loading the dataset, which takes time to understand and modify to read it from the labeled dataset. 
Hence we limited accuracy evaluation to top-tier conferences only.  
Further, our goal is to be fully sure when we report abnormal accuracy. 
%Many \red{sampling-based GNN} systems do show accuracy, but they suffer from other pitfalls that we discuss in \cref{sec.evaluation}.
%Though we already mentioned that a large body of GNN systems has not shown training accuracy,
It is possible that other systems that did not show accuracy may be correct, but will not solve the pitfall as future works may continue to make erroneous decisions if accuracy is not measured. 
%Further, it may encourage other invalid optimizations as we discuss next.  

%\textbf{Impact.} The impacts are discussed next.

% \textbf{Inadequate Benchmarking Practices.} 
% The results so far suggest an inadequate evaluation that has masked the true comparison of their underlying optimization techniques. If one has to solve the pitfalls using known techniques, such as those proposed by DGL, these works not only will suffer from extreme slowdown but will also increase their memory consumption. \td

\noindent \textbf{Hypothesis: Automatic Backward Computation.}
%We do not doubt the intention of the researcher for the pitfalls, because in that case, they would have not made their code open-source.
%While systems with no backward computation cannot measure the accuracy, we focus on works that at least have a training loop implemented. 
%The datasets used in their experiments are all open-source along with their labels.  %and prior works have access to those datasets anyway. 
%It should be noted that the above systems do provide training scripts if they have a backward computation implemented. Hence, it is not very clear why they would not evaluate the accuracy by adding some additional lines in their code to check accuracy.
We hypothesize that a lack of understanding of the DL framework abstraction could be a reason: the model and layer definitions only explain the forward computation, while the backward code is invoked automatically for each forward operation and remains hidden from the usual code walk-through. 
So many works have either focused on evaluating forward-only computation, where they end up with using performance enhancing bugs while others miss the semantic in backward computation to gain performance in absence of accuracy measurement. 
%We further suspect that tradition from related domains, such as sparse kernel implementation where researchers usually verify the output at the kernel level may have impacted the evaluation strategies.


%shown SpMM performance comparison, but we could not find any GNN system that has specifically compared SpMM$^T$, which appears only in the backward computation. However, such low-level verification needs to be extended to fused kernels, backward kernels, etc. though one cannot verify the backward operations semantically, which is related to requirement understanding such as the order of kernels in fused backward, etc. 
%Hence end-to-end verification such as accuracy measurement is needed. 

% tradition from related domains, such as sparse kernel implementation where researchers usually verify the output at the kernel level may have impacted the evaluation strategies. 
% %When floating point operations are involved, the comparison usually allows some error. 
% Rather, a few GNN systems do contain such code that verifies the output at the kernel level, specifically for forward SpMM kernels.


\noindent
\textbf{Impact.} 
%\noindent 
\textit{Inadequate Training to Future Leaders:}
The discussed pitfalls indicate questionable research practices~\cite{NAP1864}, otherwise, they would not have open-sourced their code. Hence, these works include inappropriate research design and flawed analysis to support a hypothesis. These issues indicate that senior researchers not dedicating enough time to review trainees' deliverable or teach them appropriate research methods~\cite{anderson2007}.
Today's trainee researchers are future leaders, leading to compromised human resource development.

\textit{Questionable Speedup:}
Lack of accuracy measurement breaks an important feedback loop that could make researchers aware of possible issues in system design. The presence of such issues questions whether the claimed speedup is practical or not. In systems, many optimizations are due to better insights into the fundamental trade-offs. A wrong training also implies wrong inference, thereby affecting wider classes of GNN systems. Hence, the performance speedup result could be misleading as we show in \cref{sec.exp.kernel}. 

\textit{Stifling Innovations:}
Baselines play an out-sized impact as they are used in almost all papers. Hence, sub-optimal baseline (DGL/PyG) have inflated the results of other systems, questioning real applicability of many proposed techniques. 
Further, a new system with valid optimization may not outperform pitfall-infested works without committing similar or other pitfalls. Indeed, it is very hard to find a working single-GPU GNN system as a baseline except DGL which can support \textit{both the GNN classes}. Hence if the community is unaware of them, genuine progress in system optimization may not happen.  




%that a few systems are slower against the same baseline to which the paper claimed speedup. %thereby questioning the proposed optimization technique.

%To show this, we measure the kernel runtime of two systems, namely GNNAdvisor and TC-GNN, and compare against Cusparse on Reddit and OGB-Product, and found that both the systems are slower. \td. 

%Apart from the above, that model needed to be almost the same in comparison to prior works unless the new proposed model is discussed and evaluated for the changes. For example, We should not be removing bias parameters without explanation, as it is a mistake. 



% Hence, not measuring and acting on accuracy errors is a sure recipe for errors, leading to questioning the system design itself.


%Such bugs could be because of any aspect that contributes to the end-to-end computation, such as kernel implementation, GNN workflow, integration of kernel to DL frameworks (e.g., Pytorch), and graph preparation itself. The abnormal accuracy does not provide any hint of which parts of aspects have the problems. Out of those possibilities, some bugs are  
%in the system or introduce a new design trade-off thereby compromising the system design and lessons learned. We analyze these works in \cref{sec.semantic}. 


%For systems that do not have backward computation implementation, adding accuracy measurement requires a huge effort based on our own experience. Because they need to consider the integration with the GNN workflow and how to derive and implement backward procedures. Moreover, fixing the bugs in the system level of GNN works is hard and even more time-consuming. 









% may not be sufficient due to the involvement of backward computation and kernel fusion in GNN. For example, if kernel fusion is attempted, the low-level verification requires evaluation at the fused kernel level even if their implementation is fine. While at the backward computation,

% \noindent \textbf{Is Accuracy Measurement Mandatory.}
% Although researchers may decrease their debugging workload by verifying their optimized kernel first, this verification may not always works for an end-to-end GNN computation. That is because kernel verification is calculated by 
% checking the element-wise difference between the proposed kernel and baseline. If the difference is small, the kernel verification can be passed. 

% However, because of the machine precision property(\td not sure), it is hard to guarantee that the small element-wise difference is caused by the machine precision and the proposed kernel is bug-free. (\td maybe the kernel has the bug)

% Based on our own experience, our implemented kernel passed the verification test but actually contains a bug. But that bug causes the accuracy problem after 30 training epochs, the loss becomes NAN and the training accuracy is decreasing. To locate and fix that bug, we spend more than 1 month.

% By enabling the accuracy measurement, the previous pitfalls (P1, P2, P3, P4) as well as other bugs can be avoided. This will lead to the  verification that the proposed optimization is realistic instead of false emulated performance boosts. 



% We realize that it has become a general trend not to include accuracy for many prior works that write their own GNN layers and kernels.~\cite{huang2021understanding, wang2021gnnadvisor, fu2022tlpgnn, wu2021seastar, jangda2021accelerating, liang2020engn, zhang2021boostgcn, kim2022analyzing, yan2020hygcn}.

% \red{\subsection{Not sure}}
% \td simulation results is not accurate, it is overclaimed. Other works kernel have 4 times speed up but the end-to-end is only 1.5 times. 


%Without the accuracy measurement, it is not clear whether the implementation can be used in realistic GNN training. Moreover, without measuring the accuracy, it is likely that some issues in the implementation are unrealized. These issues may corrupt the realistic performance speed-up when deployed.



% \noindent \textbf{Summary.}
% Clearly, the performance gains from these works are not yet practical.
% But the issues that we highlighted have a fundamental impact on the systems research, though have been discovered using their open-source implementation because they do not report the training accuracy. 
% Hence, such fundamental flaws when handled by the researcher itself during accuracy measurement will not only reflect a realistic performance gain but will lead to their adoption, and also improve the system understanding-- an important goal of advancing systems research[cite NSF review criteria]. 


%However, with the accuracy measurement, these flaws can be recognized and fixed, which can guarantee that the implementation and the performance speed-up are realistic and can be deployed directly. 


